Second Order Methods for Bandit Optimization and Control

Bandit convex optimization (BCO) is a general framework for online decision making under uncertainty. While tight regret bounds for general convex losses have been established, existing algorithms achieving these bounds have prohibitive computational costs for high dimensional data. In this paper, we propose a simple and practical BCO algorithm inspired by the online Newton step algorithm. We show that our algorithm achieves optimal (in terms of horizon) regret bounds for a large class of convex functions that we call $\kappa$-convex. This class contains a wide range of practically relevant loss functions including linear, quadratic, and generalized linear models. In addition to optimal regret, this method is the most efficient known algorithm for several well-studied applications including bandit logistic regression. Furthermore, we investigate the adaptation of our second-order bandit algorithm to online convex optimization with memory. We show that for loss functions with a certain affine structure, the extended algorithm attains optimal regret. This leads to an algorithm with optimal regret for bandit LQR/LQG problems under a fully adversarial noise model, thereby resolving an open question posed in \citep{gradu2020non} and \citep{sun2023optimal}. Finally, we show that the more general problem of BCO with (non-affine) memory is harder. We derive a $\tilde{\Omega}(T^{2/3})$ regret lower bound, even under the assumption of smooth and quadratic losses.

==> Backups/average_memory.tex <==
\section{Control setting: BCO with memory}
The problem formulation is as follows:
given convex set $\K\in\mathbb{R}^{d}$, at every time step $t$, the player plays $y_t\in\mathbb{R}^{d}$, suffers quadratic cost $f_t(y_{t-m+1},\dots,y_t)$ that depends on the most recent $m$ steps. The goal is to minimize regret, defined by
\begin{align*}
\sum_{t=m}^T f_t(y_{t-m+1},\dots,y_t)-\min_{x\in\K}\sum_{t=m}^T f_t(x,\dots,x).
\end{align*}
$f_t$'s are assumed to be quadratic, convex, and $\beta$-smooth. In particular, $f_t(z)=\frac{1}{2}z^{\top}H_tz+b_t^{\top}z+c_t$, where $z,b\in\mathbb{R}^{md}, A\in\mathbb{R}^{md\times md}, c\in\mathbb{R}$, and $0\preceq H_t\preceq \beta I$. Define $\bar{f}_t(x)\coloneqq f_t(x,x,\dots x),$ and  define divergence $\nabla \cdot f_t(x_1, \dots x_m) \coloneqq \sum_{i=1}^m \nabla_i f_t(x_1,\dots x_m).$ 


\begin{algorithm}
\caption{bandit quadratic optimization with memory}\label{alg:simple-bqo-memory}
\begin{flushleft}
  {\bf Input:} convex set $\K$, step size $\eta$
\end{flushleft}
\begin{algorithmic}[1]
\STATE Initialize: $x_1 =x_2\dots = x_m\in\K$
\STATE Set $g_0 = g_1 \dots = g_{m-1} = 0$
\STATE Set $A_0 = A_1 \dots = A_{m-1} = I$
\FOR{$t = 1, \ldots, m$}
\STATE Draw $v_{t,1}, v_{t,2}$ uniformly from the unit sphere
\STATE Set $y_t = x_t + \frac{\delta}{2} A_{t-1}^{-1/2}(v_{t,1}+v_{t,2})$
\ENDFOR
\FOR{$t = m, \ldots, T$}
\STATE Play $y_t$, observe $f_t(y_{t-m+1:t})$.
\STATE Create unbiased estimate $\tilde{g}_t$ of $\nabla \cdot f_t(x_{t-m+1:t})$:
\begin{align*}
\tilde{g}_{t}=\frac{2}{\delta}df_t(y_{t-m+1:t}) \sum_{j=0}^{m-1}A_{t-j-1}^{1/2}v_{t-j,1}.
\end{align*}
\STATE Create unbiased estimate $\tilde{H}_t$ of Hessian of $\bar{f}_t$:
\begin{align*}
\tilde{H}_{t}=\frac{2}{\delta^2}d^2 f_t(y_{t-m+1:t})\sum_{j=0}^{m-1}\sum_{k=0}^{m-1}A_{t-j-1}^{1/2}(v_{t-j,1}v_{t-k,2}^{\top}+v_{t-j,2}v_{t-k,1}^{\top})A_{t-k-1}^{1/2}.
\end{align*}
\STATE Update $A_{t} = A_{t-1} + \eta \tilde{H}_t $,
$$ x_{t+1} = \prod_{\K}^{A_{t-m+1}} \left[ x_t - \eta A_{t-m+1}^{-1}  g_{t-m+1}  \right] $$
\STATE Draw $v_{t+1,1}, v_{t+1,2}$ uniformly from the unit sphere around $0$, and let $$y_{t+1}=x_{t+1}+\frac{\delta}{2} A_{t}^{-1/2}(v_{t+1,1}+v_{t+1,2}).$$
\ENDFOR
\end{algorithmic}
\end{algorithm}
\begin{lemma}[Unbiased Gradient and Hessian]
    $\E_t[g_t] = \nabla \cdot  f_t(x_{t-m+1:t})$, and $\E_t[H_t] = \nabla^2 \bar{f}_t(x).$
\end{lemma}
\begin{proof}
 Let $H_t[i,j] \in \mathbb{R}^{d\times d}$ be the $(i,j)^{th}$ sub-matrix of $H_t$, and $b_t[i]\in \mathbb{R}^d$ be the $i^{th}$ sub-vector of $b_t$. Using this notation, we can rewrite $f_t(y_{t-m+1},\dots,y_t)$ as
\[
f_t(y_{t-m+1},\dots,y_t) = \frac{1}{2}\sum_{i=0}^{m-1}\sum_{j=0}^{m-1} y_{t-i}^TH_t[m-i, m-j] y_{t-j} + \sum_{i=0}^{m-1}y_{t-i}^Tb_t[m-i] + c_t.
\]
Define $u_{t,1} \coloneqq A_{t-1}^{-1/2}v_{t,1},$ and $u_t \coloneqq u_{t,1} + u_{t,2}$. Then 
\begin{align*}
    &f_t(y_{t-m+1},\dots,y_t) - f_t(x_{t-m+1},\dots x_t) =\\
    &\quad  \frac{\delta^2}{8}\sum_{i=0}^{m-1}\sum_{j=0}^{m-1} u_{t-i}^TH_t[m-i, m-j] u_{t-j} + \frac{\delta}{2}\sum_{i=0}^{m-1}\sum_{j=0}^{m-1} x_{t-i}^TH_t[m-i, m-j] u_{t-j}\\
    &\quad + \frac{\delta}{2}\sum_{i=0}^{m-1}u_{t-i}^Tb_t[m-i].
\end{align*}

 \noindent\textbf{Gradient.} $\E[\tilde{g}_t]$ can be written as
 \begin{align*}
    \frac{\delta}{2d}  \E[\tilde{g}_t] &=  \E\left[f_t(y_{t-m+1:t}) \sum_{k=0}^{m-1}A_{t-k-1}u_{t-k,1}\right]\\
     & = \E\left[f_t(x_{t-m+1:t}) \sum_{k=0}^{m-1}A_{t-k-1}u_{t-k,1}\right] \\
     & \quad + \frac{\delta^2}{8}\sum_{i=0}^{m-1}\sum_{j=0}^{m-1}\sum_{k=0}^{m-1} \E[u_{t-i}^TH_t[m-i, m-j] u_{t-j} A_{t-k-1}u_{t-k,1}] \\
     & \quad + \frac{\delta}{2}\sum_{i=0}^{m-1}\sum_{j=0}^{m-1}\sum_{k=0}^{m-1} \E[x_{t-i}^TH_t[m-i, m-j] u_{t-j} A_{t-k-1}u_{t-k,1}]\\
     & \quad + \frac{\delta}{2}\sum_{i=0}^{m-1}\sum_{k=0}^{m-1}\E[u_{t-i}^Tb_t[m-i]A_{t-k-1}u_{t-k,1}].
 \end{align*}
Observe that $x_{t-m+1:t}$ is independent of $\{u_{t-k,1}, u_{t-k,2}\}_{k=0}^{m-1}$. Using this observation and the fact that  the first and third moments of $u_t$ are $0$, we can show that the first and second terms in the RHS above are $0$. The third and fourth terms can be bounded using the following observations
 \begin{align*}
    & \sum_{k=0}^{m-1} \E[x_{t-i}^TH_t[m-i, m-j] u_{t-j} A_{t-k-1}u_{t-k,1}] = \frac{1}{d}H_t[m-i, m-j]x_{t-i}\\
     & \sum_{k=0}^{m-1}\E[u_{t-i}^Tb_t[m-i]A_{t-k-1}u_{t-k,1}] = \frac{1}{d}b_t[m-i].
 \end{align*}
 Substituting this in the previous equation shows that
 \begin{align*}
     \frac{\delta}{2d}  \E[\tilde{g}_t] & = \frac{\delta}{2d}\sum_{i=0}^{m-1}\sum_{j=0}^{m-1}H_t[m-i, m-j]x_{t-i}\\
     &\quad + \frac{\delta}{2d} \sum_{i=0}^{m-1}b_t[m-i].
 \end{align*}
 This shows that $\E[\tilde{g}_t] = \nabla \cdot f_t(x_{t-m+1:t}).$\\
 
 \noindent\textbf{Hessian.} Consider the $(k,l)^{th}$ term of $\tilde{H}_t$ which is given by
 \[
\tilde{H}_{t,k,l} \coloneqq f_t(x_{t-m+1:t}) A_{t-k-1}(u_{t-k,1}u_{t-l,2}^{\top}+u_{t-k,2}u_{t-l,1}^{\top})A_{t-l-1}.
 \]
 Observe that $\tilde{H}_t = \sum_{k=0}^{m-1}\sum_{l=0}^{m-1}\tilde{H}_{t,k,l}.$
Now consider the following
 \begin{align*}
    \frac{\delta^2}{2d^2}  \E[\tilde{H}_{t,k,l}] &=  \E\left[f_t(y_{t-m+1:t}) A_{t-k-1}(u_{t-k,1}u_{t-l,2}^{\top}+u_{t-k,2}u_{t-l,1}^{\top})A_{t-l-1}\right]\\
    & = \E\left[f_t(x_{t-m+1:t}) A_{t-k-1}(u_{t-k,1}u_{t-l,2}^{\top}+u_{t-k,2}u_{t-l,1}^{\top})A_{t-l-1}\right] \\
     & \quad + \frac{\delta^2}{8}\sum_{i=0}^{m-1}\sum_{j=0}^{m-1} \E[u_{t-i}^TH_t[m-i, m-j] u_{t-j} A_{t-k-1}(u_{t-k,1}u_{t-l,2}^{\top}+u_{t-k,2}u_{t-l,1}^{\top})A_{t-l-1}] \\
     & \quad + \frac{\delta}{2}\sum_{i=0}^{m-1}\sum_{j=0}^{m-1} \E[x_{t-i}^TH_t[m-i, m-j] u_{t-j} A_{t-k-1}(u_{t-k,1}u_{t-l,2}^{\top}+u_{t-k,2}u_{t-l,1}^{\top})A_{t-l-1}]\\
     & \quad + \frac{\delta}{2}\sum_{i=0}^{m-1}\E[u_{t-i}^Tb_t[m-i]A_{t-k-1}(u_{t-k,1}u_{t-l,2}^{\top}+u_{t-k,2}u_{t-l,1}^{\top})A_{t-l-1}].
 \end{align*}
 It is easy to check that the first, third and last terms in the RHS are exactly equal to 0 (this follows from the fact that odd moments of $u_t$ are 0). The second term can be shown to be equal to 
 \[
 \sum_{i=0}^{m-1}\sum_{j=0}^{m-1} \E[u_{t-i}^TH_t[m-i, m-j] u_{t-j} A_{t-k-1}(u_{t-k,1}u_{t-l,2}^{\top}+u_{t-k,2}u_{t-l,1}^{\top})A_{t-l-1}] = \frac{4}{d^2}H_t[m-k, m-l].
 \]
 Plugging this in the previous equation shows that $\tilde{H}_t  = \sum_{k=0}^{m-1}\sum_{l=0}^{m-1} H_t[m-k, m-l] = \nabla^2 \bar{f}_t.$
\end{proof}
% \begin{proof}
%  Let $H_t[i,j] \in \mathbb{R}^{d\times d}$ be the $(i,j)^{th}$ sub-matrix of $H_t$, and $b_t[i]\in \mathbb{R}^d$ be the $i^{th}$ sub-vector of $b_t$. Using this notation, we can rewrite $f_t(y_{t-m+1},\dots,y_t)$ as
% \[
% f_t(y_{t-m+1},\dots,y_t) = \frac{1}{2}\sum_{i=0}^{m-1}\sum_{j=0}^{m-1} y_{t-i}^TH_t[m-i, m-j] y_{t-j} + \sum_{i=0}^{m-1}y_{t-i}^Tb_t[m-i] + c_t.
% \]
% Define $u_{t} \coloneqq A_{t-1}^{-1/2}v_{t}$. Then 
% \begin{align*}
%     &f_t(y_{t-m+1},\dots,y_t) - f_t(x_{t-m+1},\dots x_t) =\\
%     &\quad  \frac{1}{2}\sum_{i=0}^{m-1}\sum_{j=0}^{m-1} u_{t-i}^TH_t[m-i, m-j] u_{t-j} + \sum_{i=0}^{m-1}\sum_{j=0}^{m-1} x_{t-i}^TH_t[m-i, m-j] u_{t-j}\\
%     &\quad + \sum_{i=0}^{m-1}u_{t-i}^Tb_t[m-i].
% \end{align*}

%  \noindent\textbf{Gradient.} $\E[\tilde{g}_t]$ can be written as
%  \begin{align*}
%      \E[\tilde{g}_t] &=  \E\left[f_t(y_{t-m+1:t}) \sum_{k=0}^{m-1}A_{t-k-1}u_{t-k}\right]\\
%      & = \E\left[f_t(x_{t-m+1:t}) \sum_{k=0}^{m-1}A_{t-k-1}u_{t-k}\right] \\
%      & \quad + \frac{1}{2}\sum_{i=0}^{m-1}\sum_{j=0}^{m-1}\sum_{k=0}^{m-1} \E[u_{t-i}^TH_t[m-i, m-j] u_{t-j} A_{t-k-1}u_{t-k}] \\
%      & \quad + \sum_{i=0}^{m-1}\sum_{j=0}^{m-1}\sum_{k=0}^{m-1} \E[x_{t-i}^TH_t[m-i, m-j] u_{t-j} A_{t-k-1}u_{t-k}]\\
%      & \quad + \sum_{i=0}^{m-1}\sum_{k=0}^{m-1}\E[u_{t-i}^Tb_t[m-i]A_{t-k-1}u_{t-k}].
%  \end{align*}
% Observe that $x_{t-m+1:t}$ is independent of $\{u_{t-k}\}_{k=0}^{m-1}$. Using this observation and the fact that  the first and third moments of $u_t$ are $0$, we can show that the first and second terms in the RHS above are $0$. The third and fourth terms can be bounded using the following observations
%  \begin{align*}
%     & \sum_{k=0}^{m-1} \E[x_{t-i}^TH_t[m-i, m-j] u_{t-j} A_{t-k-1}u_{t-k}] = H_t[m-i, m-j]x_{t-i}\\
%      & \sum_{k=0}^{m-1}\E[u_{t-i}^Tb_t[m-i]A_{t-k-1}u_{t-k}] =b_t[m-i].
%  \end{align*}
%  Substituting this in the previous equation shows that
%  \begin{align*}
%       \E[\tilde{g}_t] & = \sum_{i=0}^{m-1}\sum_{j=0}^{m-1}H_t[m-i, m-j]x_{t-i} +  \sum_{i=0}^{m-1}b_t[m-i].
%  \end{align*}
%  This shows that $\E[\tilde{g}_t] = \nabla \cdot f_t(x_{t-m+1:t}).$\\
 
%  \noindent\textbf{Hessian.} Consider the $(k,l)^{th}$ term of $\tilde{H}_t$ which is given by
%  \[
% \tilde{H}_{t,k,l} \coloneqq f_t(x_{t-m+1:t}) A_{t-k-1}^{1/2}(v_{t-k}v_{t-l}^{\top}-\ind{k=l}I)A_{t-l-1}^{1/2}.
%  \]
%  Observe that $\tilde{H}_t = \sum_{k=0}^{m-1}\sum_{l=0}^{m-1}\tilde{H}_{t,k,l}.$
% Now consider the following
%  \begin{align*}
%     \E[\tilde{H}_{t,k,l}] &=  \E\left[f_t(y_{t-m+1:t}) A_{t-k-1}^{1/2}(v_{t-k}v_{t-l}^{\top}-\ind{k=l}I)A_{t-l-1}^{1/2}\right]\\
%     & = \E\left[f_t(x_{t-m+1:t}) A_{t-k-1}^{1/2}(v_{t-k}v_{t-l}^{\top}-\ind{k=l}I)A_{t-l-1}^{1/2}\right] \\
%      & \quad + \sum_{i=0}^{m-1}\sum_{j=0}^{m-1} \E[u_{t-i}^TH_t[m-i, m-j] u_{t-j} A_{t-k-1}^{1/2}(v_{t-k}v_{t-l}^{\top}-\ind{k=l}I)A_{t-l-1}^{1/2}] \\
%      & \quad + \sum_{i=0}^{m-1}\sum_{j=0}^{m-1} \E[x_{t-i}^TH_t[m-i, m-j] u_{t-j} A_{t-k-1}^{1/2}(v_{t-k}v_{t-l}^{\top}-\ind{k=l}I)A_{t-l-1}^{1/2}]\\
%      & \quad + \sum_{i=0}^{m-1}\E[u_{t-i}^Tb_t[m-i]A_{t-k-1}^{1/2}(v_{t-k}v_{t-l}^{\top}-\ind{k=l}I)A_{t-l-1}^{1/2}].
%  \end{align*}
%  Consider the first term in the RHS above. It's expectation is determined by $$\E[A_{t-k-1}^{1/2}(v_{t-k}v_{t-l}^{\top}-\ind{k=l}I)A_{t-l-1}^{1/2}].$$ When $k\neq l,$ it is easy to see that the expectation is $0$. When $k = l,$ the expectation is again $0$ because $\E[A_{t-k-1}^{1/2}v_{t-k}v_{t-l}^{\top}A_{t-l-1}^{1/2}] = \E[A_{t-k-1}^{1/2}A_{t-l-1}^{1/2}].$ \js{should there be a dimension factor $d$ here?} 
%   Next, the third and last terms in the RHS can be shown to be  exactly equal to 0 (this follows from the fact that odd moments of $u_t$ are 0). The second term can be shown to be equal to 
%  \begin{align*}
%     \sum_{i=0}^{m-1}\sum_{j=0}^{m-1} \E[u_{t-i}^TH_t[m-i, m-j] u_{t-j}  A_{t-k-1}^{1/2}(v_{t-k}v_{t-l}^{\top}-\ind{k=l}I)A_{t-l-1}^{1/2}] = H_t[m-k, m-l]. 
%  \end{align*}
%  Plugging this in the previous equation shows that $\tilde{H}_t  = \sum_{k=0}^{m-1}\sum_{l=0}^{m-1} H_t[m-k, m-l] = \nabla^2 \bar{f}_t.$
%  \end{proof}

\begin{theorem}
\label{lem:expected_regret_bound_bco_memory}
Suppose the adversary is oblivious. Moreover, suppose the sequence of loss functions chosen by the adversary are smooth and bounded. Suppose the algorithm is run with $\eta = T^{-1/2}$. Then the following holds for any $x\in\K$,
$$   \sum_{t=m}^T \E[f_t(y_{t-m+1:t})  -  \bar{f}_t(x)] = O(\sqrt{T}).    $$
\end{theorem}
\begin{proof}
Let's assume the estimated cumulative Hessian concentrates around the true cumulative Hessian.
\begin{align*}
\sum_{t=m}^T \E[f_t(y_{t-m+1:t})  -  \bar{f}_t(x)]& = \underbrace{\sum_{t=m}^T\E[f_t(y_{t-m+1:t})  -  f_t(x_{t-m+1:t})]}_{(1)} + \underbrace{\sum_{t=m}^T\E[f_t(x_{t-m+1:t})  -  \bar{f}_t(x_t)]}_{(2)}\\
&\quad + \underbrace{\sum_{t=m}^T\E[\bar{f}_t(x_t) - \bar{f}_t(x)]}_{(3)}
\end{align*}
The first and third terms can be bounded using similar arguments as in the proof of Theorem~\ref{lem:expected_regret_bound}. The second term relies on the stability of iterates and can be bounded as follows \dots

\end{proof}
\begin{remark}
    Related work \cite{gradu2020non}.
\end{remark}

\newpage

\subsection{With-memory regret analysis}

\subsubsection{Definitions and assumptions}
\label{sec:with-memory-loss-defs-and-assumptions}

\paragraph{Setting.} At time $t$, the learner chooses an action $y_t\in\mathbb{R}^d$, and the adversary reveals a convex quadratic cost function $f_t$ that depends on at most $N$ of the learner's past decisions. However, these past decisions can come from any of the previous time steps. Denote the memory set at time $t$ as $m(t)$ such that $m(t)$ satisfies: 
\begin{enumerate}
\item $t\in m(t)$, $\forall s\in m(t)$, $s\le t$,
\item $N=\max_{t}|m(t)|$,
\item Denote as $\first(t)=\min_{s\in m(t)} s$. $M=\frac{1}{T}\sum_{t=1}^T t-\first(t)$. 
\end{enumerate}
We will assume that $N, M=\Theta (\log T)$. For a given $\alpha\in (0,1)$, let $S_{\alpha}=\{t: t-\first(t)> MT^{\alpha}\}$. Then, $S_{\alpha}$ satisfies $|S_{\alpha}|\le T^{1-\alpha}$. Denote $H=MT^{\alpha}$. 

At time $t$, a loss function $f_t:\mathbb{R}^{d|m(t)|}\rightarrow \mathbb{R}_{+}$ is given. $f_t$ satisfies the following assumptions over a convex set $\K^{|m(t)|}$, where $\K\subset\mathbb{R}^d$ is a compact, convex subset of $\mathbb{R}^d$:
\begin{enumerate}
\item (Quadratic) $f_t$ admits the following representation: $\exists H_t\in\mathbb{R}^{d|m(t)|\times d|m(t)|}$, $b_t\in\mathbb{R}^{d|m(t)|}$, $d_t\in\mathbb{R}$ such that $f_t(z)=\frac{1}{2}z^{\top}H_t z+b_t^{\top}z+d_t$, $\forall z\in\mathbb{R}^{d|m(t)|}$. 
\item (Convexity) $H_t\succeq 0$. 
\item (Smoothness) $H_t\preceq \beta I_{|m(t)|\times |m(t)|}$, $\beta >0$. 
\item (Diameter and gradient bounds) $\K$ has Euclidean diameter bound $D$, i.e. $\sup_{x,y\in\K}\|x-y\|_2\le D$. $f_t$ has diameter bound $B$ and gradient bound $G$ over $\K^{|m(t)|}$, i.e.
\begin{align*}
\sup_{t\in [T]}\sup_{\mathbf{x}\in\K^{|m(t)|}} f_t(x) \le B, \ \ \ \sup_{t\in[T]} \sup_{\mathbf{x}\in\K^{|m(t)|}} \|\nabla f_t(x)\|_2 \le G.
\end{align*}
\end{enumerate}
Define the \textit{unary form} of $f_t$ as following: $\bar{f}_{t}:\mathbb{R}^{d}\rightarrow\mathbb{R}_{+}$ is the unary form of $f_t$ if $\bar{f}_{t}(x)=f_t(x,\dots,x)$, $\forall x\in\mathbb{R}^d$. 
\begin{remark}
$\bar{f}_{t}$ is quadratic, convex, and $|m(t)|\beta$-smooth. 
\begin{enumerate}
\item (Quadratic) $\bar{f}_{t}(x)=\frac{1}{2}x^{\top}\left(\sum_{i,j=1}^{|m(t)|} (H_t)_{ij}\right)x+\left(\sum_{i=1}^{|m(t)|} (b_t)_{i}\right)^{\top}x+d_t$, where $(H_t)_{ij}$ is the $ij$-th $d\times d$ block of $H_t$, $(b_t)_i$ is the $i$-th $d$-block of $b_t$. Namely, $(H_t)_{ij}=H_t[(i-1)d+1:id, (j-1)d+1:jd]$, $(b_t)_i=b_t[(i-1)d+1:id]$.
\item (Convex) It is easy to check that $\nabla\bar{f}_{t}(y)=\sum_{i=1}^{|m(t)|}\nabla_if_t(z_1,\dots,z_{|m(t)|})\mid_{z_1=\dots=z_{|m(t)|}=y}$. By convexity of $f_t$, $\forall x,y\in\mathbb{R}^{d}$,
\begin{align*}
\bar{f}_{t}(y)-\bar{f}_{t}(x)&\le \nabla f_t(y\mathbf{1}_{|m(t)|})^{\top}(y\mathbf{1}_{|m(t)|}-x\mathbf{1}_{|m(t)|})\\
&=\sum_{i=1}^{|m(t)|} \nabla_if_t(z_1,\dots,z_{|m(t)|})\mid_{z_1=\dots=z_{|m(t)|}=y}(y-x)\\
&=\nabla\bar{f}_{t}(y)^{\top}(y-x). 
\end{align*}
\item (Smooth) $\bar{f}_{t}$ is $|m(t)|\beta$-smooth since
\begin{align*}
\bar{f}_{t}(y)-\bar{f}_{t}(x)&\le \nabla f_{t}(x\mathbf{1}_{|m(t)|})^{\top}(y\mathbf{1}_{|m(t)|}-x\mathbf{1}_{|m(t)|})+\frac{\beta}{2}\|y\mathbf{1}_{|m(t)|}-x\mathbf{1}_{|m(t)|}\|_2^2\\
&=\nabla \bar{f}_{t}(x)^{\top}(y-x)+\frac{|m(t)|\beta}{2}\|y-x\|_2^2.
\end{align*}
\end{enumerate}
\end{remark}

\subsubsection{Algorithm}
We introduce a gradient based efficient algorithm that achieves sublinear regret in this setting. The algorithm makes use of the self-concordant barrier, which given by the following definition. 
\begin{definition} [Self-concordant barrier]
A $C^3$ function $R(\cdot)$ over a closed convex set $\K\subset\mathbb{R}^d$ with non-empty interior is a $\nu$-self-concordant barrier of $\K$ if it satisfies the following two properties:
\begin{enumerate}
\item (Boundary property) For any sequence $\{x_n\}_{n\in\mathbb{N}}\subset \mathrm{int}(\K)$ such that $\lim_{n\rightarrow\infty}x_n=x\in\partial\K$, $\lim_{n\rightarrow\infty}R(x_n)=\infty$. 
\item (Self-concordant) $\forall x\in\mathrm{int}(\K)$, $h\in\mathbb{R}^d$, 
\begin{enumerate}
\item $|\nabla^3R(x)[h,h,h]|\le 2|\nabla^2 R(x)[h,h]|^{3/2}$.
\item $|\langle \nabla R(x),h\rangle|\le \sqrt{\nu}|\nabla^2 R(x)[h,h]|^{1/2}$. 
\end{enumerate}
\end{enumerate}
\end{definition} 

Self-concordant functions satisfy the following properties, which we will make use of in our regret analysis of Algorithm~\ref{alg:bqo-memory-first-order}:

\begin{proposition}  $\nu$-self-concordant barriers over $\K$ satisfy the following properties:
\label{prop:self-concordant-barrier}
\begin{enumerate}
\item Sum of two self-concordant functions is self-concordant. Linear and quadratic functions are self-concordant.
\item If $x,y\in\K$ satisfies $\|x-y\|_{\nabla^2 R(x)}<1$, then the following inequality holds:
\begin{align}
(1-\|x-y\|_{\nabla^2 R(x)})^2 \nabla^2 R(x)\preceq \nabla^2 R(y)\preceq \frac{1}{(1-\|x-y\|_{\nabla^2 R(x)})^2}\nabla^2 R(x). \label{eqn:scb-hessian-inequality}
\end{align}
\item The Dikin ellipsoid centered at any point in the interior of $\K$ w.r.t. a self-concordant barrier $R(\cdot)$ over $\K$ is completely contained in $\K$. Namely,
\begin{align}
\{y\in\mathbb{R}^d\mid \|y-x\|_{\nabla^2 R(x)}\le 1\}\subset \K, \ \ \forall x\in \text{int}(\K). \label{eqn:dikin-ellipsoid}
\end{align}
where 
\begin{align*}
    \|v\|_{\nabla^2 R(x)}\defeq\sqrt{v^\top \nabla^2 R(x) v}
\end{align*}
\item $\forall x,y\in\text{int}(\K)$:
\begin{align*}
R(y)-R(x)\le \nu\log\frac{1}{1-\pi_x(y)},
\end{align*}
where $\pi_x(y)\defeq\inf\{t\ge0:x+t^{-1}(y-x)\in\K\}$.
\item If $\K$ does not contain any straight lines, then $\nabla^2 R(x)\succ 0$, $\forall x\in\mathrm{int}(\K)$.
\end{enumerate}
\end{proposition}

\begin{algorithm}
\caption{Bandit Quadratic Optimization with Memory (\texttt{BQO-M})}\label{alg:bqo-memory-first-order}
\begin{flushleft}
{\bf Input:} convex set $\K$, step size $\eta>0$, perturbation parameter $\delta\in[0,1]$, self-concordant barrier $R$ over $\K$ with Hessian lower bounded by $\lambda I$, $\lambda > 0$, memory capacity $H$. 
\end{flushleft}
\begin{algorithmic}[1]
\STATE Initialize: $x_1=\dots=x_H\in\argmin_{x\in\K} R(x)$, set $A_i=\nabla^2 R(x_i)$, $\forall 1\le i\le H$.
\STATE Sample $u_1,\dots, u_H\sim S^{d-1}$ i.i.d. uniformly at random.
\STATE Set $y_i = x_i + \delta A_{i}^{-\frac{1}{2}}u_i$, $\forall 1\le i\le H$. Set $g_i=0$, $\forall 1\le i\le H-1$. 
\FOR{$t = H, \ldots, T$}
\STATE Play $y_t$, observe $f_t(y_{m(t)})$.
\STATE Create gradient estimator:
\begin{align*}
\tilde{g}_{t}&=\frac{d}{\delta}f_t(y_{m(t)}) \sum_{s=t-H+1}^{t}A_{s}^{\frac{1}{2}}u_{s}\in\mathbb{R}^{d}.
\end{align*}
\STATE Update
$ x_{t+1} = \argmin_{x\in\K} \eta\sum_{s=1}^{t-H+1} \langle \tilde{g}_{s}, x\rangle + R(x)$, $A_{t+1}=\nabla^2 R(x_{t+1})$. 
\STATE Independently from previous steps, sample $u_{t+1}\sim S^{d-1}$ uniformly at random. 
\STATE Set $y_{t+1}=x_{t+1}+\delta A_{t+1}^{-\frac{1}{2}}u_{t+1}$. 
\ENDFOR
\end{algorithmic}
\end{algorithm}


\subsubsection{Analysis}
\begin{lemma} [Lemma 14 in~\cite{hazan2014bandit}]
\label{lem:newton-decrement}
For a self-concordant function $R$ over $\K$, if the Newton decrement $\lambda(x, R)=\|\nabla R(x)\|_{\nabla^2R(x)}^*\le \frac{1}{2}$, then
\begin{align*}
\|x-\argmin_{x\in\K} R(x)\|_{\nabla^2R(x)}\le 2 \lambda(x,R).
\end{align*}
\end{lemma}

\paragraph{Correctness and independence.} We make the following observations of Algorithm~\ref{alg:bqo-memory-first-order}:
\begin{itemize}
\item (Correctness) All $y_t$'s played by Algorithm~\ref{alg:bqo-memory-first-order} satisfy that $y_t\in\K$ since $\|y_t-x_t\|_{\nabla^2 R(x_t)}^2=\delta^2 u_t^{\top}A_{t}^{-\frac{1}{2}}A_tA_t^{-\frac{1}{2}}u_t=\delta^2\le 1$. By the secocnd property in Proposition~\ref{prop:self-concordant-barrier}, $y_t\in\K$. 
\item (Independence) Let $\F_t=\sigma(\{u_s\}_{s\le t})$ denote the filtration generated by the algorithm's random sampling of noises up to time $t$. By construction, $x_t, A_t$ is $\F_{t-H}$-measurable, and $y_t, \tilde{g}_t$ is $\F_t$-measurable. In particular, $x_t, A_t$ are independent of the algorithm's sampled random vectors $u_{t-H+1:t}$.
\end{itemize}


The expected regret against any $x\in\K$ can be decomposed as the following:
\begin{align*}
\E[\regret_T]=\underbrace{\sum_{t=1}^T \E[f_t(y_{m(t)})-f_t(x_{m(t)})]}_{(1):\text{exploration loss}}+\underbrace{\sum_{t=1}^T \E[f_t(x_{m(t)})-\bar{f}_t(x_t)]}_{(2):\text{movement loss}}+\underbrace{\sum_{t=1}^T \E[\bar{f}_t(x_t)-\bar{f}_t(x)]}_{(3):\text{underlying regret}}\, .
\end{align*}
We will bound each of the terms respectively. 

\paragraph{Bounding exploration loss.} By Taylor expansion and $\beta$-smoothness assumption, the exploration loss can be bounded by
\begin{align*}
\sum_{t=1}^T \E[f_t(y_{m(t)})-f_t(x_{m(t)})]&\le \delta\sum_{t=1}^T \E[\nabla f_t(x_{m(t)})^{\top}A_{m(t)}^{-\frac{1}{2}}u_{m(t)}]+\frac{\delta^2\beta}{2}\sum_{t=1}^T\E[u_{m(t)}^{\top}A_{m(t)}^{-1}u_{m(t)}].
\end{align*}
The first term is $0$ since by delayed independence,
\begin{align*}
\E[\nabla f_t(x_{m(t)})^{\top}A_{m(t)}^{-\frac{1}{2}}u_{m(t)}]=\E[\nabla f_t(x_{m(t)})^{\top}A_{m(t)}^{-\frac{1}{2}}\E[u_{m(t)}\mid \F_{t-H}]]=0.
\end{align*}
The second term can be bounded by
\begin{align*}
\frac{\delta^2\beta}{2}\sum_{t=1}^T\E[u_{m(t)}^{\top}A_{m(t)}^{-1}u_{m(t)}]&=\frac{\delta^2\beta}{2}\sum_{t=1}^T\sum_{s\in m(t)}\E[u_{s}^{\top}(\nabla^2 R(x_s))^{-1}u_{s}]\\
&\le \frac{\delta^2\beta}{2}\sum_{t=1}^T\sum_{s\in m(t)}\frac{1}{\lambda}\\
&\le \frac{\delta^2\beta NT}{2\lambda}.
\end{align*}

\paragraph{Bounding movement loss.} We first establish a bound on the neighboring iterates and gradient estimators produced by Algorithm.~\ref{alg:bqo-memory-first-order}.

\begin{lemma} [Iterates and gradient bounds]
\label{lem:iterate-grad-bounds}
$\forall t\ge 2$, the following two inequalities holds assuming $16\eta\delta^{-1}dBH^2\le 1$:
\begin{enumerate}
\item $(1-4\eta \delta^{-1}dBH)^2 A_{t-1}\preceq A_t\preceq (1-4\eta\delta^{-1}dBH)^{-2}A_{t-1}$,
\item $\|\tilde{g}_s\|_{A_{t-1}}^*\le 2\delta^{-1}dBH$, $\forall t-H\le s\le t-1$. 
\end{enumerate}
\end{lemma}
\begin{proof}
We show the two inequalities via induction. Note that by design of Algorithm~\ref{alg:bqo-memory-first-order}, we have that $x_1=x_2\in\argmin_{x\in \K}R(x)$, and $g_1=0$. Thus, the base case holds clearly. 

Suppose the two inequalities holds for some $t$. Consider for $t+1$. We have for fixed $s\in[t-H+1, t]$,
\begin{align*}
\left(\|\tilde{g}_s\|_{A_t}^*\right)^2&\le \left(\frac{dB}{\delta}\right)^2 \sum_{q,r=s-H+1}^{s}u_q^{\top} A_{q}^{\frac{1}{2}} A_t^{-1} A_{r}^{\frac{1}{2}} u_r\\
&\le \left(\frac{dBH}{\delta}\right)^2\max_{s-H+1\le r\le s} u_r^{\top} A_{r}^{\frac{1}{2}}A_t^{-1}A_r^{\frac{1}{2}}u_r\\
&\le \left(\frac{dBH}{\delta}\right)^2\max_{s-H+1\le r\le s} \|A_{r}^{\frac{1}{2}}A_t^{-1}A_r^{\frac{1}{2}}\|_2\\
&=\left(\frac{dBH}{\delta}\right)^2\max_{s-H+1\le r\le s} \|A_{r}^{\frac{1}{2}}A_t^{-1}A_r^{-\frac{1}{2}}\|_2.
\end{align*}
By induction hypothesis, we have $r$ in the interval $\forall s-H+1\le r\le s$, 
\begin{align*}
A_r\preceq (1-4\eta \delta^{-1}dBH)^{-2(t-r)}A_t\preceq (1-4\eta \delta^{-1}dBH)^{-4H} A_t.
\end{align*}
Thus,
\begin{align*}
\|\tilde{g}_s\|_{A_t}^* \le \frac{dBH}{\delta} (1-4\eta \delta^{-1}dBH)^{-2H}\le \frac{dBH}{\delta} (1-8\eta \delta^{-1}dBH^2)\le \frac{2dBH}{\delta},
\end{align*}
where the second inequality follows from Bernoulli's inequality that $(1+x)^r\ge 1+rx$ for every $x\ge -1$, $r\ge 1$, and the last inequality follows from the assumption that $16\eta\delta^{-1}dBH^2\le 1$. 

Define $\Phi_t(x)=\eta\sum_{s=1}^{t-H} \langle\tilde{g}_s, x\rangle + R(x)$, $\forall t\ge H$. Then $x_t\in \argmin_{x\in\K} \Phi_t(x)$. By Lemma~\ref{lem:newton-decrement}, we have
\begin{align*}
\|x_t-x_{t+1}\|_{A_t}\le 2\|\nabla \Phi_{t+1}(x_t)\|_{A_t}^*=2\eta\|\tilde{g}_{t-H+1}\|_{A_t}^*\le \frac{4\eta dBH}{\delta},
\end{align*}
where the equality comes from that $\Phi_{t+1}(x)=\Phi_{t}(x)+\eta\tilde{g}_{t-H+1}$ and $x_t$ is the minimizer of $\Phi_t(\cdot)$. By the second property in Proposition~\ref{prop:self-concordant-barrier}, we have
\begin{align*}
\left(1-\frac{4\eta dBH}{\delta}\right)^2 A_t\preceq A_{t+1}\preceq \left(1-\frac{4\eta dBH}{\delta}\right)^{-2}A_t.
\end{align*}
\end{proof}

Lemma~\ref{lem:iterate-grad-bounds} and the Lipschitz assumption on the loss functions directly implies a bound on the movement loss. Since 
\begin{align*}
\|x_t-x_{t+1}\|_2\le \frac{1}{\lambda} \|x_t-x_{t+1}\|_{A_t}\le \frac{4\eta dBH}{\lambda \delta},
\end{align*}
we have
\begin{align*}
\sum_{t=1}^T \E[f_t(x_{m(t)})-\bar{f}_{t}(x_t)]&\le G\sum_{t=1}^T \sum_{s\in m(t)} \E[\|x_s-x_t\|_2]\\
&\le G\sum_{t=1}^T \sum_{s\in m(t)} \frac{4\eta dBH(t-s)}{\lambda \delta}\\
&\le \frac{4\eta dGBNH}{\lambda\delta}\sum_{t=1}^T t-\first(t)\\
&\le \frac{4\eta dGBNMHT}{\lambda\delta}. 
\end{align*}

\paragraph{Bounding underlying regret.} We split the term of underlying regret further into two terms: the FTRL-sum and the gradient bias:
\begin{align*}
\sum_{t=1}^T \E[\bar{f}_{t}(x_t)-\bar{f}_{t}(x)]&\le \sum_{t=1}^T\E[\nabla \bar{f}_t(x_t)^{\top} (x_t-x)]\\
&= \underbrace{\sum_{t=H}^T\E[\tilde{g}_{t}^{\top} (x_t-x)]}_{((a):\text{ FTRL-sum})}+\underbrace{\sum_{t=1}^T\E[(\nabla \bar{f}_t(x_t)-\E[\tilde{g}_t\mid \F_{t-H}])^{\top}(x_t-x)]}_{((b):\text{ gradient bias})}.
\end{align*}
We bound the two terms respectively. To bound the FTRL-sum, we use a variant of the FTL-BTL lemma for our delayed gradient updates:
\begin{lemma} [FTL-BTL variant]
$\forall x\in\K$, $\forall T$, the following inequality holds:
\begin{align*}
\eta\sum_{t=H}^T \langle\tilde{g}_t, x\rangle + R(x)\ge \eta \sum_{t=H}^T \langle \tilde{g}_t, x_{t+H}\rangle + R(x_{2H-1}). 
\end{align*}
\end{lemma}
\begin{proof}
We show the proof by induction. Fix $x\in\K$. If $T\le H$, by algorithm design since $\tilde{g}_1=\dots=\tilde{g}_{H-1}=0$, we have $x_{2H-1}=\argmin_{x\in\K}R(x)$, and thus $R(x_{2H-1})\le R(x)$. 

Suppose the above inequality holds for some $T$. Then, since 
\begin{align*}
x_{T+H+1}=\argmin_{x\in\K} \eta\sum_{t=H}^{T+1}\langle \tilde{g}_{t}, x\rangle + R(x),
\end{align*}
we have
\begin{align*}
\eta\sum_{t=H}^{T+1} \langle\tilde{g}_t, x\rangle + R(x)&\ge \eta\sum_{t=H}^{T+1} \langle\tilde{g}_t, x_{T+H+1}\rangle + R(x_{T+H+1})\\
&\ge \eta \langle \tilde{g}_t, x_{T+H+1}\rangle +\eta\sum_{t=H}^{T} \langle\tilde{g}_t, x_{t+H}\rangle + R(x_{2H-1})\\
&=\eta\sum_{t=H}^{T+1} \langle\tilde{g}_t, x_{t+H}\rangle + R(x_{2H-1}). 
\end{align*}
\end{proof}
Therefore, the FTRL-sum term is bounded by
\begin{align*}
\sum_{t=H}^T \E[\tilde{g}_t^{\top} (x_t-x)]&\le\sum_{t=H}^T \E[\tilde{g}_t^{\top}(x_t-x_{t+H})] + \frac{1}{\eta} (R(x)-R(x_{2H-1}))\\
&\le\sum_{t=H}^T \sum_{s=t}^{t+H-1} \E[\tilde{g}_t^{\top}(x_s-x_{s+1})]+\frac{R(x)}{\eta}\\
&\le \sum_{t=H}^T \sum_{s=t}^{t+H-1} \E[\|\tilde{g}_t\|_{A_s}\|x_s-x_{s+1}\|_{A_s}^*]+\frac{R(x)}{\eta}\\
&\le \frac{8\eta d^2B^2H^3T}{\delta^2}+\frac{\nu \log T}{\eta}.
\end{align*}

\js{TODO: explain why we can assume $R(x)\le \nu \log T$.}

It is left to show the gradient bias. First, we note that by construction, $\forall t\notin S_{\alpha}$, we have that $\tilde{g}_t$ is an unbiased estimator of the following statistics of $f_t$:
\begin{lemma} [Unbiased estimator]
\label{lem:unbiased-div}
$\forall t\notin S_{\alpha}$, $\tilde{g}_t$ satisfies
\begin{align*}
\E[\tilde{g}_t\mid \F_{t-H}]=\sum_{i\in [|m(t)|]}[\nabla f_t(x_{m(t)})]_i,
\end{align*}
where $[\nabla f_t(x_{m(t)})]_i$ denotes the $i$-th chunk of $\mathbb{R}^d$ vector in $\nabla f_t(x_{m(t)})\in\mathbb{R}^{d|m(t)|}$, i.e. if $\nabla f_t(x_{m(t)})=(v_1,\dots,v_{d|m(t)|})$, then $[\nabla f_t(x_{m(t)})]_i=(v_{d(i-1)+1},\dots,v_{di})$, $i\in [1, |m(t)|]\cap \mathbb{Z}_{++}$. 
\end{lemma}
\begin{proof}
First, for a given symmetric, positive semi-definite matrix $A$, and a deterministic quadratic function $q(x)=\frac{1}{2}x^{\top} Qx+p^{\top}x+c$ over $\mathbb{R}^d$, we have that for a random vector $v$ drawn from a centered distribution such that all odd moments are $0$ and $\E[vv^{\top}]=rI$, $\forall \eps >0$,
\begin{align*}
\frac{1}{r\eps}\E[q(x+\eps A^{-1}v)Av]&=\frac{1}{r\eps}\left(\E\left[\frac{1}{2}(x+\eps A^{-1}v)^{\top}Q(x+\eps A^{-1}v)Av]+\E[p^{\top}(x+\eps A^{-1}v)Av\right]\right)\\
&=\frac{1}{2r}\left(A\E[vv^{\top}]A^{-1}(Q+Q^{\top})x\right)+\frac{1}{r}\left(A\E[vv^{\top}]A^{-1}p\right)\\
&=\frac{1}{2}(Q+Q^{\top})x+p\\
&=\nabla q(x).
\end{align*}
Then since $\forall t\notin S_{\alpha}$,
\begin{align*}
\E[\tilde{g}_t\mid \F_{t-H}]&=\E\left[\frac{d}{\delta}f_t(y_{m(t)}) \sum_{s=t-H+1}^{t}A_{s}^{\frac{1}{2}}u_{s}\mid \F_{t-H}\right]\\
&=\E\left[\frac{d}{\delta}f_t(y_{m(t)}) \sum_{s\in m(t)}A_{s}^{\frac{1}{2}}u_{s}\mid \F_{t-H}\right],
\end{align*}
where $u_{m(t)}\in\mathbb{R}^{d|m(t)|}$ is sampled from a centered distribution and $\E\left[u_{m(t)}u_{m(t)}^{\top}\right]=\frac{1}{d}I_{d|m(t)|\times d|m(t)|}$. Enumerate $m(t)=\{s_1,\dots, s_{|m(t)|}\}$, and denote
\begin{align*}
\mathrm{diag}(\{A_s^{\frac{1}{2}}\}_{{s\in m(t)}})&=\begin{bmatrix}
A_{s_1}^{\frac{1}{2}} & 0_{d\times d} & \dots & \dots & 0_{d\times d} \\
0_{d\times d} & A_{s_2}^{\frac{1}{2}}& \dots & \dots & 0_{d\times d} \\
& & \dots & &\\
0_{d\times d} & 0_{d\times d} & \dots & \dots & A_{s_{|m(t)|}}^{\frac{1}{2}}
\end{bmatrix}\in \mathbb{R}^{d|m(t)|\times d|m(t)|}.
\end{align*}

By above, we have
\begin{align*}
\E\left[\frac{d}{\delta}f_t(y_{m(t)})\mathrm{diag}(\{A_s^{\frac{1}{2}}\}_{_{s\in m(t)}})u_{m(t)}\mid \F_{t-H}\right]=\nabla f_t(x_{m(t)}). 
\end{align*}
Thus, by definition of $\tilde{g}_{t}$, we have that
\begin{align*}
\E[\tilde{g}_{t}\mid \F_{t-H}]=\sum_{i\in [|m(t)|]}[\nabla f_t(x_{m(t)})]_i. 
\end{align*}
\end{proof}

Note that the unary form of $f_t$ over $\mathbb{R}^d$ admits the following expression:
\begin{align*}
\bar{f}_t(x)=\frac{1}{2}x^{\top}\left(\sum_{i,j\in [|m(t)|]}H_{t}^{ij}\right)x+\left(\sum_{i\in[|m(t)|]}b_{t}^{i}\right)^{\top}x+c_t.
\end{align*}
Thus, the gradient of $\bar{f}_t$ equals
\begin{align*}
\nabla \bar{f}_t(x)= \left(\sum_{i,j\in [|m(t)|]}H_{t}^{ij}\right)x+\sum_{i\in[|m(t)|]}b_{t}^{i}=\sum_{i\in [|m(t)|]}[\nabla f_t(x,\dots,x)]_i.
\end{align*}

Therefore, the gradient estimation bias on the complement of $S_{\alpha}$ is bounded by
\begin{align*}
\sum_{t\notin S_{\alpha}} \E[(\nabla \bar{f}_t(x_t)-\E[\tilde{g}_t\mid \F_{t-H}])^{\top}(x_t-x)]&\le D\sum_{t\notin S_{\alpha}}\E\left[\left\|\sum_{i\in [|m(t)|]}(\nabla f_t(x_t,\dots,x_t))_i-[\nabla f_t(x_{m(t)})]_i\right\|_2\right]\\
&\le D\sqrt{|m(t)|} \sum_{t\notin S_{\alpha}}\E\left[\left\|\nabla f_t(x_t,\dots,x_t)-\nabla f_t(x_{m(t)})\right\|_2\right]\\
&\le \beta D\sqrt{N}\sum_{t\notin S_{\alpha}}\sum_{s\in m(t)}\|x_t-x_s\|_2\\
&\le \beta D\sqrt{N}\sum_{t\notin S_{\alpha}}\sum_{s\in m(t)} \frac{4\eta dBH(t-s)}{\lambda\delta}\\
&\le \frac{4\eta D\beta dBN^{\frac{3}{2}}MHT}{\lambda\delta}. 
\end{align*}
We need to bound the gradient bias on $S_{\alpha}$. Fix $t\in S_{\alpha}$. Consider the sets $m_1(t)=[t-H+1, t]\cap m(t)$ and $m_0(t)=m(t)\setminus m_1(t)$. First, suppose $m_1(t)=\emptyset$, then $\E[\tilde{g}_t\mid \F_{t-H}]=0$. Thus, from now on assume $m_1(t)\ne \emptyset$. We denote $x_{m(t)}=[x_{m_0(t)}, x_{m_1(t)}]$. Let $f_t(x_{m(t)})=x_{m(t)}^{\top} H_t x_{m(t)}+b_t^{\top}x_{m(t)}+c$, write 
\begin{align*}
H_t=\begin{bmatrix}
H_t^{00}, H_t^{01}\\
H_t^{10}, H_t^{11}
\end{bmatrix}\in\mathbb{R}^{d|m(t)|\times d|m(t)|}, \ \ \ b_t = [b_{m_0(t)}, b_{m_1(t)}]\in\mathbb{R}^{d|m(t)|},
\end{align*}
where $H_t^{00}\in\mathbb{R}^{d|m_0(t)|\times d|m_0(t)|}$, $H_t^{01}\in\mathbb{R}^{d|m_0(t)|\times d|m_1(t)|}$, $H_t^{10}\in\mathbb{R}^{d|m_1(t)|\times d|m_0(t)|}$, $H_t^{11}\in\mathbb{R}^{d|m_1(t)|\times d|m_1(t)|}$, $b_{m_0(t)}\in\mathbb{R}^{d|m_0(t)|}$, $b_{m_1(t)}\in\mathbb{R}^{d|m_1(t)|}$. 
Note that we can decompose the conditional expectation of the gradient estimator as
\begin{align*}
\E[\tilde{g}_t\mid \F_{t-H}]&= \frac{d}{\delta}\E\left[[y_{m_0(t)}, y_{m_1(t)}]^{\top} \begin{bmatrix}
H_t^{00}, H_t^{01}\\
H_t^{10}, H_t^{11}
\end{bmatrix}\begin{bmatrix}
y_{m_0(t)}\\
y_{m_1(t)}
\end{bmatrix}
\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]\\
& \ \ \ \ \ +\frac{d}{\delta} \E\left[[b_{m_0(t)}, b_{m_1(t)}]^{\top}[y_{m_0(t)}, y_{m_1(t)}]\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]\\
&=\frac{d}{\delta} \E\left[y_{m_0(t)}^{\top}H_t^{00}y_{m_0(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]+\frac{d}{\delta} \E\left[y_{m_0(t)}^{\top}H_t^{01}y_{m_1(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]\\
& \ \ \ \ \  + \frac{d}{\delta} \E\left[y_{m_1(t)}^{\top}H_t^{10}y_{m_0(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]+ \frac{d}{\delta} \E\left[y_{m_1(t)}^{\top}H_t^{11}y_{m_1(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]\\
& \ \ \ \ \ +\frac{d}{\delta} \E\left[b_{m_0(t)}^{\top}y_{m_0(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]+\frac{d}{\delta} \E\left[b_{m_1(t)}^{\top}y_{m_1(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right].
\end{align*}
Denote $(X)_i$ as the $i$-th row vector of a matrix $X$. For each of the terms, we have 
\begin{align*}
\frac{d}{\delta} \E\left[y_{m_0(t)}^{\top}H_t^{00}y_{m_0(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]&=\frac{d}{\delta}y_{m_0(t)}^{\top}H_t^{00}y_{m_0(t)} \sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}\E\left[u_s\mid \F_{t-H}\right]=0.
\end{align*}
\begin{align*}
\frac{d}{\delta} \E\left[y_{m_0(t)}^{\top}H_t^{01}y_{m_1(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]&=\frac{d}{\delta} \E\left[y_{m_0(t)}^{\top}H_t^{01}x_{m_1(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]\\
& \ \ \ \ \ + d\E\left[y_{m_0(t)}^{\top}H_t^{01}A_{m_1(t)}^{-\frac{1}{2}}u_{m_1(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]\\
&=d\E\left[\left(\sum_{s\in m_1(t)} A_{s}^{\frac{1}{2}}u_s\right)\left(\sum_{s\in m_1(t)}(y_{m_0(t)}^{\top} H_t^{01})_s A_s^{-\frac{1}{2}}u_s\right)\mid \F_{t-H}\right]\\
&=d\sum_{s\in m_1(t)} A_{s}^{\frac{1}{2}}\E[u_su_s^{\top}]A_s^{-\frac{1}{2}}((H_t^{01})^{\top}y_{m_0(t)})_s\\
&=\sum_{s\in m_1(t)}((H_t^{01})^{\top}y_{m_0(t)})_s.
\end{align*}
Similarly, we can bound the other cross term in the quadratic term by
\begin{align*}
\frac{d}{\delta} \E\left[y_{m_1(t)}^{\top}H_t^{10}y_{m_0(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]&=\frac{d}{\delta}\E\left[y_{m_0(t)}^{\top}(H_t^{10})^{\top}A_{m_1(t)}^{-\frac{1}{2}}u_{m_1(t)}\sum_{s\in m_1(t)}A_s^{\frac{1}{2}}u_s\mid \F_{t-H}\right]\\
&=\sum_{s\in m_1(t)}(H_t^{10}y_{m_0(t)})_s,
\end{align*}
and 
\begin{align*}
\frac{d}{\delta} \E\left[y_{m_1(t)}^{\top}H_t^{11}y_{m_1(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]&=\frac{d}{\delta} \E\left[y_{m_1(t)}^{\top}H_t^{11}y_{m_1(t)}\sum_{s\in m_1(t)} A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]\\
&=d\E\left[x_{m_1(t)}^{\top}(H_t^{11}+(H_t^{11})^{\top})A_{m_1(t)}^{-\frac{1}{2}}u_{m_1(t)}\mid \sum_{s\in m_1(t)} \F_{t-H}\right]\\
&=\sum_{s\in m_1(t)}((H_t^{11}+(H_t^{11})^{\top})x_{m_1(t)})_s.
\end{align*}
The linear terms are bounded similarly.
\begin{align*}
\frac{d}{\delta} \E\left[b_{m_0(t)}^{\top}y_{m_0(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]&=0,\\
\frac{d}{\delta} \E\left[b_{m_1(t)}^{\top}y_{m_1(t)}\sum_{s=t-H+1}^t A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]&=d\E\left[b_{m_1(t)}^{\top}A_{m_1(t)}^{-\frac{1}{2}}u_{m_1(t)}\sum_{s\in m_1(t)} A_{s}^{\frac{1}{2}}u_s\mid \F_{t-H}\right]\\
&=d\E\left[\left(\sum_{s\in m_1(t)}b_s^{\top} A_{s}^{-\frac{1}{2}}u_{s}\right)\left(\sum_{s\in m_1(t)}A_s^{\frac{1}{2}}u_s\right)\mid \F_{t-H}\right]\\
&=d\E\left[\sum_{s\in m_1(t)}A_{s}^{\frac{1}{2}}u_su_s^{\top}A_s^{-\frac{1}{2}}b_s\mid \F_{t-H}\right]\\
&=d\sum_{s\in m_1(t)}A_s^{\frac{1}{2}}\E[u_su_s^{\top}] A_s^{-\frac{1}{2}}b_s\\
&=\sum_{s\in m_1(t)}b_s. 
\end{align*}
Combining above, we have the following expression for the $\ell_2$-norm of the conditional expectation of the gradient estimator:
\begin{align*}
\|\E[\tilde{g}_t\mid \F_{t-H}]\|_2&=
 \left\|\sum_{s\in m_1(t)} ((H_t^{11}+(H_t^{11})^{\top})x_{m_1(t)})_s +((H_{t}^{10}+(H_t^{01})^{\top})y_{m_0(t)})_s+\sum_{s\in m_1(t)}b_s\right\|_2\\
&\le \left\|\sum_{s\in m_1(t)}((H_t^{11}+(H_t^{11})^{\top})x_{m_1(t)})_s\right\|_2 +\left\|\sum_{s\in m_1(t)}((H_{t}^{10}+(H_t^{01})^{\top})y_{m_0(t)})_s\right\|_2+\left\|\sum_{s\in m_1(t)}b_s\right\|_2.
\end{align*}

By assumption, $H_t\preceq \beta I$, and thus $\max_{ij}|(H_t)_{ij}|\le \|H_t\|_2\le \beta$, and $H_{t}^{11}\preceq\beta I_{d|m_1(t)|\times d|m_1(t)|}$. The first and second term are thus bounded by
\begin{align*}
 \left\|\sum_{s\in m_1(t)}((H_t^{11}+(H_t^{11})^{\top})x_{m_1(t)})_s\right\|_2\le 2\beta |m_1(t)| \|x_{m_1(t)}\|_2\le 2\beta |m_1(t)|\sqrt{|m_1(t)|}D\le 2\beta DN^{\frac{3}{2}}.
\end{align*}

\begin{align*}
\left\|\sum_{s\in m_1(t)}((H_t^{01})^{\top}y_{m_0(t)})_s+(H_t^{10}y_{m_0(t)})_s\right\|_2
&\le 2 |m_1(t)|\sqrt{|m_1(t)|}\beta \|y_{m_0(t)}\|_1\\
&\le  2 |m_1(t)|\sqrt{|m_1(t)|}\beta \sqrt{d|m_0(t)|}\|y_{m_0(t)}\|_2\\
&\le 2 |m_1(t)|\sqrt{|m_1(t)|}\beta \sqrt{d|m_0(t)|}D\sqrt{|m_0(t)|}\\
&\le 2\beta\sqrt{d}DN^{\frac{5}{2}}. 
\end{align*}
To bound the second term, note that
\begin{align*}
G\ge \sup_{x\in\K^{|m(t)|}}\|H_tx+b_t\|_2\ge \|b_t\|_2-\sup_{x\in\K^{|m(t)|}} \|H_tx\|_2 \ge \|b_t\|_2-\beta D\sqrt{|m(t)|}\ge \|b_t\|_2-\beta D\sqrt{N}.
\end{align*}
Thus, $\|b_t\|_2\le G+\beta D\sqrt{N}$, and
\begin{align*}
\left\|\sum_{s\in m_1(t)}b_s\right\|_2&\le |m_1(t)|(G+\beta D\sqrt{N})\le (G+\beta D\sqrt{N})N.
\end{align*}
Putting together, we have that
\begin{align*}
\|\E[\tilde{g}_t\mid \F_{t-H}]\|_2\le 2\beta DN^{\frac{3}{2}}+2\beta\sqrt{d}DN^{\frac{5}{2}}+(G+\beta D\sqrt{N})N. 
\end{align*}
Thus, the gradient bias term over $S_{\alpha}$ can be bounded by
\begin{align*}
\sum_{t\in S_{\alpha}}\E[(\nabla \bar{f}_t(x_t)-\E[\tilde{g}_t\mid \F_{t-H}])^{\top}(x_t-x)]&\le D\sum_{t\in S_{\alpha}}\E[\|\nabla \bar{f}_t(x_t)-\E[\tilde{g}_t\mid \F_{t-H}]\|_2]\\
&\le D|S_{\alpha}|(G\sqrt{N}+2\beta DN^{\frac{3}{2}}+2\beta\sqrt{d}DN^{\frac{5}{2}}+(G+\beta D\sqrt{N})N)\\
&\le D|S_{\alpha}|(2GN+5\beta\sqrt{d}DN^{\frac{5}{2}}). 
\end{align*}
Putting together, we have that the underlying regret term is bounded by
\begin{align*}
\sum_{t=1}^T \E[\bar{f}_t(x_t)-\bar{f}_t(x)] & \le \frac{8\eta d^2B^2H^3T}{\delta^2}+\frac{\nu\log T}{\eta}+\frac{4\eta D\beta dBNMHT}{\lambda \delta}+D|S_{\alpha}|(2GN+5\beta\sqrt{d}DN^{\frac{5}{2}}). 
\end{align*}
The total regret of Algorithm~\ref{alg:bqo-memory-first-order} is bounded by
\begin{align*}
\max_{x\in\K}\E[\regret_T(x)]&\le \frac{\delta^2\beta NT}{2\lambda}+\frac{4\eta D\beta dBN^{\frac{3}{2}}MHT}{\lambda\delta}+ \frac{8\eta d^2B^2H^3T}{\delta^2}+\frac{\nu\log T}{\eta}+\frac{4\eta D\beta dBNMHT}{\lambda \delta}\\
& \ \ \ \ \ +D|S_{\alpha}|(2GN+5\beta\sqrt{d}DN^{\frac{5}{2}}).
\end{align*}
Choose $\alpha=\frac{1}{6}$, $\delta=T^{-\frac{1}{12}}$, $\eta=T^{-\frac{5}{6}}$, the expected regret is bounded by $\tilde{O}(T^{\frac{5}{6}})$. 

\begin{remark}
In the standard BCO with memory framework, we have the additional assumption that $\alpha=0$ and $S_0=\emptyset$. The above expected regret bound translates to the state-of-art bound $\tilde{O}(T^{\frac{2}{3}})$ by taking $\eta=T^{-\frac{2}{3}}$ and $\delta=T^{-\frac{1}{6}}$. 
\end{remark}

\begin{remark}
In the slightly more general setting, if we know in advance that $|S_{0}|= \tilde{O}(T^{\frac{2}{3}})$, then we can take $H=\poly \log(T)$ and have the expected regret bounded by $\tilde{O}(T^{\frac{2}{3}})$. 
\end{remark}

==> Backups/backup_second_order.tex <==
\subsubsection{BQO-M algorithm: second order}
\js{Conjecture: second-order algorithm allowing playing outside of the set should give a better bound than the first-order algorithm. So far, with tighter analysis can obtain same bound.}
\begin{algorithm}
\caption{Bandit Quadratic Optimization with Memory (\texttt{BQO-M})}\label{alg:bqo-memory}
\begin{flushleft}
  {\bf Input:} convex set $\K$, step size $\eta>0$, perturbation parameter $\delta\in[0,1]$. 
\end{flushleft}
\begin{algorithmic}[1]
\STATE Initialize: $x_{1}=\dots=x_{m}\in\K$, $\tilde{g}_{0:m-1} = \mathbf{0}_{d}$, $\tilde{H}_{0:m-1}=\hat{H}_{0:m-1}=\mathbf{0}_{d\times d}$, $ \tilde{A}_{-(m-1):m-1} =\hat{A}_{-(m-1):m-1} = mI$.
\STATE Sample $v_{t,1}, v_{t,2}\sim S^{d-1}$ i.i.d. uniformly at random for $t=1,\dots,m$. 
\STATE Set $y_t = x_t + \frac{\delta}{2}\tilde{A}_{t-m}^{-1/2}(v_{t,1}+v_{t,2})$, $t=1,\dots,m$. 
\FOR{$t = m, \ldots, T$}
\STATE Play $y_t$, observe $f_t(y_{t-m+1:t})$.
\STATE Create gradient and Hessian estimates:
\begin{align*}
\tilde{g}_{t}&=2\frac{d}{\delta}f_t(y_{t-m+1:t}) \sum_{j=0}^{m-1}\tilde{A}_{t-j-m}^{1/2}v_{t-j,1}\in\mathbb{R}^{d}, \\
\tilde{H}_{t}&=2\frac{d^2}{\delta^2}f_t(y_{t-m+1:t})\sum_{j=0}^{m-1}\tilde{A}_{t-j-m}^{1/2}(v_{t-j,1}v_{t-j,2}^{\top}+v_{t-j,2}v_{t-j,1}^{\top})\tilde{A}_{t-j-m}^{1/2}\in\mathbb{R}^{d\times d},\\ 
\hat{H}_{t}&=2\frac{d^2}{\delta^2}f_t(y_{t-m+1:t})\sum_{j,k=0}^{m-1}\tilde{A}_{t-j-m}^{1/2}(v_{t-j,1}v_{t-k,2}^{\top}+v_{t-k,2}v_{t-j,1}^{\top})\tilde{A}_{t-k-m}^{1/2}\in\mathbb{R}^{d\times d}.
\end{align*}
\STATE Update $\tilde{A}_{t} = \tilde{A}_{t-1} + \eta \tilde{H}_t $, $\hat{A}_{t}=\hat{A}_{t-1}+\eta\hat{H}_t$.
\STATE Update
$ x_{t+1} = \prod_{\K}^{\hat{A}_{t-m+1}} \left[ x_{t} - \eta \hat{A}_{t-m+1}^{-1}  \tilde{g}_{t-m+1}  \right]$.
\STATE Set $y_{t+1}=x_{t+1}+\frac{\delta}{2} \tilde{A}_{t-m+1}^{-1/2}(v_{t+1,1}+v_{t+1,2})$, $v_{t+1,1}, v_{t+1,2}\sim S^{d-1}$ i.i.d. uniformly at random. 
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsubsection{BQO-M analysis: second order}

\begin{lemma} [Unbiased estimators]
\label{lem:unbiased-estimators}
$\tilde{g}_{t}$ and $\tilde{H}_{t}$ are conditionally unbiased estimators of the following statistics: 
\begin{align*}
\E[\tilde{g}_{t}\mid \F_{t-m}]= \nabla\cdot f_t(x_{t-m+1:t}), \ \ \E[\tilde{H}_{t}\mid\F_{t-m}]=\sum_{i=1}^m(\nabla^2f_t)_{ii},
\ \   
\E[\hat{H}_{t}\mid\F_{t-m}] = \nabla^2 \bar{f}_{t},
\end{align*}
where $\F_t=\sigma(\{(v_{s,1},v_{s,2})\}_{s\le t})$ is the filtration generated by the algorithm's random sampling up to time $t$, and $(\nabla^2 f_t)_{ii}$ denote the $i$-th $d\times d$ diagonal block of $\nabla^2 f_t\in\mathbb{R}^{dm\times dm}$.
\end{lemma}
\begin{proof}
First, note that by design of Algorithm~\ref{alg:bqo-memory}, $y_t, \tilde{g}_t, \tilde{H}_t, \hat{H}_t, \tilde{A}_t, \hat{A}_t, \in\F_t$, $x_t\in\F_{t-m}$. Let $v_1,v_2$ be i.i.d. drawn from some symmetric distribution on $\mathbb{R}^d$ such that it satisfies that $\E[v_1v_1^{\top}]=r I$, and $\E[v_1v_2^{\top} Wv_1v_2^{\top}]=r^2W^{\top}$ for $W\in\mathbb{R}^{d\times d}$, $r>0$. Let $q:\mathbb{R}^d\rightarrow \mathbb{R}$ be a quadratic function. Then $\forall M\in\mathrm{Sym}(d)$ such that $M\succ 0$,
\begin{align}
\nabla q(x) &= \E_{v_1,v_2} \left[\frac{2}{r\delta}q\left(x+\frac{\delta}{2}M(v_1+v_2)\right)M^{-1}v_1\right], \label{equation:quadratic-grad}\\
\nabla^2 q &= \E_{v_1,v_2} \left[\frac{2}{r^2\delta^2}q\left(x+\frac{\delta}{2}M(v_1+v_2)\right) M^{-1}(v_1v_2^{\top}+v_2v_1^{\top})M^{-1}\right]. \label{equation:quadratic-hessian}
\end{align}
This can be checked by expanding $q(z)=\frac{1}{2}z^{\top}Az+b^{\top}z+c$ for some $A\in\mathbb{R}^{d\times d}, b\in\mathbb{R}^{d}, c\in\mathbb{R}$ and using the independence of $v_1, v_2$ and the fact that odd moments of $v_1, v_2$ are $0$. The details of the proof follows almost similarly to the proof of Proposition 1 in \cite{suggala2021efficient}. Consider the concatenated vector $v_{t-m+1:t,1}=(v_{t-m+1,1},\dots,v_{t,1})\in\mathbb{R}^{dm}$, where $v_{t-m+1,1},\dots, v_{t,1}$ are sampled i.i.d. from $S^{d-1}$. We show that $v_{t-m+1:t,1}, v_{t-m+1:t,2}$ satisfy that $\forall W\in\mathbb{R}^{dm\times dm}$,
\begin{align}
\label{equation:concated-distribution}
\E[v_{t-m+1:t,1}v_{t-m+1:t,1}^{\top}]=\frac{1}{d}I, \ \ \ \E[v_{t-m+1:t,1}v_{t-m+1:t,2}^{\top} W v_{t-m+1:t,1}v_{t-m+1:t,2}^{\top}]=\frac{1}{d^2}W^{\top}.
\end{align}
The first equality directly follows from independence and that $\E[vv^{\top}]=\frac{1}{d} I$ if $v$ is uniformly sampled from $S^{d-1}$. To see the second equality, first note that $\E[v_1v_2^{\top} U v_1v_2^{\top}]=\frac{1}{d^2}U^{\top}$, $\forall U\in\mathbb{R}^{d\times d}$, if $v_1,v_2$ are sampled i.i.d. uniformly from the unit sphere in $\mathbb{R}^{d}$. Let $W_{ij}$ denote the $(i,j)$-th $d\times d$ block of $W\in\mathbb{R}^{dm\times dm}$, i.e. $W_{ij}=W[(i-1)d+1:id, (j-1)d+1:jd]$. Then, $\forall W\in\mathbb{R}^{dm\times dm}$, 
\begin{align*}
&\E[v_{t-m+1:t,1}v_{t-m+1:t,2}^{\top} W v_{t-m+1:t,1}v_{t-m+1:t,2}^{\top}]\\
&=\E\left[\begin{bmatrix}
\sum_{j,k=t-m+1}^{t} v_{t-m+1,1}v_{k,2}^{\top}W_{k-t+m,j-t+m}v_{j,1}v_{t-m+1,2}^{\top}
& \dots & \sum_{j,k=t-m+1}^{t} v_{t-m+1,1}v_{k,2}^{\top}W_{k-t+m,j-t+m}v_{j,1}v_{t,2}^{\top} \\
\dots & \dots & \dots \\
\sum_{j,k=t-m+1}^{t} v_{t,1}v_{k,2}^{\top} W_{k-t+m,j-t+m}v_{j,1}v_{t-m+1,2}^{\top} & \dots & \sum_{j,k=t-m+1}^{t}v_{t,1}v_{k,2}^{\top}W_{k-t+m,j-t+m}v_{j,1}v_{t,2}^{\top}\\
\end{bmatrix}\right] \\
&=_{(1)}\E\left[\begin{bmatrix}
v_{t-m+1,1}v_{t-m+1,2}^{\top}W_{11}v_{t-m+1,1}v_{t-m+1,2}^{\top}
& \dots & v_{t-m+1,1}v_{t,2}^{\top}W_{m1}v_{t-m+1,1}v_{t,2}^{\top} \\
\dots & \dots & \dots \\
v_{t,1}v_{t-m+1,2}^{\top} W_{1m}v_{t,1}v_{t-m+1,2}^{\top} & \dots & v_{t,1}v_{t,2}^{\top}W_{mm}v_{t,1}v_{t,2}^{\top}\\
\end{bmatrix}\right] \\
&=\frac{1}{d^2} \begin{bmatrix}
W_{11}^{\top} & \dots & W_{m1}^{\top} \\
\dots & \dots & \dots \\
W_{1m}^{\top} & \dots & W_{mm}^{\top}
\end{bmatrix}
=\frac{1}{d^2} W^{\top},
\end{align*}
where (1) follows from independence of $\{v_{s,1}, v_{s,2}\}_{s=t-m+1}^t$ and that $\E[v_{s,1}]=\E[v_{s,2}]=0$. 

Let $\tilde{M}_t=\mathrm{diag}(\tilde{A}_{t-2m+1},\dots, \tilde{A}_{t-m})$. Recall that $y_{t-m+1:t}=x_{t-m+1:t}+\frac{\delta}{2}\tilde{M}_{t}^{-\frac{1}{2}}(v_{t-m+1:t,1}+v_{t-m+1:t,2})$. By Eq.(\ref{equation:quadratic-grad}-\ref{equation:concated-distribution}), we have that
\begin{align*}
\nabla f_t(x_{t-m+1:t}) &= \E[2d\delta^{-1}f_t(y_{t-m+1:t})\tilde{M}_t^{\frac{1}{2}}v_{t-m+1:t,1}\mid\F_{t-m}], \\
\nabla^2 f_t &= \E[2d^2\delta^{-2}f_t(y_{t-m+1:t})\tilde{M}_t^{\frac{1}{2}}(v_{t-m+1:t,1}v_{t-m+1:t,2}^{\top}+v_{t-m+1:t,2}v_{t-m+1:t,1}^{\top})\tilde{M}_t^{\frac{1}{2}}\mid\F_{t-m}]. 
\end{align*}
Then $\E[\tilde{g}_t\mid \F_{t-m}]=\nabla\cdot f_t(x_{t-m+1:t})$ by definition. To see that $\E[\hat{H}_{t}\mid \F_{t-m}]=\nabla^2\bar{f}_{t}$ and $\E[\tilde{H}_{t}\mid\F_{t-m}]=\sum_{i=1}^m (\nabla^2 f_t)_{ii}$, note that by expanding the matrix product in the unbiased estimator of $\nabla^2 f_t$ derived above, we have
\begin{align*}
& \ \ \ \ \ \tilde{M}_t^{\frac{1}{2}}(v_{t-m+1:t,1}v_{t-m+1:t,2}^{\top}+v_{t-m+1:t,2}v_{t-m+1:t,1}^{\top})\tilde{M}_t^{\frac{1}{2}}\\
&=\begin{bmatrix}
\tilde{A}_{t-2m+1}^{\frac{1}{2}}(v_{t-m+1,1}v_{t-m+1,2}^{\top}+v_{t-m+1,2}v_{t-m+1,1}^{\top})\tilde{A}_{t-2m+1}^{\frac{1}{2}} & \dots & \tilde{A}_{t-2m+1}^{\frac{1}{2}}(v_{t-m+1,1}v_{t,2}^{\top}+v_{t,2}v_{t-m+1,1}^{\top})\tilde{A}_{t-m}^{\frac{1}{2}} \\
\dots & \dots & \dots \\
\tilde{A}_{t-m}^{\frac{1}{2}}(v_{t,1}v_{t-m+1,2}^{\top}+v_{t-m+1,2}v_{t,1}^{\top})\tilde{A}_{t-2m+1}^{\frac{1}{2}} & \dots & \tilde{A}_{t-m}^{\frac{1}{2}}(v_{t,1}v_{t,2}^{\top}+v_{t,2}v_{t,1}^{\top})\tilde{A}_{t-m}^{\frac{1}{2}},
\end{bmatrix}
\end{align*}
and thus using the observation that $\nabla^2 \bar{f}_{t}=\sum_{i,j=1}^m (\nabla^2 f_t)_{ij}$, where $(\nabla^2 f_t)_{ij}$ denotes the $(i,j)$-th $d\times d$ block of $\nabla^2 f_t$, we have
\begin{align*}
\nabla^2 \bar{f}_{t}&=\E[2d^2\delta^{-2}f_t(y_{t-m+1:t})\sum_{j,k=0}^{m-1}\tilde{A}_{t-j-m}^{\frac{1}{2}}(v_{t-j,1}v_{t-k,2}^{\top}+v_{t-k,2}v_{t-j,1}^{\top})\tilde{A}_{t-k-m}^{\frac{1}{2}}\mid \F_{t-m}]\\
&=\E[\hat{H}_{t}\mid\F_{t-m}],\\
\sum_{i=1}^m(\nabla^2 f_t)_{ii}&=\E[2d^2\delta^{-2}f_t(y_{t-m+1:t})\sum_{j=0}^{m-1}\tilde{A}_{t-j-m}^{\frac{1}{2}}(v_{t-j,1}v_{t-j,2}^{\top}+v_{t-j,2}v_{t-j,1}^{\top})\tilde{A}_{t-j-m}^{-\frac{1}{2}}\mid\F_{t-m}]\\
&=\E[\tilde{H}_{t}\mid\F_{t-m}].
\end{align*}
\end{proof}

Lemma~\ref{lem:concentration-with-memory} shows that the constructed preconditioners $\tilde{A}_{t}, \hat{A}_{t}$ concentrate well. 

\begin{lemma} [Concentration of Hessian estimator, with-memory case] 
\label{lem:concentration-with-memory}
Let 
\begin{align*}
\bar{A}_{t}=\eta \sum_{s=m}^t \nabla^2 \bar{f}_{s}+mI, \ \ \
A_t=\eta\sum_{s=m}^t \left(\sum_{i=1}^m(\nabla^2f_t)_{ii}\right)+mI.
\end{align*}
Assume that $\eta \le \left(8 \left(\beta+\frac{6d^2}{\delta^2}(B+\delta\sqrt{2m}(G+\delta\sqrt{2m}\beta))\right)m^2\sqrt{T\log 2dmT^2}\right)^{-1}$. Then $\forall t$, with probability at least $1-\frac{t}{T^2}$, 
\begin{align*}
\|I-\bar{A}_{s}^{-\frac{1}{2}}\hat{A}_s\bar{A}_{s}^{-\frac{1}{2}}\|_2\le \frac{1}{2}, \ \ \|I-A_{s}^{-\frac{1}{2}}\tilde{A}_sA_{s}^{-\frac{1}{2}}\|_2\le \frac{1}{2}, \ \ \forall s\le t.
\end{align*}
\end{lemma}
\begin{proof}
The proof follows similarly to the no-memory case. $\forall 0\le i\le m-1$, denote $C(i)=\{t\in[T]: t\equiv i \ \mathrm{mod} \ m\}$.

\paragraph{Base case.} For $0\le t\le m-1$, the inequality holds trivially since by algorithm definition, $\tilde{A}_{0:m-1}=\hat{A}_{0:m-1}=mI=\bar{A}_{0:m-1}=A_{0:m-1}$. 


\paragraph{Induction hypothesis.} Assume for some $t\ge m$, with probability at least $1-\frac{t-1}{T^2}$, $\|I-\bar{A}_{s}^{-\frac{1}{2}}\hat{A}_s\bar{A}_{s}^{-\frac{1}{2}}\|_2\le\frac{1}{2}$ and $\|I-A_{s}^{-\frac{1}{2}}\tilde{A}_sA_{s}^{-\frac{1}{2}}\|_2\le\frac{1}{2}$ hold $\forall s\le t-1$. 
We show that with probability at least $1-\frac{t}{T^2}$, the two inequalities hold for all $s\le t$.

\paragraph{Induction.} First, assume that $\|I-\bar{A}_{s}^{-\frac{1}{2}}\hat{A}_s\bar{A}_{s}^{-\frac{1}{2}}\|_2\le\frac{1}{2}$ and $\|I-A_{s}^{-\frac{1}{2}}\tilde{A}_sA_{s}^{-\frac{1}{2}}\|_2\le\frac{1}{2}$ hold $\forall s\le t-1$. Under the assumption that $f_t$ is $\beta$-smooth, $G$-Lipschitz on $\K^m$ and $|f_t|\le B$ on $\K^m$, we can bound the loss values of the $y_t$'s actually played by
\begin{align*}
|f_t(y_{t-m+1:t})|&\le |f_t(x_{t-m+1:t})|+\|\nabla f_t(y_{t-m+1:t})\|_2\|y_{t-m+1:t}-x_{t-m+1:t}\|_2\\
&\le B+(G+\beta\|y_{t-m+1:t}-x_{t-m+1:t}\|_2)\|y_{t-m+1:t}-x_{t-m+1:t}\|_2,
\end{align*}
where 
\begin{align*}
\|y_{t-m+1:t}-x_{t-m+1:t}\|_2 =\left\|\frac{\delta}{2}\tilde{A}_{t-2m+1:t-m}^{-\frac{1}{2}}(v_{t-m+1:t,1}+v_{t-m+1:t,2})\right\|_2\le \delta\sum_{s=t-2m+1}^{t-m}\|\tilde{A}_{s}^{-\frac{1}{2}}\|_2\le \delta\sqrt{2m},
\end{align*}
where the last inequality follows the assumption $\tilde{A}_s\succeq \frac{1}{2}A_{s}\succeq \frac{m}{2}I$, $\forall s\le t-1$. Therefore, $|f_t(y_{t-m+1:t})|\le B+\delta\sqrt{2m}(G+\delta\sqrt{2m}\beta )=B^*$. 

With the bound on $|f_t(y_{t-m+1:t})|$, we are one step closer to bound the two quantities. Notice that the two quantities are the sum of $m$ martingale sums, allowing the following representations: 
\begin{align*}
I-\bar{A}_{t}^{-\frac{1}{2}}\hat{A}_t\bar{A}_{t}^{-\frac{1}{2}}&=\eta\sum_{i=0}^{m-1}\sum_{s\in C(i), s\le t} Z_s, \ \ Z_s=\bar{A}_{t}^{-\frac{1}{2}}(\nabla^2\bar{f}_{s}-\hat{H}_{s})\bar{A}_{t}^{-\frac{1}{2}},\\
I-A_{t}^{-\frac{1}{2}}\tilde{A}_tA_{t}^{-\frac{1}{2}}&=\eta\sum_{i=0}^{m-1}\sum_{s\in C(i), s\le t}Y_s, \ \ Y_s=A_t^{-\frac{1}{2}}\left(\sum_{i=1}^m(\nabla^2 f_t)_{ii}-\tilde{H}_{s}\right)A_t^{-\frac{1}{2}},
\end{align*}
where $\E[Z_s\mid \F_{s-m}]=\E[Y_s\mid \F_{s-m}]=0$, and therefore $\sum_{s\in C(i), s\le t}Z_s$ is a martingale sum for all $i$. 
First, note that for any $u,v\in S^{d-1}$, $-2I\preceq -uu^{\top}-vv^{\top}\preceq uv^{\top}+vu^{\top}\preceq uu^{\top}+vv^{\top}\preceq 2I$. Thus, $Z_s$ and $Y_s$ can be bounded as following: 
\begin{align*}
Z_s&\in \left[-\bar{A}_{t}^{-\frac{1}{2}}\hat{H}_{s}\bar{A}_{t}^{-\frac{1}{2}}, \ \bar{A}_{t}^{-\frac{1}{2}}(m^2\beta I-\hat{H}_{s})\bar{A}_{t}^{-\frac{1}{2}}\right]\\
&\subseteq \left[-\bar{A}_{t}^{-\frac{1}{2}}\left(\frac{4d^2}{\delta^2}B^*\sum_{j,k=0}^{m-1}\tilde{A}_{s-j-m}^{\frac{1}{2}}\tilde{A}_{s-k-m}^{\frac{1}{2}}\right)\bar{A}_{t}^{-\frac{1}{2}}, \ \bar{A}_{t}^{-\frac{1}{2}}\left(m^2\beta I+\frac{4d^2}{\delta^2}B^*\sum_{j,k=0}^{m-1}\tilde{A}_{s-j-m}^{\frac{1}{2}}\tilde{A}_{s-k-m}^{\frac{1}{2}}\right)\bar{A}_{t}^{-\frac{1}{2}}\right]\\
&\subseteq \frac{4d^2}{\delta^2}B^*\left[-\sum_{j,k=0}^{m-1}(\bar{A}_{s-j-m}^{-\frac{1}{2}}\tilde{A}_{s-j-m}^{\frac{1}{2}})(\tilde{A}_{s-k-m}^{\frac{1}{2}}\bar{A}_{s-k-m}^{-\frac{1}{2}}), \  \frac{m^2\beta\delta^2}{4B^*d^2} I+  \sum_{j,k=0}^{m-1}(\bar{A}_{s-j-m}^{-\frac{1}{2}}\tilde{A}_{s-j-m}^{\frac{1}{2}})(\tilde{A}_{s-k-m}^{\frac{1}{2}}\bar{A}_{s-k-m}^{-\frac{1}{2}})\right]\\
&\subseteq \left[-\frac{6d^2}{\delta^2}B^*m^2 I, \ \left(\beta + \frac{6d^2}{\delta^2}B^*\right)m^2 I\right],
\end{align*}
and similarly $Y_s$ can be bounded by
\begin{align*}
Y_s&\in \left[-A_t^{-\frac{1}{2}}\tilde{H}_sA_{t}^{-\frac{1}{2}}, \ A_t^{-\frac{1}{2}}(m\beta I-\tilde{H}_s)A_{t}^{-\frac{1}{2}}\right]\\
&\subseteq \left[-A_t^{-\frac{1}{2}}\left(\frac{4d^2}{\delta^2}B^*m \sum_{j=0}^{m-1}\tilde{A}_{t-j-m}\right)A_{t}^{-\frac{1}{2}}, \ A_t^{-\frac{1}{2}}\left(m\beta I+\frac{4d^2}{\delta^2}B^*m \sum_{j=0}^{m-1}\tilde{A}_{t-j-m}\right)A_{t}^{-\frac{1}{2}}\right]\\
&\subseteq \left[-\frac{4d^2}{\delta^2} B^*m \sum_{j=0}^{m-1}A_{t-j-m}^{-\frac{1}{2}}\tilde{A}_{t-j-m}A_{t-j-m}^{-\frac{1}{2}}, \ m\beta I + \frac{4d^2}{\delta^2} B^*m \sum_{j=0}^{m-1}A_{t-j-m}^{-\frac{1}{2}}\tilde{A}_{t-j-m}A_{t-j-m}^{-\frac{1}{2}}\right]\\
&\subseteq \left[-\frac{6d^2}{\delta^2}B^*mI, \ \left(\beta+\frac{6d^2}{\delta^2}B^*\right)mI\right].
\end{align*}
Thus, $\|Z_s\|_2\le \left(\beta+\frac{6d^2}{\delta^2}B^*\right)m^2$, and $\|Y_s\|_2\le \left(\beta+\frac{6d^2}{\delta^2}B^*\right)m$. 

\begin{lemma} [Matrix Azuma, \cite{tropp2012user}]
\label{lem:matrix-azuma}
Consider a finite adapted sequence $\left\{X_k\right\}$ of self-adjoint matrices in dimension d, and a fixed sequence $\left\{A_k\right\}$ of self-adjoint matrices that satisfy
$$
\mathbb{E}_{k-1} X_k=0 \quad \text { and } \quad X_k^2 \preceq A_k^2 \quad \text { almost surely. }
$$
Compute the variance parameter
$$
\sigma^2:=\left\|\sum_k A_k^2\right\|.
$$
Then, for all $a \ge 0$,
$$
\mathbb{P}\left\{\lambda_{\max }\left(\sum_k X_k\right) \geq a\right\} \leq d \cdot e^{-a^2 / 8 \sigma^2}. 
$$
\end{lemma}

By Lemma~\ref{lem:matrix-azuma}, union bound, and choice of $\eta$, with probability at least $1-\frac{1}{T^2}$, the following two inequalities hold simultaneously:
\begin{align*}
\|I-\bar{A}_{t}^{-\frac{1}{2}}\hat{A}_t\bar{A}_{t}^{-\frac{1}{2}}\|_2&\le 4\eta \left(\beta+\frac{6d^2}{\delta^2}B^*\right)m^2\sqrt{T\log 2dmT^2}\le \frac{1}{2},\\
\|I-A_{t}^{-\frac{1}{2}}\tilde{A}_tA_{t}^{-\frac{1}{2}}\|_2&\le 4\eta \left(\beta+\frac{6d^2}{\delta^2}B^*\right)m\sqrt{T\log 2dmT^2}\le \frac{1}{2}.
\end{align*}
Therefore, induction hypothesis implies that
\begin{align*}
& \ \ \ \ \mathbb{P}\left(\|I-\bar{A}_{s}^{-\frac{1}{2}}\hat{A}_s\bar{A}_{s}^{-\frac{1}{2}}\|_2\vee \|I-A_{s}^{-\frac{1}{2}}\tilde{A}_sA_{s}^{-\frac{1}{2}}\|_2\le \frac{1}{2}, \forall s\le t\right)\\
&=\mathbb{P}\left(\|I-\bar{A}_{t}^{-\frac{1}{2}}\hat{A}_t\bar{A}_{t}^{-\frac{1}{2}}\|_2\vee \|I-A_{t}^{-\frac{1}{2}}\tilde{A}_tA_{t}^{-\frac{1}{2}}\|_2\le\frac{1}{2}\mid \|I-\bar{A}_{s}^{-\frac{1}{2}}\hat{A}_s\bar{A}_{s}^{-\frac{1}{2}}\|_2\vee \|I-A_{s}^{-\frac{1}{2}}\tilde{A}_sA_{s}^{-\frac{1}{2}}\|_2\le \frac{1}{2}, \forall s\le t-1\right)\\
& \ \ \ \ \ \mathbb{P}\left(\|I-A_{s}^{-\frac{1}{2}}\tilde{A}_sA_{s}^{-\frac{1}{2}}\|_2\vee \|I-A_{s}^{-\frac{1}{2}}\tilde{A}_sA_{s}^{-\frac{1}{2}}\|_2\le \frac{1}{2}, \forall s\le t-1\right)\\
&\ge\left(1-\frac{1}{T^2}\right)\left(1-\frac{t-1}{T^2}\right)\\
&\ge 1-\frac{t}{T^2}.
\end{align*}
\end{proof}

\begin{corollary} [Bounded exploration cost]  With probability at least $1-\frac{1}{T}$, $\forall y_t$ played by Algorithm~\ref{alg:bqo-memory}, $|f_t(y_{t-m+1:t})|\le B^*=B+\delta\sqrt{2m}(G+\delta\sqrt{2m}\beta)$. 
\end{corollary}
\begin{proof}
The proof is provided in the proof of Lemma~\ref{lem:concentration-with-memory}.
\end{proof}

\begin{remark} [Well-defined preconditioners] As an immediate implication of Lemma~\ref{lem:concentration-with-memory}, $\tilde{A}_{t}, \hat{A}_{t}\succ 0$ $\forall t$ holds with probability at least $1-\frac{1}{T}$ and thus the preconditioners in Algorithm~\ref{alg:bqo-memory} are well-defined. 
\end{remark}

\begin{theorem}
The regret can be decomposed as
\begin{align*}
\E[\regret_T(x)]=\underbrace{\sum_{t=m}^T \E[f_t(y_{t-m+1:t})-f_t(x_{t-m+1:t})]}_{(1: \text{exploration  loss})} + \underbrace{\sum_{t=m}^T \E[f_t(x_{t-m+1:t})-\bar{f}_{t}(x_t)]}_{(2: \text{movement loss})}+\underbrace{\sum_{t=m}^T\E[\bar{f}_{t}(x_t)-\bar{f}_{t}(x)]}_{(3: \text{ONS regret})},
\end{align*}
where with probability at least $1-\frac{1}{T}$,
\begin{align*}
(1)&\le C_8\frac{\delta^2}{\eta},\\
(2)&\le C_6\frac{\eta^3T^2}{\delta^2} +C_7\frac{\eta^2T}{\delta^2}, \\
(3)&\le C_1 \frac{\eta (1+\eta\beta T)T}{\delta^2}  +C_2\frac{\eta\sqrt{1+\eta\beta T}T}{\delta} + C_3\frac{\eta(\sqrt{\eta T}+1) T}{\delta} +C_4\frac{1}{\eta}+C_5,
\end{align*}
where 
\begin{align*}
C_1&=90d^2(B^*)^2m^6, \ C_2=(17d+16\beta )DB^* m^{\frac{5}{2}}, \ C_3=6dB^*Gm^{\frac{7}{2}}, C_4=mD^2,\\
C_5&=mB, \ C_6 = 16\beta^2d^2(B^*)^2m^4, \ C_7 = 16\beta d^2(B^*)^2m^4, \ C_8=d\log(\eta\beta mT+m).
\end{align*}
In particular, setting $\delta=1$ and $\eta=\tilde{\Theta}(T^{-\frac{2}{3}})$, the expected regret with respect to any $x\in\K$ is bounded by $\tilde{O}(T^{\frac{2}{3}})$. 
\end{theorem}
\begin{proof}
With probability at least $1-\frac{1}{T}$, $\|I-\bar{A}_{t}^{-\frac{1}{2}}\hat{A}_{t}\bar{A}_{t}^{-\frac{1}{2}}\|_2\le \frac{1}{2}$ and $\|I-A_t^{-\frac{1}{2}}\tilde{A}_{t}A_t^{-\frac{1}{2}}\|_2\le\frac{1}{2}$ hold for all $t$. We prove the bounds for (1), (2), and (3) under the assumption that these inequalities hold. We begin by stating some bounds on key quantities that we will be using frequently in the proof:

\begin{lemma}
\label{lem:useful-bounds}
The following bounds hold $\forall t$: assume $\eta\beta m\le 1$,
\begin{align}
\max\{\|\tilde{A}_{t}\|_2,\|\hat{A}_{t}\|_2\}&\le \frac{3}{2}m(1+\eta\beta t),\label{eqn:preconditioner-bound}\\
\max\{\|\tilde{A}_{t}^{-1}\|_2,\|\hat{A}_{t}^{-1}\|_2\}&\le \frac{2}{m},\label{eqn:inv-preconditioner-bound}\\
\|\tilde{g}_{t}\|_2&\le \frac{2\sqrt{2}dB^*m^\frac{3}{2}}{\delta}\sqrt{1+\eta\beta t}\label{eqn:grad-est-bound},\\
\frac{1}{6}\hat{A}_t &\preceq \hat{A}_{t-i}\preceq \frac{3}{2}\hat{A}_t, \ \forall 0\le i\le m-1\label{eqn:neighbor-preconditioner-bound}.
\end{align}
\end{lemma}
\begin{proof}
Eq.(\ref{eqn:preconditioner-bound}-\ref{eqn:inv-preconditioner-bound}) follows from the concentration assumption. We have that $mI\preceq A_t\preceq m(1+\eta\beta t)I$ and $mI\preceq \bar{A}_t\preceq m(1+\eta\beta t)I$ by construction. Thus,
\begin{align*}
\tilde{A}_{t}\preceq \frac{3}{2}A_t\preceq \frac{3}{2}m(1+\eta\beta t)I, \ \ \  
\tilde{A}_{t}^{-1}\preceq 2A_t^{-1}\preceq \frac{2}{m}I,
\end{align*}
and similarly for $\hat{A}_{t}$. By definition of $\tilde{g}_{t}$,
\begin{align*}
\|\tilde{g}_{t}\|_2&\le \frac{2dB^*}{\delta}\sum_{j=0}^{m-1}\|\tilde{A}_{t-j-m}^{\frac{1}{2}}\|_2\le \frac{2\sqrt{2}dB^*m}{\delta}\|A_{t-m}^{\frac{1}{2}}\|_2\le \frac{2\sqrt{2}dB^*m^\frac{3}{2}}{\delta}\sqrt{1+\eta\beta t}. 
\end{align*}
The second inequality in Eq.(\ref{eqn:neighbor-preconditioner-bound}) follows directly from $\hat{A}_{t-i}\preceq \frac{3}{2}\bar{A}_{t-i}\preceq\bar{A}_{t}$. To see the first inequality, it suffcies to show that $\frac{1}{2}\bar{A}_{t}\preceq \bar{A}_{t-i}$. 
\begin{align*}
\frac{1}{2}\bar{A}_{t}=\frac{1}{2}\bar{A}_{t-i}+\frac{\eta}{2} \sum_{s=t-i+1}^t \nabla^2 \bar{f}_{s}\preceq \frac{1}{2} \bar{A}_{t-i}+\frac{\eta \beta m^2}{2} I\preceq_{(a)} \bar{A}_{t-i}, 
\end{align*}
where $(a)$ follows since $\bar{A}_{t-i}\succeq mI$ and $\eta\beta m\le 1$. 
\end{proof}

\paragraph{Exploration perturbation loss.} First, we bound $(1)$. Let $u_t=\frac{1}{2}(v_{t,1}+v_{t,2})$. $y_t=x_t+\delta\tilde{A}_{t-m}^{-\frac{1}{2}}u_t$. 
\begin{align*}
(1)&=\sum_{t=m}^T \E\left[\nabla f_t(x_{t-m+1:t})^{\top}(y_{t-m+1:t}-x_{t-m+1:t})+\frac{1}{2}(y_{t-m+1:t}-x_{t-m+1:t})^{\top}H_t(y_{t-m+1:t}-x_{t-m+1:t})\right]\\
&=\sum_{t=m}^T\E\left[\delta\nabla f_t(x_{t-m+1:t})^{\top}\tilde{A}_{t-2m+1:t-m}^{-\frac{1}{2}}u_{t-m+1:t}+\frac{\delta^2}{2}u_{t-m+1:t}^{\top}\tilde{A}_{t-2m+1:t-m}^{-\frac{1}{2}}H_t\tilde{A}_{t-2m+1:t-m}^{-\frac{1}{2}}u_{t-m+1:t}\right]\\
&=\delta \sum_{t=m}^T \underbrace{\E[\E[\nabla f_t(x_{t-m+1:t})^{\top}\tilde{A}_{t-2m+1:t-m}^{-\frac{1}{2}}u_{t-m+1:t}\mid\F_{t-m}]]}_{=0} \\
& \ \ \ \ \ + \frac{\delta^2}{2}\sum_{t=m}^T \E[u_{t-m+1:t}^{\top}\tilde{A}_{t-2m+1:t-m}^{-\frac{1}{2}}H_t\tilde{A}_{t-2m+1:t-m}^{-\frac{1}{2}}u_{t-m+1:t}]\\
&=\frac{\delta^2}{2}\sum_{t=m}^T \sum_{j=1}^m \mathbb{E}[u_{t-m+j}^{\top} \tilde{A}_{t-2m+j}^{-\frac{1}{2}}(H_t)_{jj}\tilde{A}_{t-2m+j}^{-\frac{1}{2}}u_{t-m+j}]\\
&=\frac{\delta^2}{2}\sum_{t=m}^T \sum_{j=1}^m \trace(\tilde{A}_{t-2m+j}^{-\frac{1}{2}}(H_t)_{jj}\tilde{A}_{t-2m+j}^{-\frac{1}{2}})\\
&\le_{(a)} \delta^2\sum_{t=m}^T \sum_{j=1}^m \trace(A_{t}^{-\frac{1}{2}}(H_t)_{jj}A_t^{-\frac{1}{2}})\\
&=\delta^2\sum_{t=m}^T \trace\left(A_t^{-\frac{1}{2}}\sum_{j=1}^m (H_t)_{jj}A_t^{-\frac{1}{2}}\right)\\
&=\frac{\delta^2}{\eta} \sum_{t=m}^T \trace\left(A_t^{-\frac{1}{2}}(A_{t}-A_{t-1})A_t^{-\frac{1}{2}}\right)\\
&\le \frac{\delta^2}{\eta}\sum_{t=m}^T \log\left(\frac{|A_t|}{|A_{t-1}|}\right)\\
&\le \frac{\delta^2\log(|A_T|)}{\eta}\\
&\le \frac{\delta^2d\log(\eta\beta mT + m)}{\eta}\\
&=C_8\frac{\delta^2}{\eta},
\end{align*}
where (a) follows from that with probability at least $1-\frac{1}{T}$, $\tilde{A}_{t}\succeq \frac{1}{2}A_t$, $\forall t$, and $A_t\succeq A_s$, $\forall s<t$. 

\paragraph{Movement loss.} (2) depends on the iterate bound on $\|x_{t-1}-x_{t}\|_2^2$. Note that by Algorithm~\ref{alg:bqo-memory}, $x_1=\dots=x_{2m-2}$. For $t\ge 2m-1$, $\|x_{t-1}-x_t\|_2^2$ can be bounded as following: \textcolor{red}{ Working in $\|\cdot\|_2$ norm can give sub-optimal rates. A better approach would be to work in $\|\cdot\|_{\hat{A}_t}$ norm or its dual.} \js{yes, you are right. will try the new approach.}
\begin{align}
\|x_{t-1}-x_{t}\|_2^2&\le \|\eta \hat{A}_{t-m}^{-1}\tilde{g}_{t-m}\|_2^2 \le_{(b)} \frac{32\eta^2d^2(B^*)^2m}{\delta^2}(1+\eta\beta t), \label{eqn:iterate-bound}
\end{align}
where (b) follows from Lemma~\ref{lem:useful-bounds}. (2) can be thus bounded by
\begin{align*}
(2)&\le \frac{\beta}{2} \sum_{t=m}^T\|x_{t-m+1:t}-(x_t,\dots,x_t)\|_2^2\\&
=\frac{\beta}{2}\sum_{t=m}^T \sum_{s=t-m+1}^t \|x_s-x_t\|_2^2\\
&\le\frac{\beta}{2}\sum_{t=m}^T \sum_{s=t-m+1}^t (t-s)\sum_{r=s+1}^t\|x_r-x_{r-1}\|_2^2\\
&\le \frac{16\beta d^2\eta^2(B^*)^2m}{\delta^2} \sum_{t=m}^T \sum_{s=t-m+1}^t (t-s)^2(1+\eta \beta t)\\
&\le \frac{16\beta d^2\eta^2(B^*)^2m^4}{\delta^2}\sum_{t=m}^T 1+\eta \beta t\\
&\le \frac{16\beta^2 d^2\eta^3(B^*)^2m^4T^2}{\delta^2} +\frac{16\beta d^2\eta^2(B^*)^2 m^4T}{\delta^2}\\
&= C_6\frac{\eta^3T^2}{\delta^2} +C_7\frac{\eta^2T}{\delta^2}.
\end{align*}

\paragraph{ONS regret.} To bound the third term, first we bound the conditional bias of $\tilde{g}_{t}$ as an estimator of $\nabla\bar{f}_{t}(x_t)$:
\begin{align}
\|\E[\tilde{g}_{t}\mid\F_{t-m}]-\nabla \bar{f}_{t}(x_{t+m-1})\|_2&=_{(d)}\|\nabla\cdot f_t(x_{t-m+1:t})-\nabla\bar{f}_{t}(x_{t+m-1})\|_2\\
&\le_{(e)} \sqrt{m}\|\nabla f_t(x_{t-m+1:t}) - \nabla f_t(x_{t+m-1},\dots,x_{t+m-1})\|_2\\
&\le \sqrt{m}\beta \|x_{t-m+1:t}-(x_{t+m-1},\dots,x_{t+m-1})\|_2\\
&\le_{(f)} \frac{8\eta B^*dm^{\frac{5}{2}}\beta\sqrt{1+\eta\beta t}}{\delta} \label{eqn:grad-bias-bound},
\end{align}
where (d) follows from Lemma~\ref{lem:unbiased-estimators}; (e) follows from the fact that $\forall a,b\in\mathbb{R}^n$, $\|\sum_{i=1}^n a_i-b_i\|_2\le \sqrt{n} \|a-b\|_2$, and $\nabla \bar{f}_t(x)=\sum_{i=1}^m \nabla_i f_t(x,\dots,x)$; (f) follows similarly as the bound on $\|x_{t-m+1:t}-(x_t,\dots,x_t)\|_2^2$ when bounding (2). 
By the projection step in Algorithm~\ref{alg:bqo-memory}, $\forall x\in\K$,
\begin{align*}
\E[\|x_t-x\|_{\hat{A}_{t-m}}^2]&\le \E[\|x_{t-1}-x-\eta \hat{A}_{t-m}^{-1}\tilde{g}_{t-m}\|_{\hat{A}_{t-m}}^2]\\
&=\underbrace{\E[\|x_{t-1}-x\|_{\hat{A}_{t-m}}^2]}_{(g)}-2\eta \underbrace{\E[\tilde{g}_{t-m}^{\top}(x_{t-1}-x)]}_{(h)}+\eta^2\underbrace{\E[\|\tilde{g}_{t-m}\|_{\hat{A}_{t-m}^{-1}}^2]}_{(i)},
\end{align*}
where $(g),(h),(i)$ can be further bounded by
\begin{align*}
(g)&=\E[\|x_{t-m}-x\|_{\hat{A}_{t-m}}^2]+\E[\|x_{t-1}-x_{t-m}\|_{\hat{A}_{t-m}}^2] + \E[(x_{t-m}-x)^{\top}\hat{A}_{t-m}(x_{t-1}-x_{t-m})]\\
&\le \E[\|x_{t-m}-x\|_{\hat{A}_{t-m-1}}^2] + \eta\E[\|x_{t-m}-x\|_{\E[\hat{H}_{t-m}\mid\F_{t-2m}]}^2] + m\sum_{s=t-m+1}^{t-1}\E[\|x_{s}-x_{s-1}\|_{\hat{A}_{t-m}}^2] \\
& \ \ \ \ \ +D\E[\|\hat{A}_{t-m}(x_{t-1}-x_{t-m})\|_2]\\
&\le \E[\|x_{t-m}-x\|_{\hat{A}_{t-m-1}}^2] + \eta\E[\|x_{t-m}-x\|_{\nabla^2\bar{f}_{t-m}}^2]+6\eta^2m\sum_{s=t-m+1}^{t-1}\E[\|\hat{A}_{s-m}^{-1}\tilde{g}_{s-m}\|_{\hat{A}_{s-m}}^2]\\
& \ \ \ \ \ + 6D\sum_{s=t-m+1}^{t-1}\E[\|\hat{A}_{s-m}(x_s-x_{s-1})\|_2]\\
& \le \E[\|x_{t-m}-x\|_{\hat{A}_{t-m-1}}^2] + \eta\E[\|x_{t-m}-x\|_{\nabla^2\bar{f}_{t-m}}^2]+6\eta^2m\sum_{s=t-m+1}^{t-1}\E[\|\tilde{g}_{s-m}\|_{\hat{A}_{s-m}^{-1}}^2]\\
& \ \ \ \ \ + 6\eta D\sum_{s=t-m+1}^{t-1}\E[\|\tilde{g}_{s-m}\|_2]\\
& \le \E[\|x_{t-m}-x\|_{\hat{A}_{t-m-1}}^2] + \eta\E[\|x_{t-m}-x\|_{\nabla^2\bar{f}_{t-m}}^2]+\frac{54\eta^2d^2(B^*)^2m^6}{\delta^2}(1+\eta \beta t)\\
& \ \ \ \ \ + \frac{12\sqrt{2}\eta dDB^*m^\frac{5}{2}}{\delta}\sqrt{1+\eta\beta t}\\
(h)&\ge \E[\E[\tilde{g}_{t-m}\mid\F_{t-2m}]^{\top}(x_{t-m}-x)] - \E[\|\tilde{g}_{t-m}\|_2\|x_{t-m}-x_{t-1}\|_2] \\
&\ge \E[\nabla \bar{f}_{t-m}(x_{t-1})^{\top}(x_{t-m}-x)] - \E[(\nabla \bar{f}_{t-m}(x_{t-1})-\E[\tilde{g}_{t-m}\mid \F_{t-2m}])^{\top}(x_{t-m}-x)]\\
& \ \ \ \ \ -\frac{18\eta d^2(B^*)^2m^3}{\delta^2}(1+\eta\beta t)\\
&\ge \E[\nabla \bar{f}_{t-m}(x_{t-1})^{\top}(x_{t-m}-x)] -\frac{8\eta D B^*dm^{\frac{5}{2}}\beta\sqrt{1+\eta\beta t}}{\delta} -\frac{18\eta d^2(B^*)^2m^3}{\delta^2}(1+\eta\beta t), \\
(i) &\le \frac{1}{m}\E[\|\tilde{g}_{t-m}\|_2^2]\le \frac{9d^2(B^*)^2m^3}{\delta^2}(1+\eta \beta t), 
\end{align*}
Putting together, we have
\begin{align*}
\frac{1}{\eta}\E[\|x_t-x\|_{\hat{A}_{t-m}}^2]&\le \frac{1}{\eta}\E[\|x_{t-m}-x\|_{\hat{A}_{t-m-1}}^2] + \E[\|x_{t-m}-x\|_{\nabla^2\bar{f}_{t-m}}^2] \\
& \ \ \ \ \ - 2 \E[\nabla \bar{f}_{t-m}(x_{t-1})^{\top}(x_{t-m}-x)] + C_1 \frac{\eta(1+\eta\beta t)}{\delta^2} \\
& \ \ \ \ \ +C_2\frac{\eta\sqrt{1+\eta\beta t}}{\delta},
\end{align*}
where
\begin{align*}
C_1 =90d^2(B^*)^2m^6, \ C_2=(17d+16\beta )DB^* m^{\frac{5}{2}}.
\end{align*}
Rearranging, we have
\begin{align*}
\E[\nabla\bar{f}_{t-m}(x_{t-1})^{\top}(x_{t-1}-x)]-\frac{1}{2}\E[\|x_{t-1}-x\|_{\nabla^2\bar{f}_{t-m}}^2]&\le \frac{1}{\eta}(\E[\|x_{t-1}-x\|_{\hat{A}_{t-m-1}}^2]-\E[\|x_t-x\|_{\hat{A}_{t-m}}^2])\\
& \ \ \ \ \ +C_1 \frac{\eta(1+\eta\beta t)}{\delta^2}  +C_2\frac{\eta\sqrt{1+\eta\beta t}}{\delta}.
\end{align*}
Summing over all iterations, we have
\begin{align*}
\sum_{t=2m}^{T}\E[\nabla\bar{f}_{t-m}(x_{t-m})^{\top}(x_{t-1}-x)]-\frac{1}{2}\E[\|x_{t-1}-x\|_{\nabla^2\bar{f}_{t-m}}^2]&\le \frac{1}{\eta}\E[\|x_{2m-1}-x\|_{\hat{A}_{m-1}}^2]+M\\
&\le \frac{mD^2}{\eta}+M,
\end{align*}
where $M=C_1 \frac{\eta(1+\eta\beta T)T}{\delta^2}  +C_2\frac{\eta\sqrt{1+\eta\beta T}T}{\delta}$. 
\begin{align*}
(3)&\le\sum_{t=m}^{T-m}\E\left[\bar{f}_{t}(x_t)-\bar{f}_{t}(x_{t+m-1})\right]+\E[\bar{f}_{t}(x_{t+m-1})-\bar{f}_{t}(x)]+mB\\
&=\underbrace{\sum_{t=m}^{T-m}\E\left[\nabla\bar{f}_{t}(x_t)^{\top}(x_t-x_{t+m-1})\right]}_{(j)}+\underbrace{\sum_{t=2m}^{T}\E[\bar{f}_{t-m}(x_{t-1})-\bar{f}_{t-m}(x)]}_{(k)} + mB.
\end{align*}
We can bound (j) and (k) separately:
\begin{align*}
(j)&\le \sum_{t=m}^{T-m} \E[\|\nabla \bar{f}_{t}(x_t)\|_2\|x_t-x_{t+m-1}\|_2] \\
&\le m\sum_{t=m}^{T-m}\E\underbrace{\left\|\sum_{i=1}^m\nabla_if_t(x_t,\dots,x_t)\right\|_2}_{\le\sqrt{m}\|\nabla f_t(x_t,\dots,x_t)\|}\sum_{s=t+1}^{t+m-1}\underbrace{\|x_s-x_{s-1}\|_2}_{\le 6\delta^{-1}\eta dB^*m(\sqrt{\eta s}+1)}\\
&\le \frac{6d\eta B^*G m^{\frac{7}{2}} (\sqrt{\eta T}+1)T}{\delta},\\
(k)&\le \sum_{t=2m}^T \E[\nabla\bar{f}_{t-m}(x_{t-1})^{\top}(x_{t-1}-x)]-\frac{1}{2}\E[\|x_{t-1}-x\|_{\nabla^2\bar{f}_{t-m}}^2]\le \frac{mD^2}{\eta}+M.
\end{align*}
Putting together, we have that
\begin{align*}
(3)&\le \frac{mD^2}{\eta} + mB + C_1 \frac{\eta (1+\eta\beta T)T}{\delta^2}  +C_2\frac{\eta\sqrt{1+\eta\beta T}}{\delta} + C_3\frac{\eta(\sqrt{\eta T}+1) T}{\delta},
\end{align*}
where $C_3=6dB^*Gm^{\frac{7}{2}}$. 
\end{proof}

\newpage



==> Backups/control_lower_bound.tex <==
\section{Beyond BCO with memory}
\subsection{Bandit LQR}
%There is a body of works in the nonstochastic control literature that studies the upper bounds of controlling a linear dynamical system with adversarial cost functions and perturbations under bandit feedback. Notably, \cite{cassel2020bandit} proves an upper bound of $\tilde{O}(T^{\frac{2}{3}})$ for smooth, adversarially chosen cost functions and adversarial perturbations. \cite{sun2023optimal} proved an optimal bound of $\tilde{O}(\sqrt{T})$ for strongly convex and smooth, adversarially chosen cost functions and semi-adversarial perturbations. These state-of-the-art results raise the natural questions that whether the gap between these two settings can be closed, or if there is a fundamental difference between the two settings. We answer this question. Indeed, Theorem~\ref{thm:lower-bound} induces natural corollaries that show lower bounds for both of the following settings: (1) bandit nonstochastic control with general convex, smooth cost functions, and (2) bandit nonstochastic control with strongly convex and smooth cost functions with adversarially chosen perturbation sequence. This shows that the results of \cite{cassel2020bandit} and \cite{sun2023optimal} are tight, even when we impose quadratic assumptions on the cost functions. 

\begin{definition} [Online LQR]
\label{def:lqr}
An online LQR problem concerns a linear dynamical system parametrized by matrices $(A,B)$
against a sequence of quadratic cost functions $c_t$. In particular, the linear dynamical system is given by
\begin{align*}
x_{t+1}=Ax_t+Bu_t+w_t,
\end{align*}
where $A\in\mathbb{R}^{d_x\times d_x}$, $B\in\mathbb{R}^{d_x\times d_u}$, $x_t$ is the system's state at time $t$, $u_t$ is the control exerted to the system by the controller at time $t$, and $w_t$ is the perturbation. At time $t$, after $u_t$ is played, the learner receives a cost $c_t(x_t,u_t)$. 
\end{definition}

Since in Definition~\ref{def:lqr}, we impose no distributional assumptions on $w_t, c_t$, and both can be time-varying, the performance of a control algorithm $\A$ that outputs the sequence $\{u_t\}_{t=1}^T$ is measured by \textit{regret} with respect to some policy class $\Pi$:
\begin{align*}
\regret_T^{\A,\Pi}=\sum_{t=1}^T c_t(x_t^{\A}, u_t^{\A})-\min_{\pi\in\Pi}\sum_{t=1}^T c_t(x_t^{\pi}, u_t^{\pi}).
\end{align*}
If we view the algorithm $\A$ as a control policy, then the notation $u_t^{\pi}$ for a control policy $\pi$ is the control the learner would play if they adopt $\pi$, and similarly $x_t^{\pi}$ is the state the system would reach if the $\pi$ was executed from the beginning of the time. 

It is intuitive from this expression that the validity and strength of an upper on the regret defined above strongly depends on the richness of the comparator policy class $\Pi$. If $\Pi$ is expressive, then a sublinear regret bound in the time horizon $T$ implies that the decisions played by $\A$ competes with a strong policy in hindsight. The state-of-art $\Pi$ used in a line of nonstochastic control of fully observable systems (which the LQR problem in Definition~\ref{def:lqr} belongs to) is the \textbf{DAC policy class}. We formally introduce the definition of the DAC policy class in Definition~\ref{def:dac}. On a high level, a DAC policy constructs its controller based on the past perturbations, which can be directly calculated by the state evolution equation in Definition~\ref{def:lqr}, had $A, B$ known to the learner. For simplicity, we assume the system is stable, i.e. the spectral radius of $A$ satisfies $\rho(A)<1$.

\begin{definition} [DAC policy class]
\label{def:dac}
A DAC policy $\pi_M$ of length $m$ is a sequence of $m$ matrices in $\mathbb{R}^{d_u\times d_x}$, $M=\{M^{[i]}\}_{i=1}^m$, such that at time $t$, the control played according of $\pi_M$ is given by
\begin{align*}
u_t^{\pi_M}=\sum_{i=1}^mM^{[i]}w_{t-i}.
\end{align*}
The DAC policy class parameterized by $(R, m)$ is any DAC policy $\pi_M$ of length $m$ and satisfy
\begin{align*}
\|M\|_{\ell_1,\mathrm{op}}\defeq \sum_{i=1}^{m} \|M^{[i]}\|_{\mathrm{op}}\le R.
\end{align*}
\end{definition}

\paragraph{Upper bounds in previous work.} Since there is a long line of research studying efficient online control algorithms with upper regret bounds in the setting, we will quickly discuss the setting and assumptions of these results, which will also hopefully help explain how the lower bound established in this work position among these results. In the full information setting where the function $c_t$ is given to the learner every round after the cost was incurred, without further assumptions on the curvature of $c_t$, \cite{agarwal2019online} attains $\tilde{O}(\sqrt{T})$ regret upper bound. If the perturbation sequence is stochastic, \cite{agarwal2019logarithmic} obtains the optimal $\poly(\log(T))$ regret upper bound. Or, if the quadratic function is strongly convex and smooth, \cite{simchowitz2020making} obtains the same optimal $\poly(\log(T))$ regret upper bound. In the bandit setting, where only a scalar cost evaluated at the resulting state and control played by the learner is accessible, without further assumptions on the curvature of $c_t$, \cite{cassel2020bandit} obtains a $\tilde{O}(T^{\frac{3}{4}})$ regret upper bound. If $c_t$ is smooth and the perturbation sequence is stochastic, \cite{cassel2020bandit} obtains a better regret bound of $\tilde{O}(T^{\frac{2}{3}})$ regret upper bound. Or, if $c_t$ is strongly convex and smooth and the perturbation model is semi-adversarial, \cite{sun2023optimal} obtains the optimal $\tilde{O}(\sqrt{T})$ regret upper bound. 

With these established results, it is natural to wonder whether the bandit LQR problem, when facing strongly convex cost functions but adversarial perturbations, would enjoy the optimal regret guarantee as in the full information setting. In other words, are the strong convexity assumption and the stochastic component in the perturbation model in bandit control of LQR with smooth quadratic costs necessary to establish optimal regret bound? 

The lower bound in Section~\ref{sec:bco-m} hints at the existence of such a lower bound. Most of the upper bounds established in the works listed above rely on the reduction of the online control problem to OCO-M since for a stable/stabilizable system the effects from past states and controls decay exponentially over time. However, as pointed out by \cite{simchowitz2020making}, the online control problem has a more specific memory structure, i.e. affine dependence on memory for DAC policy class, which they utilized to establish the optimal regret upper bound for the full information setting. Indeed, due to the special structure of the control problem, the hard instance constructed in Section~\ref{sec:bco-m} does not directly imply a lower bound in bandit LQR. Moreover, the result of \cite{simchowitz2020making} hints at the possibility of a tight upper bound if we utilize the affine memory structure. Interestingly, it turns out that in the bandit setting, it is impossible to obtain a $\tilde{O}(\sqrt{T})$ upper bound. We prove this lower bound in Theorem~\ref{thm:control-lower-bound}. 

%For now, we take a moment to explain why the bandit setting would not benefit from utilizing the affine structure of the memory. As pointed out by Theorem 2.3 in \cite{simchowitz2020making}, the reduction to OCO-M in the full information setting cannot achieve optimal regret bound because it relies on bounding the total Euclidean variation of the iterates produced. \cite{simchowitz2020making}


\begin{theorem}[LQR lower bound: general convex and smooth quadratic costs with adversarial perturbations.]
\label{thm:control-lower-bound}
There exists a stable linear dynamical system, a sequence of quadratic, smooth, and convex cost functions and a sequence of bounded perturbations chosen by an oblivious adversary such that any proper online control algorithm with bandit feedback incurs regret $\tilde{\Omega}(T^{\frac{3}{5}})$ against the DAC policy class. 
\end{theorem}
\begin{proof}
Consider the following linear dynamical system:
\begin{align*}
x_{t+1} = \frac{1}{2}u_{t} + 1,
\end{align*}
where $x_t\in\mathbb{R}$ is the state of the system at time $t$, $u_t\in\mathbb{R}$ is the control exerted to the system by the learner at time $t$. 

Suppose otherwise, $\exists$ proper online algorithm $\A$ such that $\forall$ sequence of convex and $\Theta(1)$-smooth quadratic costs $\{c_t\}_{t=1}^T$, we have the expected regret of $\A$ to be of order $\tilde{o}(T^{\frac{3}{5}})$ w.r.t. the DAC policy class. We show via a hard instance that such $\A$ does not exist. 

Consider $c_t$ of the following form:
\begin{align*}
c_t(x_t,u_t)=\ell_t(x_t)+(2x_t-2-u_t)^2,
\end{align*}
where $\ell_t$ is a linear function in $x_t$ that will be defined later. First, we note that $c_t$ is a convex and smooth quadratic function in $(x_t, u_t)$ since
\begin{align*}
c_t(x_t, u_t)= (x_t, u_t)^{\top}\begin{bmatrix}
4 & -2 \\
-2 & 1
\end{bmatrix}
(x_t, u_t)-4(2x_t-u_t)+\ell_t(x_t)+4,
\end{align*}
where $0\preceq \begin{bmatrix}
4 & -2 \\
-2 & 1
\end{bmatrix}\preceq 5I$. Let the benchmark DAC policy class $\Pi$ be of size $m$ and have radius bounded by $R$. Note that since we are in $\mathbb{R}$, $\Pi$ is simply a sequence of $M$ real numbers with sum of absolute values bounded above by $R$.  
Since the learning algorithm $\A$ is proper w.r.t. the DAC policy class, each $x_t, u_t$ admits the following representation: for some $M_1,\dots,M_T\in \Pi$,
\begin{align*}
x_t=\frac{1}{2}\sum_{i=1}^m M_{t-1}^{[i]}+1, \ u_t=\sum_{i=1}^m M_t^{[i]}.
\end{align*}
Therefore, we can rewrite $c_t$ as
\begin{align*}
c_t(x_t,u_t)&=\ell_t\left(\frac{1}{2}\sum_{i=1}^m M_{t-1}^{[i]}+1\right)+\left(\sum_{i=1}^m M_t^{[i]}-M_{t-1}^{[i]}\right)^2\\
&=\tilde{\ell}_t\left(\sum_{i=1}^m M_{t-1}^{[i]}\right)+\ell_t(1)+\left(\sum_{i=1}^m M_t^{[i]}-M_{t-1}^{[i]}\right)^2,
\end{align*}
where $\tilde{\ell}_t=\frac{1}{2}\ell_t$. Since we are interested in the regret, we can drop the term $\ell_t(1)$ as a constant offset. Note that by assumption, if suffices to consider $\tilde{\ell}_t$ defined on $\left[-R, R\right]$.

Recall the random process $\{\bar{n}_t\}_{t=1}^T$ defined in Section~\ref{sec:bco-m}, and define the functions $\tilde{\ell}_t$ as follows:
\begin{align*}
\tilde{\ell}_t\left(R\right)=\bar{n}_t+\frac{1}{2}-\mathbf{1}(\chi=1), \ \ \tilde{\ell}_t\left(-R\right)=\bar{n}_t+\frac{1}{2}-\mathbf{1}(\chi=0),
\end{align*}
where $\chi\sim \mathrm{Ber}\left(\frac{1}{2}\right)$ is sampled before the game starts. To preserve the linear structure of $\tilde{\ell}_t$, for any $x\in \left[-R, R\right]$, let
\begin{align*}
\tilde{\ell}_t(x)=\tilde{\ell}_t\left(-R\right)+\frac{\tilde{\ell}_t\left(R\right)-\tilde{\ell}_t\left(-R\right)}{R}x.
\end{align*}
Note that $\tilde{\ell}_t$ is oblivious to the learner's previous decisions. For simplicity, denote $S(M)=\sum_{i=1}^m M^{[i]}$. By assumption, $\A$ produces a sequence of $\{M_t\}_{t=1}^T$ satisfies
\begin{align*}
\E\left[\sum_{t=1}^T \tilde{\ell}_t\left(\sum_{i=1}^m M_{t-1}^{[i]}\right)+\left(\sum_{i=1}^m M_t^{[i]}-M_{t-1}^{[i]}\right)^2-\min_{S(M)\in\{-R, R\}}\sum_{t=1}^T\tilde{\ell}_t\left(\sum_{i=1}^m M^{[i]}\right)\right]=\tilde{o}(T^{\frac{3}{5}}), 
\end{align*}
where we make use of the fact that since $\tilde{\ell}_t$ is linear, its minimum over $\Pi$ is attained either at $-R$ or $R$. We relax the assumption on the bandit model: suppose $\A$ has full access to the moving cost $\left(\sum_{i=1}^m M_t^{[i]}-M_{t-1}^{[i]}\right)^2$ but only bandit access to the linear cost $\tilde{\ell}_t$. The first argument is given by the following lemma: 

\begin{lemma} [Rounding to discretized interval]
There exists an online algorithm $\A_1$ such that it outputs $Y_t$ such that $S(Y_t)=-R+\frac{2R}{n}k$ for some $0\le k\le n\in\mathbb{Z}$ and satisfies the following regret bound:
\begin{align*}
\E_{\A_1}\left[\sum_{t=1}^T \tilde{\ell}_t\left(\sum_{i=1}^m Y_t^{[i]}\right)+\left(\sum_{i=1}^m Y_t^{[i]}-Y_{t-1}^{[i]}\right)^2-\min_{S(M)\in\{-R, R\}}\sum_{t=1}^T \tilde{\ell}_t\left(\sum_{i=1}^m M^{[i]}\right)\right]\le \tilde{o}(T^{\frac{3}{5}})+\frac{T}{2n^2}. 
\end{align*}
\end{lemma}
\begin{proof}
The idea is to construct a rounding algorithm $\mathcal{R}_1$ that calls $\A$ as a subroutine and rounds its decision to a point in the feasible set, and the resulting algorithm $\A_1=\mathcal{R}_1\circ \A$. The tricky part is that the scalar loss seen by $\A_1$ will be evaluated at the rounded point. 

\js{Can we make the assumption that the algorithm, when given an unbiased estimator of the feedback, incurs the same regret?}

Consider the following rounding scheme $\mathcal{R}_1$: discretize the interval $[-R, R]$ into $n$ intervals (where we will decide $n$ later) of equal lengths, with endpoints $v_0=-R,\dots, v_k=-R+\frac{2R}{n},\dots, v_n=R$. At time $t$, after $\A$ output a decision $M_t$ such that $s(M_t)\in [v_k, v_{k+1}]$ for some $k$, let 
\begin{align*}
Y_t^{[i]}=\begin{cases}
M_t^{[i]}+\frac{v_{k+1}-S(M_t)}{m} & \forall i, \text{w.p. } n(S(M_t)-v_k)\\
M_t^{[i]}-\frac{S(M_t)-v_{k}}{m} & \forall i, \text{w.p. } n(v_{k+1}-S(M_t))\\
\end{cases},
\end{align*}
and $Y_{t_1}, Y_{t_2}$ are sampled independently for $t_1\ne t_2$, given $M_{t_1}, M_{t_2}$. Note that we have $\forall i\in[m]$,
\begin{align*}
\E_{\mathcal{R}_1}[Y_t^{[i]}\mid M_{1:t}]&=n(S(M_t)-v_k)\left(M_t^{[i]}+\frac{v_{k+1}-S(M_t)}{m}\right)+n(v_{k+1}-S(M_t))\left(M_t^{[i]}-\frac{S(M_t)-v_{k}}{m}\right)\\
&=M_t^{[i]}+\frac{n}{m}[(S(M_t)-v_k)(v_{k+1}-S(M_t))-(v_{k+1}-S(M_t))(S(M_t)-v_k)]\\
&=M_t^{[i]},\\
\mathrm{Var}_{\mathcal{R}_1}(Y_t^{[i]}\mid M_{1:t})&\le \frac{1}{4}\left(v_{k(M_t)+1}-v_{k(M_t)}\right)^2=\frac{1}{4n^2},
\end{align*}
where $v_{k(M_t)}$ is the endpoint where $M_t\in[v_{k(M_t)}, v_{k(M_t)+1}]$. Therefore, $\forall t$, we have
\begin{align*}
\E_{\mathcal{R}_1,\A}\left[\tilde{\ell}_t\left(\sum_{i=1}^m Y_t^{[i]}\right)+\left(\sum_{i=1}^m Y_t^{[i]}-Y_{t-1}^{[i]}\right)^2\right]&= \E_{\A}\left[\E_{\mathcal{R}_1}\left[\tilde{\ell}_t\left(\sum_{i=1}^m Y_t^{[i]}\right)+\left(\sum_{i=1}^m Y_t^{[i]}-Y_{t-1}^{[i]}\right)^2\mid M_{1:t}\right]\right]\\
&=\E_{\A}\left[\tilde{\ell}_{t}\left(\sum_{i=1}^m M_t^{[i]}+\left(\sum_{i=1}^m M_t^{[i]}-M_{t-1}^{[i]}\right)^2\right)\right] \\
& \ \ \ \ \ +\E_{\A}\left[\mathrm{Var}_{\mathcal{R}_1}\left(\sum_{i=1}^m Y_t^{[i]}\mid M_{1:t}\right)\right]\\
& \ \ \ \ \ +\E_{\A}\left[\mathrm{Var}_{\mathcal{R}_1}\left(\sum_{i=1}^m Y_{t-1}^{[i]}\mid M_{1:t-1}\right)\right]\\
&\le \E_{\A}\left[\tilde{\ell}_{t}\left(\sum_{i=1}^m M_t^{[i]}+\left(\sum_{i=1}^m M_t^{[i]}-M_{t-1}^{[i]}\right)^2\right)\right]+\frac{m}{2n^2}.
\end{align*}
Therefore, the regret bound of $\A$ implies that $\exists$ bandit algorithm $\mathcal{R}_1\circ \A$ over $\{v_0,\dots, v_n\}$ such that
\begin{align*}
\E_{\mathcal{R}_1, \A}\left[\sum_{t=1}^T \tilde{\ell}_t\left(\sum_{i=1}^m Y_t^{[i]}\right)+\left(\sum_{i=1}^m Y_t^{[i]}-Y_{t-1}^{[i]}\right)^2-\min_{S(M)\in\{-R, R\}}\sum_{t=1}^T \tilde{\ell}_t\left(\sum_{i=1}^m M^{[i]}\right)\right]\le \tilde{o}(T^{\frac{3}{5}})+\frac{T}{2n^2}. 
\end{align*}
Now, by construction of the $Y_t$'s, we have that
\begin{align*}
\left(\sum_{i=1}^m Y_t^{[i]}-Y_{t-1}^{[i]}\right)^2\ge \frac{1}{n}\left|\sum_{i=1}^m Y_t^{[i]}-Y_{t-1}^{[i]}\right|.
\end{align*}
Thus, the above regret bound implies that
\begin{align*}
\E_{\mathcal{R}_1, \A}\left[\sum_{t=1}^T \tilde{\ell}_t\left(\sum_{i=1}^m Y_t^{[i]}\right)+\frac{1}{n}\left|\sum_{i=1}^m Y_t^{[i]}-Y_{t-1}^{[i]}\right|-\min_{S(M)\in\{-R, R\}}\sum_{t=1}^T \tilde{\ell}_t\left(\sum_{i=1}^m M^{[i]}\right)\right]\le \tilde{o}(T^{\frac{3}{5}})+\frac{T}{2n^2}. 
\end{align*}
Now, we consider a second rounding algorithm $\mathcal{R}_2$ on $Y_t$. We construct $Z_t$ as the following:
\begin{enumerate}
\item At time $t=1$, let $p=\frac{S(Y_1)+R}{2R}$.Let
\begin{align*}
Z_1^{[i]}=\begin{cases}
Y_1^{[i]}+\frac{R-S(Y_1)}{m} & \forall i, \text{w.p. } p,\\
Y_1^{[i]}-\frac{R+S(Y_1)}{m} & \forall i, \text{w.p. } 1-p.
\end{cases}
\end{align*}
\item At time $t>1$, $\forall i\in[m]$, let
\begin{align*}
Z_t^{[i]}=\begin{cases}
\begin{cases}
Y_{t}^{[i]}+\frac{R-S(Y_t)}{m} & \forall i, \ \text{if } S(Z_{t-1})=R \\
\begin{cases}
Y_{t}^{[i]}+\frac{R-S(Y_t)}{m} & \forall i, \ \text{w.p. }\frac{S(Y_t)-S(Y_{t-1})}{R-S(Y_{t-1})} \\
Y_{t}^{[i]}-\frac{R+S(Y_t)}{m} & \forall i, \ \text{w.p. }1-\frac{S(Y_t)-S(Y_{t-1})}{R-S(Y_{t-1})}
\end{cases}
& \text{otherwise}
\end{cases}
& \text{if } S(Y_t)> S(Y_{t-1}) \\
\begin{cases}
Y_t^{[i]}-\frac{R+S(Y_t)}{m} & \forall i, \ \text{if }S(Z_{t-1})=-R \\
\begin{cases}
Y_{t}^{[i]}+\frac{R-S(Y_t)}{m} & \forall i, \ \text{w.p. }\frac{S(Y_t)+R}{S(Y_{t-1})+R}\\
Y_{t}^{[i]}-\frac{R+S(Y_t)}{m} & \forall i, \ \text{w.p. }1-\frac{S(Y_t)+R}{S(Y_{t-1})+R}
\end{cases}
& \text{otherwise}
\end{cases}
& \text{if } S(Y_t)\le S(Y_{t-1})
\end{cases}
\end{align*}
\end{enumerate}
First of all, to make the sampling distribution well defined, we introduce the following  claim:
\begin{claim}
$S(Z_t)=-R$ almost surely provided that $S(Y_t)=-R$.
\end{claim}
\begin{proof}
For $t=1$, by definition we have that if $S(Y_1)=-R$, then $p=0$, and thus $S(Z_1)=S(Y_1)-m\cdot\frac{R+S(Y_1)}{m}=-R$. For $t>1$,
\begin{align*}
\mathbb{P}_{\mathcal{R}_2}(S(Z_t)=-R\mid S(Y_t)=-R)&= \mathbb{P}_{\mathcal{R}_2}(S(Z_t)=-R\mid S(Z_{t-1})=-R, S(Y_t)=-R)\mathbb{P}_{\mathcal{R}_2}(S(Z_{t-1})=-R) \\
& \ \ \ \ \ + \mathbb{P}_{\mathcal{R}_2}(S(Z_t)=-R\mid S(Z_{t-1})=R, S(Y_t)=-R)\mathbb{P}_{\mathcal{R}_2}(S(Z_{t-1})=R).
\end{align*}
Note that by construction we have
\begin{align*}
\mathbb{P}_{\mathcal{R}_2}(S(Z_t)=-R\mid S(Z_{t-1})=-R, S(Y_t)=-R)&=1,\\
 \mathbb{P}_{\mathcal{R}_2}(S(Z_t)=-R\mid S(Z_{t-1})=R, S(Y_t)=-R)&=1.
\end{align*}
Thus, we have shown that $\mathbb{P}_{\mathcal{R}_2}(S(Z_t)=-R\mid S(Y_t)=-R)=1$.
\end{proof}
WE make the following observation of the conditional distribution of $Z_t$:
\begin{observation}
$\forall 1\le t\le T$, $\E_{\mathcal{R}_2}[Z_t\mid Y_{1:t}]=Y_t$, $\mathbb{P}_{\mathcal{R}_2}(S(Z_t)\ne S(Z_{t-1})\mid Y_{1:t})=|S(Y_{t})-S(Y_{t-1})|$.
\end{observation}
Since $S(Z_t)\in\{-R, R\}$, we have 
\begin{align*}
\frac{1}{2R}\E_{\R_2}\left[\left|\sum_{i=1}^m Z_t^{[i]}-Z_{t-1}^{[i]}\right|\mid Y_{1:t}\right]=\mathbb{P}\left(S(Z_t)\ne S(Z_{t-1})\mid Y_{1:t}\right)=\left|\sum_{i=1}^m Y_t^{[i]}-Y_{t-1}^{[i]}\right|.
\end{align*}

\end{proof}

\end{proof}

\newpage




==> Backups/lower-bound__3-5_bound_via_rounding.tex <==
\section{Bandit Lower Bound}
Theorem~\ref{thm:lower-bound} shows lower bound but has the following problems that we need to resolve:
\begin{enumerate}
\item The algorithm's decisions are strictly contained in the convex set $\K$, whereas in Algorithm~\ref{alg:bqo-memory} allows to play outside of the set. 
\item The reduction uses rounding: the feedback that the reduced algorithm receives should be the loss at the rounded point (an unbiased estimator of the original point) instead of the original point. We can assume that the algorithm, when given an unbiased estimator of the feedback, incurs the same regret. 
\item We are solving a harder problem: in the model of (\cite{dekel2014bandits, koren2017multi}), the moving cost is accessible to the algorithm. Only the loss vector is bandit information. Here, we have both loss and moving cost as bandit information. Can we do better?
\end{enumerate}

\begin{lemma}
Let $f_1,\dots,f_T\in\F$ be a sequence of loss functions of the form $f_t(x)=\ell_t(x)+g_t(x)$, $\forall x\in\K$, where $\ell_t$ is linear.
A possibly random online algorithm $\A$ has access to the function $g_t$ and bandit access to $\ell_t(x)$. Suppose $\A$ is supplied with feedback $\tilde{f}_t(x)=\ell_t(x+n_t(x))+g_t(x)$, where $n_t(x)$  is a random vector sampled from $\mathcal{D}(x)$ in the same space as $x$ satisfying $\E_{\mathcal{D}(x)}[n_t(x)]=0$, $n_t(x)$ is independent of $n_s(x)$ $\forall s\ne t$, $\forall x\in\K$. Furthermore, suppose the decisions $\{x_{t}^{\A}\}_{1\le t\le T}$ output by $\A$ satisfies expected regret guarantee $R_T$ with respect to $\{\tilde{f}_{t}\}_{t=1}^T$. Then, 
\begin{align*}
\E_{\A}\left[\sum_{t=1}^T f_t(x_t^{\A})-\min_{x\in\K}\sum_{t=1}^T f_t(x)\right]\le R_T.
\end{align*}
\end{lemma}
\begin{proof}
Let $x^*=\argmin_{x\in\K}\sum_{t=1}^T f_t(x)$. Note that
\begin{align*}
\E_{\mathcal{D},\A}[\tilde{f}_t(x_t^{\A})-\tilde{f}_{t}(x^*)]&=\E_{\mathcal{D},\A}[\ell_t(x_t^{\A}+n_t(x_t^{\A}))+g_t(x_t^{\A})-\ell_t(x^*+n_t(x^*))-g_t(x^*)]\\
&=_{(1)}\E_{\A}[f_t(x_t^{\A})-f_t(x^*)]+\E_{\A}[\ell_t(\E_{\mathcal{D}(x_t^{\A}),\mathcal{D}(x^*)}[n_t(x_t^{\A})-n_t(x^*)\mid x_{1:t}^{\A}])]\\
&=\E_{\A}[f_t(x_t^{\A})-f_t(x^*)]. 
\end{align*}
\end{proof}

\begin{theorem}
\label{thm:lower-bound}
There exists a sequence of $\{f_t\}_{t=2}^T$ with memory length $2$ defined on $\K=[0,1]$ satisfying assumptions stated in Section~\ref{sec:with-memory-loss-defs-and-assumptions} such that any online bandit algorithm $\A$ over $\K$ incurs regret $\tilde{\Omega}(T^{\frac{3}{5}})$. 
\end{theorem}
\begin{proof}
Suppose otherwise, $\forall$ sequence $\{f_t\}_{t=2}^T$ satisfying the assumptions stated in Section~\ref{sec:with-memory-loss-defs-and-assumptions}, $\exists$ an online bandit algorithm $\A$ over $[0,1]$ with regret guarantee $\tilde{o}(T^{\frac{3}{5}})$. We show via a hard instance that such $\A$ implies an upper bound that violates the known lower bound proved in existing literature (\cite{dekel2014bandits,koren2017multi}). 

Consider the $f_t$ constructed in the following way: let $L_t\in[0,1]^2$ be the loss vector over $2$ experts constructed in \cite{dekel2014bandits}. In particular, $L_t(1), L_t(2)\in[0,1]$ is the loss suffered by expert $1, 2$ at time $t$, respectively.
Construct the linear function $\ell_t:[0,1]\rightarrow[0,1]$, defined by $\ell_t(x)=L_t(1)+(L_t(2)-L_t(1))x$. In particular, $\ell_t(0)=L_t(1)$, $\ell_t(1)=L_t(2)$. Let $f_t(x_{t-1},x_t)=\ell_t(x_t)+(x_t-x_{t-1})^2$. $f_t$ satisfies the assumptions in Section~\ref{sec:with-memory-loss-defs-and-assumptions}. By assumption, $\exists \A$ bandit online algorithm that outputs a sequence of $\{x_t\}_{t=1}^T$ with regret guarantee:
\begin{align*}
\E_{\A}\left[\sum_{t=2}^T \ell_t(x_t)+(x_t-x_{t-1})^2-\min_{x\in\{0,1\}} \sum_{t=2}^T\ell_t(x)\right]=\tilde{o}(T^{\frac{3}{5}}),
\end{align*}
where the expectation is taken over any possible randomness in generating $\{x_t\}_{t=1}^T$ according to $\A$. Note that it suffices to consider the comparator class to be $\{0,1\}$, as with the unary form of $f_t$, the quadratic moving cost is always zero, and the minimum of a linear function is attained at the boundary of the set $[0,1]$. We can assume that the algorithm access $f_t$ is a semi-bandit way: $\A$ has full access to the moving cost function $(x_t-x_{t-1})^2$ and access $\ell_t(x_t)$ through bandit information. 

Consider the following rounding scheme $\mathcal{R}_1$: discretize $[0,1]$ into $n$ intervals of equal lengths, with endpoints $v_0=0, \dots, v_k=\frac{k}{n}, \dots, v_n=1$. At time $t$, after $\A$ output a decision $x_t\in[v_k,v_{k+1}]$, let $y_t=v_k$ with probability $n(v_{k+1}-x_t)$, and $y_t=v_{k+1}$ with probability $n(x_t-v_k)$. $y_s$ and $y_t$ are sampled independently for $s\ne t$, given $x_s, x_t$. We have $\E_{\mathcal{R}_1}[y_t\mid x_{1:t}]=x_t$, and since when given $x_t\in[v_k,v_{k+1}]$, $y_t\in\{v_k,v_{k+1}\}$, $\mathrm{Var}_{\mathcal{R}_1}(y_t\mid x_{1:t})\le \frac{1}{4n^2}$. Then $\forall t$, 
\begin{align*}
\E_{\mathcal{R}_1,\A}[\ell_t(y_t)+(y_t-y_{t-1})^2]&=\E_{\A}[\E_{\mathcal{R}_1}[\ell_t(y_t)+(y_t-y_{t-1})^2\mid x_{1:t}]]\\
&=\E_{\A}[\ell_t(x_t)+(x_t-x_{t-1})^2]+\E_{\A}[\mathrm{Var}_{\mathcal{R}_1}(y_t\mid x_{1:t})+\mathrm{Var}_{\mathcal{R}_1}(y_{t-1}\mid x_{1:t-1})]\\
&\le \E_{\A}[\ell_t(x_t)+(x_t-x_{t-1})^2]+\frac{1}{2n^2}.
\end{align*}
Therefore, the regret bound of $\A$ implies that $\exists$ bandit algorithm $\mathcal{R}_1\circ \A$ over $\{v_0,\dots,v_n\}$ such that
\begin{align*}
\E_{\mathcal{R}_1,\A}\left[\sum_{t=2}^T \ell_t(y_t)+(y_t-y_{t-1})^2-\min_{x\in\{0,1\}}\sum_{t=2}^T\ell_t(x)\right]\le\tilde{o}\left(T^{\frac{3}{5}}\right)+\frac{T}{2n^2}.
\end{align*}
By construction of $y_t$, $(y_t-y_{t-1})^2\ge \frac{1}{n}|y_t-y_{t-1}|$, $\forall t>1$. Thus, the above bound further implies that
\begin{align*}
\E_{\mathcal{R}_1,\A}\left[\sum_{t=2}^T \ell_t(y_t)+\frac{1}{n}|y_t-y_{t-1}|-\min_{x\in\{0,1\}}\sum_{t=2}^T\ell_t(x)\right]\le\tilde{o}\left(T^{\frac{3}{5}}\right)+\frac{T}{2n^2}.
\end{align*}
So far, we have successfully reduced the quadratic movement cost to a metric cost. To see that this implies an upper bound on the multi-armed bandit (MAB) problem, we consider another rounding algorithm $\mathcal{R}_2$ that rounds each $y_t$ to $z_t\in\{0,1\}$. Let $z_1\sim\mathrm{Ber}(y_1)$. At time $t>1$, $\mathcal{R}_1\circ \A$ outputs decision $y_t$. If $y_t> y_{t-1}$, let $z_t=z_{t-1}$ if $z_{t-1}=1$, else let $z_t=1$ with probability $\frac{y_t-y_{t-1}}{1-y_{t-1}}$ and $0$ otherwise. If $y_t\le y_{t-1}$, let $z_{t}=z_{t-1}$ if $z_{t-1}=0$, else let $z_t=1$ with probability $\frac{y_t}{y_{t-1}}$ and $0$ otherwise. First of all, to make the sampling distribution of $\mathcal{R}_2$ well defined, we introduce the following claim:
\begin{claim}
\label{claim:well-defined-smapling}
$z_t=0$ almost surely provided $y_t=0$.
\end{claim}
\begin{proof} [Proof of Claim~\ref{claim:well-defined-smapling}]
For $t=1$, by definition $z_1\sim\mathrm{Ber}(y_1)$, $\mathbb{P}_{\mathcal{R}_2}(z_1=0\mid y_1=0)=1$. For $t>1$,
\begin{align*}
\mathbb{P}_{\mathcal{R}_2}(z_{t}=0\mid y_{t}=0)&=\underbrace{\mathbb{P}_{\mathcal{R}_2}(z_{t}=0\mid z_{t-1}=0, y_{t}=0)}_{=1}\mathbb{P}_{\mathcal{R}_2}(z_{t-1}=0)+ \\
& \ \ \ \ \ +\underbrace{\mathbb{P}_{\mathcal{R}_2}(z_{t}=0\mid z_{t-1}=1, y_{t}=0)}_{=1}\mathbb{P}_{\mathcal{R}_2}(z_{t-1}=1)\\
&= 1.
\end{align*}
\end{proof}
In particular, Claim~\ref{claim:well-defined-smapling} shows that if $y_t=y_{t-1}=0$, $z_{t-1}=0$ almost surely. Thus, the sampling distribution is well defined. We make the following observation of the conditional distribution of $z_t$:
\begin{observation}
$\forall 1\le t\le T$, $\E_{\mathcal{R}_2}[z_t\mid y_{1:t}]=y_t$. $\forall 1<t\le T$, $\mathbb{P}_{\mathcal{R}_2}(z_t\ne z_{t-1}\mid y_{1:t})=|y_t-y_{t-1}|$. 
\end{observation}
Note that since $z_t\in\{0,1\}$, $\E_{\mathcal{R}_2}[|z_t-z_{t-1}|\mid y_{1:t}]=\mathbb{P}_{\mathcal{R}_2}(z_t\ne z_{t-1}\mid y_{1:t})=|y_t-y_{t-1}|$. Therefore, by taking $n=(100\log_2 T)^{\frac{3}{5}}T^{\frac{1}{5}}$, the $z_t$'s output by the bandit algorithm $\mathcal{R}_2\circ \mathcal{R}_1\circ \A$ satisfies
\begin{align*}
\E_{\mathcal{R}_2, \mathcal{R}_1, \mathcal{\A}}\left[\sum_{t=2}^T \ell_t(z_t)+\frac{1}{n}|z_t-z_{t-1}|-\min_{x\in\{0,1\}}\sum_{t=2}^T\ell_t(x)\right]\le\tilde{o}\left(T^{\frac{3}{5}}\right)+\frac{1}{2}(100\log_2 T)^{-\frac{6}{5}}T^{\frac{3}{5}}.
\end{align*}
On the other hand, let $\Delta(x,y)=\frac{1}{n}|x-y|$ be the metric in Theorem 15 of \cite{koren2017multi}, which refers to the result of \cite{dekel2014bandits}, which states that the above regret is at least $\left(\frac{2}{n}\right)^{\frac{1}{3}}T^{\frac{2}{3}}/(100\log_2 T)=2^{\frac{1}{3}}(100\log_2T)^{-\frac{6}{5}}T^{\frac{3}{5}}$, contradiction.
\end{proof}


==> Backups/lower-bound__praneeth_s_notes.tex <==
\section{Rough notes about the lower bound}
Let $\ell^*$ be an unbiased Bernoulli $\pm 1$ random variable. Consider the following hard instance.
\begin{align*}
    \ell_t(x) &= \epsilon \ell^* x + \overline{n}_t \\
    \overline{n}_t &= \overline{n}_{\rho(t)} + \mathcal{N}(0,\sigma^2),
\end{align*}
where $x \in [0,1]$, the parent function $\rho:[T]\rightarrow [T]$ is as defined in~\cite{dekel2014bandits}, and $\epsilon$ is a parameter that will be chosen later.
Let $Q_0$ and $Q_1$ be the conditional distributions where $\ell^*$ is equal to $1$ and $-1$ respectively (i.e., $x=0$ and $x=1$ are the minimizers of the cumulative loss respectively). We first note that under both $Q_0$ as well as $Q_1$, the distribution of $\ell_t(x_t)$ is independent of everything else in the past given $x_t$ and $(x_{\rho(t)},\ell_{\rho(t)}(x_{\rho(t)}))$. Denoting $Y_t = (x_t, \ell_t(x_t))$, we can bound the KL divergence of $Y_t$, under $Q_0$ and $Q_1$, conditioned on $Y_{\rho^*(t)}$ as follows:
\begin{align*}
    \Delta(Y_t | Y_{\rho^*(t)}) &= \E_{Q_0} \left[KL(\mathcal{N}(\epsilon(x_t - x_{\rho(t)}), \sigma^2), \mathcal{N}(-\epsilon(x_t - x_{\rho(t)}), \sigma^2))\right] \\
    &\leq \left( \frac{\epsilon (x_t - x_{\rho(t)})}{\sigma}\right)^2.
\end{align*}
Summing over $t$, we see that the total KL divergence can be upper bounded as:
\begin{align*}
    KL(Q_0 || Q_1) \leq \frac{\epsilon^2}{\sigma^2} \sum_t \left(x_t - x_{\rho(t)}\right)^2.
\end{align*}
By Pinsker's inequality, we then have:
\begin{align*}
    TV(Q_0, Q_1) \leq \sqrt{KL(Q_0||Q_1)} \leq \frac{\epsilon }{\sigma} \sqrt{\sum_t (x_t - x_{\rho(t)})^2}.
\end{align*}
Using a similar argument as in the proof of Lemma~5 in~\cite{dekel2014bandits}, we can show that:
\begin{claim}
\begin{align*}
    \E[\textrm{Regret}] &\geq (1-TV(Q_0,Q_1)) \frac{\epsilon T}{2} + \E[M] \\
    &\geq \left({1}{}-\frac{\epsilon}{\sigma} \sqrt{\sum_t (x_t - x_{\rho(t)})^2}\right) \frac{\epsilon T}{2} + \E[M],
\end{align*}
where $M$ is the movement cost.
\end{claim}
\begin{proof}
We see that the optimum under $Q_0$ is $x=0$ and that under $Q_1$ is $x=1$. So, the regret is given by:
\begin{align*}
    \E[Regret] &= \sum_t \left(\frac{1}{2}\cdot \epsilon \E_{Q_0}[x_t] + \frac{1}{2}\cdot \epsilon \E_{Q_1}[1-x_t] \right) + \E[M]\\
    &= \frac{\epsilon T}{2} + \frac{\epsilon}{2} \sum_t \int_{x=0}^1 x \left(p(x_t=x|Q_0) - p(x_t=x|Q_1)\right) dx + \E[M] \\
    &\geq \frac{\epsilon T}{2} - \frac{\epsilon}{2} \sum_t \int_{x=0}^1 \left|p(x_t=x|Q_0) - p(x_t=x|Q_1)\right| dx + \E[M] \\
    &= \frac{\epsilon T}{2} \left(1 - TV(Q_0,Q_1)\right) + \E[M] \\
    &\geq \left({1}{}-\frac{\epsilon}{\sigma} \sqrt{\sum_t (x_t - x_{\rho(t)})^2}\right) \frac{\epsilon T}{2} + \E[M].
\end{align*}
This proves the claim.
\end{proof}
If our movement cost is $M = \sum_t (x_t - x_{\rho(t)})^2$, then choosing $\sigma = 1$ and $\epsilon = T^{-1/3}$, we note that the minimum value of right hand side above is attained when $\sum_t (x_t - x_{\rho(t)})^2 = \epsilon^{-2}$, which when minimized over $\epsilon$ gives a regret lower bound of $T^{2/3}$ as desired.

\js{Can we take $L_t'(x)=\eps\ell^*(x-x_{t-1})+\bar{n}_t$? Then we have $Y_t=L_t'(x_t)=Y_{\rho(t)}+\ell^*\eps(x_t-x_{t-1})-\eps(x_{\rho(t)}-x_{\rho(t)-1})+\xi_t$, then the KL divergence can be bounded by $4\eps^2[(x_t-x_{t-1})^2+(x_{\rho(t)}-x_{\rho(t)-1})^2]/\sigma^2]$. By the bound on the depth of the process, we have $\sum_{t=1}^T (x_{\rho(t)}-x_{\rho(t)-1})^2\le (\lfloor \log_2(T) \rfloor +1) \sum_{t=1}^T (x_t-x_{t-1})^2$.}
\pn{This sounds like a great idea! Seems like this should give the desired $T^{2/3}$ lower bound for constant memory setting.}% Equation $(6)$ in~\cite{dekel2014bandits} can be modified to show that:
% \begin{align*}
%     \Delta(Y_t | Y_{\rho^*(t)}) \leq D_{\mathrm{KL}}(N(0,\sigma^2), N(\epsilon(x_t^{(i)} - x_{\rho(t)}^{(i)}), \sigma^2))
%     \leq \frac{\eps^2 (x_t^{(i)} - x_{\rho(t)}^{(i)})^2}{2 \sigma^2}
% \end{align*}
% \begin{align*}
%     \begin{bmatrix}
%         x_{t} \\ x_{t-1}
%     \end{bmatrix}^\top \begin{bmatrix}
%         A_1 & A_2 \\ A_2^\top & A_3
%     \end{bmatrix}     \begin{bmatrix}
%         x_{t} & x_{t-1}
%     \end{bmatrix} -     \begin{bmatrix}
%         x \\ x
%     \end{bmatrix}^\top \begin{bmatrix}
%         A_1 & A_2 \\ A_2^\top & A_3
%     \end{bmatrix}     \begin{bmatrix}
%         x & x
%     \end{bmatrix} = O(||x_t - x_{t-1}||^2) + gradient based terms.
% \end{align*}

\paragraph{Average memory of the constructed lower bound.} The average memory is bounded by $\log_2 T$. 
\begin{claim}
$\forall T\ge 6$, $\frac{1}{T}\sum_{t=1}^T \delta(t)\le \log_2 T$. 
\end{claim}
\begin{proof}
Define $N_k:=\{t\le T: \delta(t)=k\}$, $k\ge 0$. Note that for a given $T$, the largest possible $k$ such that $N_k\ne\emptyset$ is $k=\lfloor \log_2 T\rfloor$. $N_0$ consists of all odd numbers and therefore has cardinality $|N_0|\le \lfloor\frac{T}{2}\rfloor + 1$. $N_1$ consists of all even numbers non-divisible by $4$ and thus has cardinality $|N_1|\le \lfloor \frac{T}{4}\rfloor + 1$. The cardinality of other $N_k$'s can be bounded similarly. Therefore, 
\begin{align*}
\frac{1}{T}\sum_{t=1}^T \delta(t)&\le \frac{1}{T}\left(\frac{T}{2}+2\cdot \frac{T}{4}+\dots+2^{k-1}\cdot\frac{T}{2^{k}}+2^k\cdot\frac{T}{2^k}+k\right)\\
&=\frac{k}{2}+ 1 + \frac{k}{T}\\
&\le \log_2 T.
\end{align*}
\end{proof}


==> Backups/perturbation_loss_bound.tex <==
\begin{align*}
\frac{1}{2} \sum_{t=m}^T \E[u_{t-m+1:t}^{\top}\hat{A}_{t-m:t-1}^{-\frac{1}{2}}\nabla^2 f_t \hat{A}_{t-m:t-1}^{-\frac{1}{2}}u_{t-m:1:t}]&\le \frac{1}{2}\sum_{t=m}^T \trace\left(\hat{A}_{t-m}^{-\frac{1}{2}}\sum_{i=1}^m [\nabla^2 f_t]_{ii}\hat{A}_{t-m}^{-\frac{1}{2}}\right)\\
&\le \frac{\beta\tilde{R}_{G}}{2}\sum_{t=m}^{T}\trace\left(\hat{A}_{t-m}^{-\frac{1}{2}}\left(\sum_{s=t-m+1}^t Y_{s}^{\top}Y_{s}\right)\hat{A}_{t-m}^{-\frac{1}{2}}\right)\\
&\le \frac{2\sigma m^2\beta\tilde{R}_{G}}{\kappa(G)}\sum_{t=m}^{T}\trace\left(\hat{A}_{t}^{-\frac{1}{2}}\left(\frac{\kappa(G)}{4m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}\right) \hat{A}_{t}^{-\frac{1}{2}}\right),
\end{align*}
where the third inequality follows from that since $\hat{A}_t\succeq mI$, $\forall t$, we have that $\forall s < t$,
\begin{align*}
\hat{A}_t=\hat{A}_s+\frac{1}{2}\sum_{r=s+1}^t H_r\preceq \hat{A}_s+\frac{\sigma m(t-s)}{2}I\preceq \left(1+\frac{\sigma(t-s)}{2}\right)\hat{A}_s,
\end{align*}
which implies that assuming $\hat{A}_{t}\preceq \max\{2,\sigma m\}\hat{A}_{t-m}\preceq \sigma m\hat{A}_{t-m}$. 
We can further decompose the sum of traces as
\begin{align*}
\sum_{t=m}^{T}\trace\left(\hat{A}_{t}^{-\frac{1}{2}}\left(\frac{\kappa(G)}{4m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}\right) \hat{A}_{t}^{-\frac{1}{2}}\right)&=\sum_{t=m}^{T}\trace\left(\hat{A}_{t}^{-\frac{1}{2}}\left(\frac{1}{2}H_t\right) \hat{A}_{t}^{-\frac{1}{2}}\right)\\
& \ \ \ \ \ +\frac{1}{2}\sum_{t=m}^{T}\trace\left(\hat{A}_{t}^{-\frac{1}{2}}\left(\frac{\kappa(G)}{2m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}-H_t\right) \hat{A}_{t}^{-\frac{1}{2}}\right).
\end{align*}
To bound the first term, note that
\begin{align*}
\sum_{t=m}^{T}\trace\left(\hat{A}_{t}^{-\frac{1}{2}}\left(\frac{1}{2}H_t\right) \hat{A}_{t}^{-\frac{1}{2}}\right)=\sum_{t=m}^{T}\trace\left(\hat{A}_{t}^{-\frac{1}{2}}\left(\hat{A}_t-\hat{A}_{t-1}\right) \hat{A}_{t}^{-\frac{1}{2}}\right)\le \sum_{t=m}^T \log \frac{|\hat{A}_{t}|}{|\hat{A}_{t-1}|}\le \log (|\hat{A}_{T}|)\le d\log (\sigma T),
\end{align*}
where $|A|$ denotes the determinant of $A$, and the first inequality follows from that for $A, B\succ 0$, $A^{-1}\cdot(A-B)\le \log\left(\frac{|A|}{|B|}\right)$. The last inequality follows from $|\hat{A}_T|\le \|\hat{A}_T\|_2^d$. 

It is left to bound the second term. We use the ``blocking" technique introduced in \cite{simchowitz2020making} to bound this term. In particular, for $\tau=\Theta(\sqrt{T})$, consider endpoints $k_j=\tau(j-1)+m$, $j=1,\dots,J$, where $J=\lfloor \frac{T}{\tau}\rfloor$. We can rewrite the sum of the second term as
\begin{align*}
\sum_{t=m}^{T}\trace\left(\hat{A}_{t}^{-\frac{1}{2}}\left(\frac{\kappa(G)}{2m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}-H_t\right) \hat{A}_{t}^{-\frac{1}{2}}\right)&=\sum_{j=1}^{J}\sum_{t=k_j}^{k_{j+1}-1}\left(\frac{\kappa(G)}{2m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}-H_t\right)\cdot \hat{A}_{t}^{-1}\\
& \ \ \ \ \ +\sum_{t=J\tau+1}^T\left(\frac{\kappa(G)}{2m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}-H_t\right)\cdot \hat{A}_{t}^{-1}\\
&\le_{(1)}\sum_{j=1}^{J}\sum_{t=k_j}^{k_{j+1}-1}\left(\frac{\kappa(G)}{2m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}-H_t\right)\cdot \hat{A}_{t}^{-1}\\
& \ \ \ \ \ +\frac{\tau\kappa(G)dR_Y^2}{2m},\\
\end{align*}
where (1) follows from that $T-J\tau\le \tau$ and 
\begin{align*}
\left(\frac{\kappa(G)}{2m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}-H_t\right)\cdot \hat{A}_{t}^{-1}\le \frac{\kappa(G)d}{2m^2}\sum_{s=t-m+1}^t \|Y_s^{\top}Y_s\|_2\le \frac{\kappa(G)dR_Y^2}{2m}.
\end{align*}
We continue to bound the first term on the right hand side. Note that we can shift $\hat{A}_{t}$ to $\hat{A}_{k_j}$ for each $t\in[k_j,k_{j+1})$ at the expense of the moving cost. In particular,
\begin{align*}
\sum_{j=1}^{J}\sum_{t=k_j}^{k_{j+1}-1}\left(\frac{\kappa(G)}{2m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}-H_t\right)\cdot \hat{A}_{t}^{-1}&=\underbrace{\sum_{j=1}^{J}\sum_{t=k_j}^{k_{j+1}-1}\left(\frac{\kappa(G)}{2m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}-H_t\right)\cdot \hat{A}_{k_j}^{-1}}_{(a)}+\\
& \ \ \ \ \ \underbrace{\sum_{j=1}^{J}\sum_{t=k_j}^{k_{j+1}-1}\left\|\frac{\kappa(G)}{2m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}-H_t\right\|_{*}\|\hat{A}_t^{-1}-\hat{A}_{k_j}^{-1}\|_2}_{(b)},
\end{align*}
where $\|A\|_*$ denotes the nuclear norm of matrix $A$. We proceed to bound (a) and (b) separately. 



To bound the second term, we use Proposition 4.8 from \cite{simchowitz2020making}, which established a relationship between the sum of $Y_t^{\top}Y_t$ and $H_t$.
\begin{lemma}[Proposition 4.8 in \cite{simchowitz2020making}]
\label{lem:YtHt-inequality}
$\forall Y_1,\dots,Y_T$, there is
\begin{align*}
\sum_{t=m}^T H_t\succeq \frac{\kappa(G)}{2}\sum_{t=1}^T Y_t^{\top}Y_t-5mR_GR_YI. 
\end{align*}
\end{lemma}
Therefore, 
\begin{align*}
\frac{1}{2}\sum_{t=m}^{T}\trace\left(\hat{A}_{t}^{-\frac{1}{2}}\left(\frac{\kappa(G)}{2m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}-H_t\right) \hat{A}_{t}^{-\frac{1}{2}}\right)&\le \frac{1}{2m}\trace\left(\sum_{t=m}^T\frac{\kappa(G)}{2m}\sum_{s=t-m+1}^tY_{s}^{\top}Y_{s}-H_t\right)\\
&\le \frac{1}{2m}\trace\left(\frac{\kappa(G)}{2}\sum_{t=1}^TY_{t}^{\top}Y_{t}-\sum_{t=m}^TH_t\right)\\
&\le \frac{5R_GR_Yd}{2}. 
\end{align*}


Combining, we have that
\begin{align*}
(\text{perturbation loss})\le \frac{2\sigma m^2\beta\tilde{R}_{G}d}{\kappa(G)}\log (\sigma T)+\frac{5\sigma m^2\beta\tilde{R}_{G}R_GR_Yd}{\kappa(G)}.
\end{align*}

==> Backups/portfolio.tex <==
\subsection{Online Portfolio Selection}

Online portfolio selection \cite{cover1991universal} is one of the most well studied problems in online learning. In the problem, the learner (investor) is faced with $d$ assets. At each time $t$, the learner needs to pick a vector $x_t$ from the $d$-dimensional simplex $\Delta_d:=\{x\in\mathbb{R}^d\mid x\ge 0, \|x\|_1=1\}$ that represents the distribution over assets, i.e. a portfolio. The adversary supplies a market return vector $r_t\in [\eps,1]^d$, $\eps\ge 0$, to which the learner suffers loss
$$ f_t(x)  = - \log (x^\top r_t) . $$  
In numerous works it is assumed that the market volatility is bounded, which amounts to $\eps > 0$. 

The loss functions in portfolio selection are $\kappa$ convex for $\kappa = \frac{1}{\eps^2}$, as can be seen since
\begin{align*}
r_tr_t^{\top}\preceq \nabla^2 f_t(x) = \frac{r_t r_t^\top}{(x_{t}^{\top} r_t)^2}\preceq \frac{1}{\eps^2}r_tr_t^{\top}.
\end{align*}
There is a long line of work studying the regret guarantee in the full information setting of the online portfolio selection problem (\cite{luo2018efficient, mhammedi2022damped}). This scenario presumes that investors have unrestricted access to the returns of all assets. Yet, this assumption doesn't hold in many practical situations where investors only see returns from their chosen investments. This limitation has led to the development of the bandit version of the problem. In this bandit framework, \cite{ito2018regret} explored the problem with an added cardinality constraint: investors are restricted to a subset of possible assets for investment of a specified cardinality. They obtained optimal regret bound via an algorithm that combines the EXP3 and the FTAL algorithms. However, the obtained regret and runtime scale with the size of the feasible combinations of assets, leading to a runtime exponential in the total number of assets if we allow full cardinality for investment. 

\js{Do we need the algorithm to be proper? Can fill this table when we finish the proper learning part.}

\begin{table*}[hbt!]
	\centering
	\small % Reducing the font size
	{
		\begin{tabular}{c||c|c|c} % Adjust the width (2cm) as needed
			\hline
			Paper & Feedback & Regret & Comp.  %&%
			\\ [0.5ex]
			\hline\hline
            \cite{ito2018regret}  & bandit & $\tilde{O}(e^d\sqrt{T})$  & $\mathrm{poly}(d)$
			\\\hline
\cite{bubeck2017kernel}  & bandit & $\tilde{O}(d^{9.5} \sqrt{T})$  & $\mathrm{poly}(d)$
			\\\hline		
   \textbf{} &  bandit & $O(d^{3/2}\sqrt{T})$ &  $d^2$
			\\\hline
		\end{tabular}
	}
 \caption{Comparison with relevant prior works for online portfolio selection.}
	\label{tab:portfolio_selection_comparisons}
\end{table*}





==> Backups/second-order.tex <==
\subsubsection{BQO-M algorithm: second order}
\js{Conjecture: second-order algorithm allowing playing outside of the set should give a better bound than the first-order algorithm. Still working in progress.} \ar{Do we expect to improve the $T^{2/3}$ upper bound from above for general smooth, convex functions? Or do we expect to see improvements in special cases?}
\begin{algorithm}
\caption{Bandit Quadratic Optimization with Memory (\texttt{BQO-M})}\label{alg:bqo-memory}
\begin{flushleft}
  {\bf Input:} convex set $\K$, step size $\eta>0$, perturbation parameter $\delta\in[0,1]$. 
\end{flushleft}
\begin{algorithmic}[1]
\STATE Initialize: $x_{1}=\dots=x_{m}\in\K$, $\tilde{g}_{0:m-1} = \mathbf{0}_{d}$, $\hat{H}_{0:m-1}=\mathbf{0}_{d\times d}$, $ \hat{A}_{-(m-1):m-1} = I$.
\STATE Sample $v_{t,1}, v_{t,2}\sim S^{d-1}$ i.i.d. uniformly at random for $t=1,\dots,m$. 
\STATE Set $y_t = x_t + \frac{\delta}{2}\hat{A}_{t-m}^{-\frac{1}{2}}(v_{t,1}+v_{t,2})$, $t=1,\dots,m$. 
\FOR{$t = m, \ldots, T$}
\STATE Play $y_t$, observe $f_t(y_{t-m+1:t})$.
\STATE Create gradient and Hessian estimates:
\begin{align*}
\tilde{g}_{t}&=2\frac{d}{\delta}f_t(y_{t-m+1:t}) \sum_{j=0}^{m-1}\hat{A}_{t-j-m}^{\frac{1}{2}}v_{t-j,1}\in\mathbb{R}^{d}, \\
\hat{H}_{t}&=2\frac{d^2}{\delta^2}f_t(y_{t-m+1:t})\sum_{j,k=0}^{m-1}\hat{A}_{t-j-m}^{\frac{1}{2}}(v_{t-j,1}v_{t-k,2}^{\top}+v_{t-k,2}v_{t-j,1}^{\top})\hat{A}_{t-k-m}^{\frac{1}{2}}\in\mathbb{R}^{d\times d}.
\end{align*}
\STATE Update $\hat{A}_{t}=\eta \sum_{s\le t, s\in M_i}\hat{H}_{s}+I$ if $t\in M_i$, where $M_i=\{t: t\equiv i\mod m\}$, for $i=0,\dots,m-1$. \js{maybe instead of total gradient estimator sum, we sum over each modular class dividing $m$}
\STATE Update
$ x_{t+1} = \prod_{\K}^{\hat{A}_{t-m+1}} \left[ x_{t-m+1} - \eta \hat{A}_{t-m+1}^{-1}  \tilde{g}_{t-m+1}  \right]$.
\STATE Set $y_{t+1}=x_{t+1}+\frac{\delta}{2} \hat{A}_{t-m+1}^{-\frac{1}{2}}(v_{t+1,1}+v_{t+1,2})$, $v_{t+1,1}, v_{t+1,2}\sim S^{d-1}$ i.i.d. uniformly at random. 
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsubsection{BQO-M analysis: second order}

\begin{lemma} [Unbiased estimators]
\label{lem:unbiased-estimators}
$\tilde{g}_{t}$ and $\tilde{H}_{t}$ are conditionally unbiased estimators of the following statistics: 
\begin{align*}
\E[\tilde{g}_{t}\mid \F_{t-m}]= \nabla\cdot f_t(x_{t-m+1:t}), 
\ \   
\E[\hat{H}_{t}\mid\F_{t-m}] = \nabla^2 \bar{f}_{t},
\end{align*}
where $\F_t=\sigma(\{(v_{s,1},v_{s,2})\}_{s\le t})$ is the filtration generated by the algorithm's random sampling up to time $t$.
\end{lemma}
\begin{proof}
First, note that by design of Algorithm~\ref{alg:bqo-memory}, $y_t, \tilde{g}_t, \tilde{H}_t, \hat{H}_t, \tilde{A}_t, \hat{A}_t, \in\F_t$, $x_t\in\F_{t-m}$. Let $v_1,v_2$ be i.i.d. drawn from some symmetric distribution on $\mathbb{R}^d$ such that it satisfies that $\E[v_1v_1^{\top}]=r I$, and $\E[v_1v_2^{\top} Wv_1v_2^{\top}]=r^2W^{\top}$ for $W\in\mathbb{R}^{d\times d}$, $r>0$. Let $q:\mathbb{R}^d\rightarrow \mathbb{R}$ be a quadratic function. Then $\forall M\in\mathrm{Sym}(d)$ such that $M\succ 0$,
\begin{align}
\nabla q(x) &= \E_{v_1,v_2} \left[\frac{2}{r\delta}q\left(x+\frac{\delta}{2}M(v_1+v_2)\right)M^{-1}v_1\right], \label{equation:quadratic-grad}\\
\nabla^2 q &= \E_{v_1,v_2} \left[\frac{2}{r^2\delta^2}q\left(x+\frac{\delta}{2}M(v_1+v_2)\right) M^{-1}(v_1v_2^{\top}+v_2v_1^{\top})M^{-1}\right]. \label{equation:quadratic-hessian}
\end{align}
This can be checked by expanding $q(z)=\frac{1}{2}z^{\top}Az+b^{\top}z+c$ for some $A\in\mathbb{R}^{d\times d}, b\in\mathbb{R}^{d}, c\in\mathbb{R}$ and using the independence of $v_1, v_2$ and the fact that odd moments of $v_1, v_2$ are $0$. The details of the proof follows almost similarly to the proof of Proposition 1 in \cite{suggala2021efficient}. Consider the concatenated vector $v_{t-m+1:t,1}=(v_{t-m+1,1},\dots,v_{t,1})\in\mathbb{R}^{dm}$, where $v_{t-m+1,1},\dots, v_{t,1}$ are sampled i.i.d. from $S^{d-1}$. We show that $v_{t-m+1:t,1}, v_{t-m+1:t,2}$ satisfy that $\forall W\in\mathbb{R}^{dm\times dm}$,
\begin{align}
\label{equation:concated-distribution}
\E[v_{t-m+1:t,1}v_{t-m+1:t,1}^{\top}]=\frac{1}{d}I, \ \ \ \E[v_{t-m+1:t,1}v_{t-m+1:t,2}^{\top} W v_{t-m+1:t,1}v_{t-m+1:t,2}^{\top}]=\frac{1}{d^2}W^{\top}.
\end{align}
The first equality directly follows from independence and that $\E[vv^{\top}]=\frac{1}{d} I$ if $v$ is uniformly sampled from $S^{d-1}$. To see the second equality, first note that $\E[v_1v_2^{\top} U v_1v_2^{\top}]=\frac{1}{d^2}U^{\top}$, $\forall U\in\mathbb{R}^{d\times d}$, if $v_1,v_2$ are sampled i.i.d. uniformly from the unit sphere in $\mathbb{R}^{d}$. Let $W_{ij}$ denote the $(i,j)$-th $d\times d$ block of $W\in\mathbb{R}^{dm\times dm}$, i.e. $W_{ij}=W[(i-1)d+1:id, (j-1)d+1:jd]$. Then, $\forall W\in\mathbb{R}^{dm\times dm}$, 
\begin{align*}
&\E[v_{t-m+1:t,1}v_{t-m+1:t,2}^{\top} W v_{t-m+1:t,1}v_{t-m+1:t,2}^{\top}]\\
&=\E\left[\begin{bmatrix}
\sum_{j,k=t-m+1}^{t} v_{t-m+1,1}v_{k,2}^{\top}W_{k-t+m,j-t+m}v_{j,1}v_{t-m+1,2}^{\top}
& \dots & \sum_{j,k=t-m+1}^{t} v_{t-m+1,1}v_{k,2}^{\top}W_{k-t+m,j-t+m}v_{j,1}v_{t,2}^{\top} \\
\dots & \dots & \dots \\
\sum_{j,k=t-m+1}^{t} v_{t,1}v_{k,2}^{\top} W_{k-t+m,j-t+m}v_{j,1}v_{t-m+1,2}^{\top} & \dots & \sum_{j,k=t-m+1}^{t}v_{t,1}v_{k,2}^{\top}W_{k-t+m,j-t+m}v_{j,1}v_{t,2}^{\top}\\
\end{bmatrix}\right] \\
&=_{(1)}\E\left[\begin{bmatrix}
v_{t-m+1,1}v_{t-m+1,2}^{\top}W_{11}v_{t-m+1,1}v_{t-m+1,2}^{\top}
& \dots & v_{t-m+1,1}v_{t,2}^{\top}W_{m1}v_{t-m+1,1}v_{t,2}^{\top} \\
\dots & \dots & \dots \\
v_{t,1}v_{t-m+1,2}^{\top} W_{1m}v_{t,1}v_{t-m+1,2}^{\top} & \dots & v_{t,1}v_{t,2}^{\top}W_{mm}v_{t,1}v_{t,2}^{\top}\\
\end{bmatrix}\right] \\
&=\frac{1}{d^2} \begin{bmatrix}
W_{11}^{\top} & \dots & W_{m1}^{\top} \\
\dots & \dots & \dots \\
W_{1m}^{\top} & \dots & W_{mm}^{\top}
\end{bmatrix}
=\frac{1}{d^2} W^{\top},
\end{align*}
where (1) follows from independence of $\{v_{s,1}, v_{s,2}\}_{s=t-m+1}^t$ and that $\E[v_{s,1}]=\E[v_{s,2}]=0$. 

Let $\hat{M}_t=\mathrm{diag}(\hat{A}_{t-2m+1},\dots, \hat{A}_{t-m})$. Recall that $y_{t-m+1:t}=x_{t-m+1:t}+\frac{\delta}{2}\hat{M}_{t}^{-\frac{1}{2}}(v_{t-m+1:t,1}+v_{t-m+1:t,2})$. By Eq.(\ref{equation:quadratic-grad}-\ref{equation:concated-distribution}), we have that
\begin{align*}
\nabla f_t(x_{t-m+1:t}) &= \E[2d\delta^{-1}f_t(y_{t-m+1:t})\hat{M}_t^{\frac{1}{2}}v_{t-m+1:t,1}\mid\F_{t-m}], \\
\nabla^2 f_t &= \E[2d^2\delta^{-2}f_t(y_{t-m+1:t})\hat{M}_t^{\frac{1}{2}}(v_{t-m+1:t,1}v_{t-m+1:t,2}^{\top}+v_{t-m+1:t,2}v_{t-m+1:t,1}^{\top})\hat{M}_t^{\frac{1}{2}}\mid\F_{t-m}]. 
\end{align*}
Then $\E[\tilde{g}_t\mid \F_{t-m}]=\nabla\cdot f_t(x_{t-m+1:t})$ by definition. To see that $\E[\hat{H}_{t}\mid \F_{t-m}]=\nabla^2\bar{f}_{t}$, note that by expanding the matrix product in the unbiased estimator of $\nabla^2 f_t$ derived above, we have
\begin{align*}
& \ \ \ \ \ \hat{M}_t^{\frac{1}{2}}(v_{t-m+1:t,1}v_{t-m+1:t,2}^{\top}+v_{t-m+1:t,2}v_{t-m+1:t,1}^{\top})\hat{M}_t^{\frac{1}{2}}\\
&=\begin{bmatrix}
\hat{A}_{t-2m+1}^{\frac{1}{2}}(v_{t-m+1,1}v_{t-m+1,2}^{\top}+v_{t-m+1,2}v_{t-m+1,1}^{\top})\hat{A}_{t-2m+1}^{\frac{1}{2}} & \dots & \hat{A}_{t-2m+1}^{\frac{1}{2}}(v_{t-m+1,1}v_{t,2}^{\top}+v_{t,2}v_{t-m+1,1}^{\top})\hat{A}_{t-m}^{\frac{1}{2}} \\
\dots & \dots & \dots \\
\hat{A}_{t-m}^{\frac{1}{2}}(v_{t,1}v_{t-m+1,2}^{\top}+v_{t-m+1,2}v_{t,1}^{\top})\hat{A}_{t-2m+1}^{\frac{1}{2}} & \dots & \hat{A}_{t-m}^{\frac{1}{2}}(v_{t,1}v_{t,2}^{\top}+v_{t,2}v_{t,1}^{\top})\hat{A}_{t-m}^{\frac{1}{2}},
\end{bmatrix}
\end{align*}
and thus using the observation that $\nabla^2 \bar{f}_{t}=\sum_{i,j=1}^m (\nabla^2 f_t)_{ij}$, where $(\nabla^2 f_t)_{ij}$ denotes the $(i,j)$-th $d\times d$ block of $\nabla^2 f_t$, we have
\begin{align*}
\nabla^2 \bar{f}_{t}&=\E[2d^2\delta^{-2}f_t(y_{t-m+1:t})\sum_{j,k=0}^{m-1}\hat{A}_{t-j-m}^{\frac{1}{2}}(v_{t-j,1}v_{t-k,2}^{\top}+v_{t-k,2}v_{t-j,1}^{\top})\hat{A}_{t-k-m}^{\frac{1}{2}}\mid \F_{t-m}]\\
&=\E[\hat{H}_{t}\mid\F_{t-m}].
\end{align*}
\end{proof}

Lemma~\ref{lem:concentration-with-memory} shows that the constructed preconditioners $\hat{A}_{t}$ concentrate well. 

\begin{lemma} [Concentration of Hessian estimator, with-memory case] 
\label{lem:concentration-with-memory}
Let $i\in\{0,\dots,m-1\}$ satisfy that $t\in M_i$, then 
\begin{align*}
\bar{A}_{t}=\eta \sum_{s\le t, s\in M_i} \nabla^2 \bar{f}_{s}+I.
\end{align*}
Assume that $\eta \le \left(4 \left(\beta+\frac{6d^2}{\delta^2}(B+\delta\sqrt{2m}(G+\delta\sqrt{2m}\beta))\right)m^2\sqrt{T\log 2dmT^2}\right)^{-1}$. Then $\forall t$, with probability at least $1-\frac{t}{T^2}$, 
\begin{align*}
\|I-\bar{A}_{s}^{-\frac{1}{2}}\hat{A}_s\bar{A}_{s}^{-\frac{1}{2}}\|_2\le \frac{1}{2}, \ \ \forall s\le t.
\end{align*}
\end{lemma}
\begin{proof}
The proof follows similarly to the no-memory case. $\forall 0\le i\le m-1$, denote $C(i)=\{t\in[T]: t\equiv i \ \mathrm{mod} \ m\}$.

\paragraph{Base case.} For $0\le t\le m-1$, the inequality holds trivially since by algorithm definition, $\hat{A}_{0:m-1}=I=\bar{A}_{0:m-1}$. 


\paragraph{Induction hypothesis.} Assume for some $t\ge m$, with probability at least $1-\frac{t-1}{T^2}$, $\|I-\bar{A}_{s}^{-\frac{1}{2}}\hat{A}_s\bar{A}_{s}^{-\frac{1}{2}}\|_2\le\frac{1}{2}$ hold $\forall s\le t-1$. 

We show that with probability at least $1-\frac{t}{T^2}$, the inequality holds for all $s\le t$.

\paragraph{Induction.} First, assume that $\|I-\bar{A}_{s}^{-\frac{1}{2}}\hat{A}_s\bar{A}_{s}^{-\frac{1}{2}}\|_2\le\frac{1}{2}$ holds $\forall s\le t-1$. Under the assumption that $f_t$ is $\beta$-smooth, $G$-Lipschitz on $\K^m$ and $|f_t|\le B$ on $\K^m$, we can bound the loss values of the $y_t$'s actually played by
\begin{align*}
|f_t(y_{t-m+1:t})|&\le |f_t(x_{t-m+1:t})|+\|\nabla f_t(y_{t-m+1:t})\|_2\|y_{t-m+1:t}-x_{t-m+1:t}\|_2\\
&\le B+(G+\beta\|y_{t-m+1:t}-x_{t-m+1:t}\|_2)\|y_{t-m+1:t}-x_{t-m+1:t}\|_2,
\end{align*}
where 
\begin{align*}
\|y_{t-m+1:t}-x_{t-m+1:t}\|_2 =\left\|\frac{\delta}{2}\hat{A}_{t-2m+1:t-m}^{-\frac{1}{2}}(v_{t-m+1:t,1}+v_{t-m+1:t,2})\right\|_2\le \delta\sum_{s=t-2m+1}^{t-m}\|\hat{A}_{s}^{-\frac{1}{2}}\|_2\le \sqrt{2}\delta m,
\end{align*}
where the last inequality follows the assumption $\hat{A}_s\succeq \frac{1}{2}\bar{A}_{s}\succeq \frac{1}{2}I$, $\forall s\le t-1$. Therefore, $|f_t(y_{t-m+1:t})|\le B+\sqrt{2}\delta m(G+\sqrt{2}\delta \beta m )=B^*$. 

With the bound on $|f_t(y_{t-m+1:t})|$, we are one step closer to bound the desired quantity. Notice that the quantity of interest is a martingale sum, allowing the following representations: 
\begin{align*}
I-\bar{A}_{t}^{-\frac{1}{2}}\hat{A}_t\bar{A}_{t}^{-\frac{1}{2}}&=\eta \sum_{s\in M_i, s\le t} Z_s, \ \ Z_s=\bar{A}_{t}^{-\frac{1}{2}}(\nabla^2\bar{f}_{s}-\hat{H}_{s})\bar{A}_{t}^{-\frac{1}{2}},
\end{align*}
where $\E[Z_s\mid \F_{s-m}]=0$, and therefore $\sum_{s\in M_i, s\le t}Z_s$ is a martingale sum for all $i$. 
First, note that for any $u,v\in S^{d-1}$, $-2I\preceq -uu^{\top}-vv^{\top}\preceq uv^{\top}+vu^{\top}\preceq uu^{\top}+vv^{\top}\preceq 2I$. Thus, $Z_s$ can be bounded as following: 
\begin{align*}
Z_s&\in \left[-\bar{A}_{t}^{-\frac{1}{2}}\hat{H}_{s}\bar{A}_{t}^{-\frac{1}{2}}, \ \bar{A}_{t}^{-\frac{1}{2}}(m^2\beta I-\hat{H}_{s})\bar{A}_{t}^{-\frac{1}{2}}\right]\\
&\subseteq \left[-\bar{A}_{t}^{-\frac{1}{2}}\left(\frac{4d^2}{\delta^2}B^*\sum_{j,k=0}^{m-1}\hat{A}_{s-j-m}^{\frac{1}{2}}\hat{A}_{s-k-m}^{\frac{1}{2}}\right)\bar{A}_{t}^{-\frac{1}{2}}, \ \bar{A}_{t}^{-\frac{1}{2}}\left(m^2\beta I+\frac{4d^2}{\delta^2}B^*\sum_{j,k=0}^{m-1}\hat{A}_{s-j-m}^{\frac{1}{2}}\hat{A}_{s-k-m}^{\frac{1}{2}}\right)\bar{A}_{t}^{-\frac{1}{2}}\right]\\
&\subseteq \frac{4d^2}{\delta^2}B^*\left[-\sum_{j,k=0}^{m-1}(\bar{A}_{s-j-m}^{-\frac{1}{2}}\hat{A}_{s-j-m}^{\frac{1}{2}})(\hat{A}_{s-k-m}^{\frac{1}{2}}\bar{A}_{s-k-m}^{-\frac{1}{2}}), \  \frac{m^2\beta\delta^2}{4B^*d^2} I+  \sum_{j,k=0}^{m-1}(\bar{A}_{s-j-m}^{-\frac{1}{2}}\hat{A}_{s-j-m}^{\frac{1}{2}})(\hat{A}_{s-k-m}^{\frac{1}{2}}\bar{A}_{s-k-m}^{-\frac{1}{2}})\right]\\
&\subseteq_{(a)} \left[-\frac{6d^2}{\delta^2}B^*m^2 I, \ \left(\beta + \frac{6d^2}{\delta^2}B^*\right)m^2 I\right],
\end{align*}
where $(a)$ follows from the induction hypothesis that $\hat{A}_{s}\preceq \frac{3}{2}\bar{A}_{s}$, $\forall s\le t-1$. 
Thus, $\|Z_s\|_2\le \left(\beta+\frac{6d^2}{\delta^2}B^*\right)m^2$. 

\begin{lemma} [Matrix Azuma, \cite{tropp2012user}]
\label{lem:matrix-azuma}
Consider a finite adapted sequence $\left\{X_k\right\}$ of self-adjoint matrices in dimension d, and a fixed sequence $\left\{A_k\right\}$ of self-adjoint matrices that satisfy
$$
\mathbb{E}_{k-1} X_k=0 \quad \text { and } \quad X_k^2 \preceq A_k^2 \quad \text { almost surely. }
$$
Compute the variance parameter
$$
\sigma^2:=\left\|\sum_k A_k^2\right\|.
$$
Then, for all $a \ge 0$,
$$
\mathbb{P}\left\{\lambda_{\max }\left(\sum_k X_k\right) \geq a\right\} \leq d \cdot e^{-a^2 / 8 \sigma^2}. 
$$
\end{lemma}

By Lemma~\ref{lem:matrix-azuma}, union bound, and choice of $\eta$, with probability at least $1-\frac{1}{T^2}$, the following inequality:
\begin{align*}
\|I-\bar{A}_{t}^{-\frac{1}{2}}\hat{A}_t\bar{A}_{t}^{-\frac{1}{2}}\|_2&\le 4\eta \left(\beta+\frac{6d^2}{\delta^2}B^*\right)m^2\sqrt{T\log 2dmT^2}\le \frac{1}{2}.
\end{align*}
Therefore, induction hypothesis implies that
\begin{align*}
& \ \ \ \ \mathbb{P}\left(\|I-\bar{A}_{s}^{-\frac{1}{2}}\hat{A}_s\bar{A}_{s}^{-\frac{1}{2}}\|_2\le \frac{1}{2}, \forall s\le t\right)\\
&=\mathbb{P}\left(\|I-\bar{A}_{t}^{-\frac{1}{2}}\hat{A}_t\bar{A}_{t}^{-\frac{1}{2}}\|_2\le\frac{1}{2}\mid \|I-\bar{A}_{s}^{-\frac{1}{2}}\hat{A}_s\bar{A}_{s}^{-\frac{1}{2}}\|_2\le \frac{1}{2}, \forall s\le t-1\right)\\
& \ \ \ \ \ \mathbb{P}\left(\|I-\bar{A}_{t}^{-\frac{1}{2}}\hat{A}_t\bar{A}_{t}^{-\frac{1}{2}}\|_2\le \frac{1}{2}, \forall s\le t-1\right)\\
&\ge\left(1-\frac{1}{T^2}\right)\left(1-\frac{t-1}{T^2}\right)\\
&\ge 1-\frac{t}{T^2}.
\end{align*}
\end{proof}

\begin{corollary} [Bounded exploration cost]  With probability at least $1-\frac{1}{T}$, $\forall y_t$ played by Algorithm~\ref{alg:bqo-memory}, $|f_t(y_{t-m+1:t})|\le B^*=B+\sqrt{2}\delta m(G+\sqrt{2}\delta m\beta)$. 
\end{corollary}
\begin{proof}
The proof is provided in the proof of Lemma~\ref{lem:concentration-with-memory}.
\end{proof}

\begin{remark} [Well-defined preconditioners] As an immediate implication of Lemma~\ref{lem:concentration-with-memory}, $\hat{A}_{t}\succ 0$ $\forall t$ holds with probability at least $1-\frac{1}{T}$ and thus the preconditioners in Algorithm~\ref{alg:bqo-memory} are well-defined with probability at least $1-\frac{1}{T}$. 
\end{remark}

\begin{theorem}
The regret can be decomposed as
\begin{align*}
\E[\regret_T(x)]=\underbrace{\sum_{t=m}^T \E[f_t(y_{t-m+1:t})-f_t(x_{t-m+1:t})]}_{(1: \text{exploration  loss})} + \underbrace{\sum_{t=m}^T \E[f_t(x_{t-m+1:t})-\bar{f}_{t}(x_t)]}_{(2: \text{movement loss})}+\underbrace{\sum_{t=m}^T\E[\bar{f}_{t}(x_t)-\bar{f}_{t}(x)]}_{(3: \text{ONS regret})},
\end{align*}
where with probability at least $1-\frac{1}{T}$,
\begin{align*}
(1)\le C_1\delta^2 T, \ \ \ 
(2)\le C_2\frac{\eta^4T^3}{\delta^2}, \ \ \ 
(3)\le ,
\end{align*}
where 
\begin{align*}
C_1&=\frac{\beta}{m}, \ C_2=128\beta^3d^2(B^*)^2m^3,
\end{align*}
%In particular, setting $\delta=1$ and $\eta=\tilde{\Theta}(T^{-\frac{2}{3}})$, the expected regret with respect to any $x\in\K$ is bounded by $\tilde{O}(T^{\frac{2}{3}})$. 
\end{theorem}
\begin{proof}
With probability at least $1-\frac{1}{T}$, $\|I-\bar{A}_{t}^{-\frac{1}{2}}\hat{A}_{t}\bar{A}_{t}^{-\frac{1}{2}}\|_2\le \frac{1}{2}$ holds for all $t$. We prove the bounds for (1), (2), and (3) under the assumption that these inequalities hold. We begin by stating some bounds on key quantities that we will be using frequently in the proof:

\begin{lemma}
\label{lem:useful-bounds}
The following bounds hold $\forall t$: assume $\eta\beta m\le 1$,
\begin{align}
\|\hat{A}_{t}\|_2&\le \frac{3}{2}(1+\eta\beta t),\label{eqn:preconditioner-bound}\\
\|\hat{A}_{t}^{-1}\|_2&\le 2,\label{eqn:inv-preconditioner-bound}\\
\|\tilde{g}_{t}\|_2&\le \frac{5dB^*m}{2\delta}\sqrt{1+\eta\beta t}\label{eqn:grad-est-bound},\\
\frac{1}{6}\hat{A}_t &\preceq \hat{A}_{t-i}\preceq \frac{3}{2}\hat{A}_t, \ \forall 0\le i\le m-1\label{eqn:neighbor-preconditioner-bound}.
\end{align}
\end{lemma}
\begin{proof}
Eq.(\ref{eqn:preconditioner-bound}-\ref{eqn:inv-preconditioner-bound}) follows from the concentration assumption. We have that $I\preceq \bar{A}_t\preceq (1+\eta\beta t)I$ by construction. Thus,
\begin{align*}
\hat{A}_{t}\preceq \frac{3}{2}\bar{A}_t\preceq \frac{3}{2}(1+\eta\beta t)I, \ \ \  
\hat{A}_{t}^{-1}\preceq 2\bar{A}_t^{-1}\preceq 2I.
\end{align*}
By definition of $\tilde{g}_{t}$,
\begin{align*}
\|\tilde{g}_{t}\|_2&\le \frac{2dB^*}{\delta}\sum_{j=0}^{m-1}\|\hat{A}_{t-j-m}^{\frac{1}{2}}\|_2\le \frac{2dB^*}{\delta}\sum_{j=0}^{m-1}\sqrt{\frac{3}{2}}\sqrt{1+\eta \beta t}\le \frac{5dB^*m}{2\delta}\sqrt{1+\eta\beta t}. 
\end{align*}
To bound Eq.(\ref{eqn:neighbor-preconditioner-bound}), note that the second inequality in Eq.(\ref{eqn:neighbor-preconditioner-bound}) follows directly from $\hat{A}_{t-i}\preceq \frac{3}{2}\bar{A}_{t-i}\preceq\bar{A}_{t}$. To see the first inequality, it suffcies to show that $\frac{1}{2}\bar{A}_{t}\preceq \bar{A}_{t-i}$. 
\begin{align*}
\frac{1}{2}\bar{A}_{t}=\frac{1}{2}\bar{A}_{t-i}+\frac{\eta}{2} \sum_{s=t-i+1}^t \nabla^2 \bar{f}_{s}\preceq \frac{1}{2} \bar{A}_{t-i}+\frac{\eta \beta m^2}{2} I\preceq_{(a)} \bar{A}_{t-i}, 
\end{align*}
where $(a)$ follows since $\bar{A}_{t-i}\succeq mI$ and $\eta\beta m\le 1$. 
\end{proof}

\paragraph{Exploration perturbation loss.} First, we bound $(1)$. Let $u_t=\frac{1}{2}(v_{t,1}+v_{t,2})$. $y_t=x_t+\delta\hat{A}_{t-m}^{-\frac{1}{2}}u_t$. 
\begin{align*}
(1)&=\sum_{t=m}^T \E\left[\nabla f_t(x_{t-m+1:t})^{\top}(y_{t-m+1:t}-x_{t-m+1:t})+\frac{1}{2}(y_{t-m+1:t}-x_{t-m+1:t})^{\top}H_t(y_{t-m+1:t}-x_{t-m+1:t})\right]\\
&=\sum_{t=m}^T\E\left[\delta\nabla f_t(x_{t-m+1:t})^{\top}\hat{A}_{t-2m+1:t-m}^{-\frac{1}{2}}u_{t-m+1:t}+\frac{\delta^2}{2}u_{t-m+1:t}^{\top}\hat{A}_{t-2m+1:t-m}^{-\frac{1}{2}}H_t\hat{A}_{t-2m+1:t-m}^{-\frac{1}{2}}u_{t-m+1:t}\right]\\
&=\delta \sum_{t=m}^T \underbrace{\E[\E[\nabla f_t(x_{t-m+1:t})^{\top}\hat{A}_{t-2m+1:t-m}^{-\frac{1}{2}}u_{t-m+1:t}\mid\F_{t-m}]]}_{=0} \\
& \ \ \ \ \ + \frac{\delta^2}{2}\sum_{t=m}^T \E[u_{t-m+1:t}^{\top}\hat{A}_{t-2m+1:t-m}^{-\frac{1}{2}}H_t\hat{A}_{t-2m+1:t-m}^{-\frac{1}{2}}u_{t-m+1:t}]\\
&\le \frac{\delta^2\beta}{m}T\\
&= C_1\delta^2T.
\end{align*}

\paragraph{Movement loss.} (2) depends on the iterate bound on $\|x_{t-1}-x_{t}\|_2^2$. Note that by Algorithm~\ref{alg:bqo-memory}, $x_1=\dots=x_{2m-2}$. For $t\ge 2m-1$, $\|x_{t-1}-x_t\|_2^2$ can be bounded as in the following lemma:
\begin{lemma} [Iterate bound] 
\label{lem:iterate-bound}
$\forall t$, the following Euclidean distance bound holds deterministically for neighboring iterates:
\begin{align}
\|x_{t-1}-x_{t}\|_2\le \frac{8\eta dB^*}{\delta}(1+\eta\beta t) \label{eqn:iterate-bound}. 
\end{align}
\end{lemma}
\begin{proof} [Proof by induction]
By algorithm definition, $x_1=\dots=x_{2m-1}$. Suppose Eq.(\ref{eqn:iterate-bound}) holds for all $s\le t-1$ for some $t\ge 2m$. Then,
\begin{align*}
\|x_{t-1}-x_t\|_2&\le \|x_{t}-x_{t-m}\|_2+\|x_{t-m}-x_{t-m-1}\|_{2}+\|x_{t-m-1}-x_{t-1}\|_{2}\\
&\le \|x_{t}-x_{t-m}\|_2+\|x_{t-m-1}-x_{t-1}\|_{2}+ \frac{8\eta dB^*}{\delta}(1+\eta\beta (t-m)).
\end{align*}
Note that since $x_t=\Pi_{\K}^{\hat{A}_{t-m}}[x_{t-m}-\eta\hat{A}_{t-m}^{-1}\tilde{g}_{t-m}]$,
\begin{align*}
\|x_t-x_{t-m}\|_{\hat{A}_{t-m}}^2&\le \|\eta \hat{A}_{t-m}^{-1}\tilde{g}_{t-m}\|_{\hat{A}_{t-m}}^2=\eta^2 \|\tilde{g}_{t-m}\|_{\hat{A}_{t-m}^{-1}}^2,
\end{align*}
where we have further bound
\begin{align*}
\|\tilde{g}_{t-m}\|_{\hat{A}_{t-m}^{-1}}^2&=\frac{4d^2}{\delta^2}f_t(y_{t-m+1:t})^2\sum_{j,k=0}^{m-1}v_{t-j,1}^{\top}\hat{A}_{t-m-j}^{\frac{1}{2}}\hat{A}_{t-m}^{-1}\hat{A}_{t-m-k}^{\frac{1}{2}}v_{t-k,1}\\
&\le \frac{4d^2(B^*)^2}{\delta^2}\sum_{j,k=0}^{m-1}\E[\|\hat{A}_{t-m-j}^{\frac{1}{2}}\hat{A}_{t-m}^{-1}\hat{A}_{t-m-k}^{\frac{1}{2}}\|_2]\\
&\le \frac{6d^2(B^*)^2m^2}{\delta^2},
\end{align*}
and thus $\|x_{t}-x_{t-m}\|_{\hat{A}_{t-m}}^2\le \frac{6\eta^2 d^2(B^*)^2 m^2}{\delta^2}$. By Lemma~\ref{lem:useful-bounds}, we have that
\begin{align*}
\|x_t-x_{t-m}\|_{2}^2&\le \frac{2}{m}\|x_{t}-x_{t-m}\|_{\hat{A}_{t-m}}^2\le \frac{12\eta^2 d^2(B^*)^2m}{\delta^2},  
\end{align*}
and thus
\begin{align*}
\|x_{t-1}-x_t\|_2&\le \frac{8\eta dB^*m}{\delta} + \frac{8 dB^*}{\delta}(1+\eta\beta (t-m))=\frac{8 dB^*}{\delta}(1+\eta\beta t).
\end{align*}
\end{proof}
Lemma~\ref{lem:iterate-bound}
implies a bound on (2):
\begin{align*}
(2)&\le \frac{\beta}{2} \sum_{t=m}^T\E[\|x_{t-m+1:t}-(x_t,\dots,x_t)\|_2^2]\\&
=\frac{\beta}{2}\sum_{t=m}^T \sum_{s=t-m+1}^t \E[\|x_s-x_t\|_2^2]\\
&\le\frac{\beta}{2}\sum_{t=m}^T \sum_{s=t-m+1}^t (t-s)\sum_{r=s+1}^t\E[\|x_r-x_{r-1}\|_2^2]\\
&\le \frac{32\eta^2\beta d^2(B^*)^2}{\delta^2} \sum_{t=m}^T \sum_{s=t-m+1}^t (t-s)^2(1+\eta \beta t)^2\\
&\le \frac{64\eta^2\beta d^2(B^*)^2m^3}{\delta^2}\sum_{t=m}^T 1+\eta^2 \beta^2 t^2\\
&\le \frac{64\eta^4\beta^3 d^2(B^*)^2m^3T^3}{\delta^2} +\frac{64\eta^2\beta d^2(B^*)^2m^3T}{\delta^2}\\
&= C_2\frac{\eta^4T^3}{\delta^2}.
\end{align*}

\paragraph{ONS regret.} To bound the third term, first we bound the conditional bias of $\tilde{g}_{t}$ as an estimator of $\nabla\bar{f}_{t}(x_t)$:
\begin{align}
\|\E[\tilde{g}_{t}\mid\F_{t-m}]-\nabla \bar{f}_{t}(x_{t+m-1})\|_2&=_{(d)}\|\nabla\cdot f_t(x_{t-m+1:t})-\nabla\bar{f}_{t}(x_{t+m-1})\|_2\\
&\le_{(e)} \sqrt{m}\|\nabla f_t(x_{t-m+1:t}) - \nabla f_t(x_{t+m-1},\dots,x_{t+m-1})\|_2\\
&\le \sqrt{m}\beta \|x_{t-m+1:t}-(x_{t+m-1},\dots,x_{t+m-1})\|_2\\
&\le_{(f)}\frac{8\eta d\beta B^*m^{\frac{3}{2}}}{\delta}(1+\eta\beta t)\label{eqn:grad-bias-bound},
\end{align}
where $(d)$ follows from Lemma~\ref{lem:unbiased-estimators}; $(e)$ follows from the fact that $\forall a,b\in\mathbb{R}^n$, $\|\sum_{i=1}^n a_i-b_i\|_2\le \sqrt{n} \|a-b\|_2$, and $\nabla \bar{f}_t(x)=\sum_{i=1}^m \nabla_i f_t(x,\dots,x)$; $(f)$ follows from Lemma~\ref{lem:iterate-bound}. 
By the projection step in Algorithm~\ref{alg:bqo-memory}, $\forall x\in\K$,
\begin{align*}
\E[\|x_t-x\|_{\hat{A}_{t-m}}^2]&\le \E[\|x_{t-m}-x-\eta \hat{A}_{t-m}^{-1}\tilde{g}_{t-m}\|_{\hat{A}_{t-m}}^2]\\
&=\underbrace{\E[\|x_{t-m}-x\|_{\hat{A}_{t-m}}^2]}_{(g)}-2\eta \underbrace{\E[\tilde{g}_{t-m}^{\top}(x_{t-m}-x)]}_{(h)}+\eta^2\underbrace{\E[\|\tilde{g}_{t-m}\|_{\hat{A}_{t-m}^{-1}}^2]}_{(i)}.
\end{align*}
We first bound $(i)$:
\begin{align*}
\E[\|\tilde{g}_{t-m}\|_{\hat{A}_{t-m}^{-1}}^2]&=\E\left[\frac{4d^2}{\delta^2}f_t(y_{t-m+1:t})^2\sum_{j,k=0}^{m-1}v_{t-j,1}^{\top}\hat{A}_{t-m-j}^{\frac{1}{2}}\hat{A}_{t-m}^{-1}\hat{A}_{t-m-k}^{\frac{1}{2}}v_{t-k,1}\right]\\
&\le \frac{4d^2(B^*)^2}{\delta^2}\sum_{j=0}^{m-1}\E[v_{t-j,1}^{\top}\hat{A}_{t-m-j}^{\frac{1}{2}}\hat{A}_{t-m}^{-1}\hat{A}_{t-m-j}^{\frac{1}{2}}v_{t-j,1}]\\
&\le \frac{4d^2(B^*)^2}{\delta^2}\sum_{j=0}^{m-1}\E[\|\hat{A}_{t-m-j}^{\frac{1}{2}}\hat{A}_{t-m}^{-1}\hat{A}_{t-m-j}^{\frac{1}{2}}\|_2]\\
&\le \frac{6d^2(B^*)^2m}{\delta^2},
\end{align*}
where the last equality follows from Lemma~\ref{lem:useful-bounds}.
$(g),(h)$ can be bounded by
\begin{align*}
(g)&=\E[\|x_{t-m}-x\|_{\hat{A}_{t-m-1}}^2] + \eta\E[\|x_{t-m}-x\|_{\hat{H}_{t-m}}^2]\\
&= \E[\|x_{t-m}-x\|_{\hat{A}_{t-m-1}}^2] + \eta\E[\E[\|x_{t-m}-x\|_{\hat{H}_{t-m}}^2\mid\F_{t-2m}]]\\
&=\E[\|x_{t-m}-x\|_{\hat{A}_{t-m-1}}^2] + \eta\E[\|x_{t-m}-x\|_{\E[\hat{H}_{t-m}\mid\F_{t-2m}]}^2]\\
&=\E[\|x_{t-m}-x\|_{\hat{A}_{t-m-1}}^2]+\eta \E[\|x_{t-m}-x\|_{\nabla^2 \bar{f}_{t-m}}^2],\\
(h)&=\E[(\tilde{g}_{t-m}-\nabla \bar{f}_{t-m}(x_{t-m}))^{\top}(x_{t-m}-x)]+\E[\nabla\bar{f}_{t-m}(x_{t-m})^{\top}(x_{t-m}-x)]\\
&\le \E[(\E[\tilde{g}_{t-m}\mid \F_{t-2m}]-\nabla\bar{f}_{t-m}(x_{t-m}))^{\top}(x_{t-m}-x)]+\E[\nabla\bar{f}_{t-m}(x_{t-m})^{\top}(x_{t-m}-x)]\\
&\le \frac{8\eta d\beta DB^*m^{\frac{3}{2}}}{\delta}(1+\eta\beta t)+\E[\nabla\bar{f}_{t-m}(x_{t-m})^{\top}(x_{t-m}-x)].
\end{align*}
Putting together, we have
\begin{align*}
\frac{1}{\eta}\E[\|x_t-x\|_{\hat{A}_{t-m}}^2]&\le \frac{1}{\eta}\E[\|x_{t-m}-x\|_{\hat{A}_{t-m-1}}^2] + \E[\|x_{t-m}-x\|_{\nabla^2\bar{f}_{t-m}}^2] - 2\E[\nabla \bar{f}_{t-m}(x_{t-m})^{\top}(x_{t-m}-x)] \\
& \ \ \ \ \ + C_3 \frac{\eta}{\delta^2}+C_4\frac{\eta(1+\eta\beta t)}{\delta},
\end{align*}
where $C_3 =6d^2(B^*)^2m, C_4=8d\beta DB^*m^{\frac{3}{2}}$.
Rearranging, we have
\begin{align*}
\E[\nabla\bar{f}_{t-m}(x_{t-m})^{\top}(x_{t-m}-x)]-\frac{1}{2}\E[\|x_{t-m}-x\|_{\nabla^2\bar{f}_{t-m}}^2]&\le \frac{1}{\eta}(\E[\|x_{t-m}-x\|_{\hat{A}_{t-m-1}}^2]-\E[\|x_t-x\|_{\hat{A}_{t-m}}^2])\\
& \ \ \ \ \ +C_3 \frac{\eta(1+\eta\beta t)}{\delta^2}  +C_4\frac{\eta\sqrt{1+\eta\beta t}}{\delta}.
\end{align*}
\end{proof}

\newpage



==> content/BQO.tex <==
\begin{algorithm}[H]
\caption{(Proper) Bandit Newton Step }\label{alg:simple-bqo-proper}
\begin{flushleft}
  {\bf Input:} convex set $\K$, self-concordant barrier $R$ of $\K$, step size $\eta$, condition number $\kappa'$
\end{flushleft}
\begin{algorithmic}[1]
\STATE Initialize: $x_1 = \argmin_{x\in \K}R(x), \tilde{H}_{0}=0$
\FOR{$t = 1, \ldots, T$}
\STATE Update $\tilde{A}_{t} = \nabla^2 R(x_t) + \frac{\eta}{\kappa'} \sum_{s=0}^{t-1}\tilde{H}_s $,
\STATE Draw $v_{t,1}$ and $v_{t,2}$ uniformly from $\sphere = \{x\in\real^d|\|x\|_2 = 1\}$, and let $y_t=x_t+\frac{1}{4} \tilde{A}_{t}^{-\frac{1}{2}}(v_{t,1}+v_{t,2})$.
\STATE Play $y_t$, observe $f_t(y_t)$.
\STATE Create gradient and Hessian estimates $\tilde{\nabla}_t,\tilde{H}_t$:
\begin{align*}
\tilde{\nabla}_{t}=4df_t(y_t) \tilde{A}_{t}^{\frac{1}{2}}v_{t,2}, \ \ \ \tilde{H}_{t}=8d^2 f_t(y_t)\tilde{A}_{t}^{\frac{1}{2}}(v_{t,1}v_{t,2}^{\top}+v_{t,2}v_{t,1}^{\top})\tilde{A}_{t}^{\frac{1}{2}}.
\end{align*}
\STATE  Compute $x_{t+1}$
\begin{align*}
&x_{t+1} = \argmin_{x\in \K} \eta\left\langle\tilde{\nabla}_t, x\right\rangle + \bregt{t+1}(x,x_{t})
\end{align*}
Here $\bregt{t+1}$ is  Bregman divergence w.r.t \mbox{$R_{t+1}(x) \stackrel{\text{def}}{=} R(x) + \underset{s=0}{\overset{t}{\sum}}\frac{\eta}{2\kappa'}(x-x_s)^T\tilde{H}_{s}(x-x_s)$}
\ENDFOR 
\end{algorithmic}
\end{algorithm}



Observe that Algorithm~\ref{alg:simple-bqo} is an improper learning algorithm; that is, it plays actions that lie outside the constraint set $\K$. We now make our algorithm proper by introducing self-concordant barriers (SCB), and replacing the traditional Newton step in Algorithm~\ref{alg:simple-bqo} with Online Mirror Descent (OMD) step (see Appendix~\ref{sec:scb} for an overview of SCBs).


==> header.tex <==
% packages
\usepackage{amsmath,amsfonts, amssymb}
\usepackage{mathtools}
\usepackage{amsthm} % better to load after ams math
\usepackage{latexsym}
\usepackage{relsize}
%\usepackage{thmtools,thm-restate}
%\usepackage[amsthm]{ntheorem}
\newcommand{\equaldef}{\stackrel{\text{\tiny def}}{=}}


\usepackage[margin=1.3in]{geometry}

\setlength\parindent{0pt}


\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
% \usepackage{amsfonts}       % blackboard math symbols
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{braket}
% \usepackage[colorinlistoftodos]{todonotes}


\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
% \usepackage{color}         % colors
% \usepackage[colorinlistoftodos]{todonotes}
\usepackage[shortlabels]{enumitem}
\usepackage[bbgreekl]{mathbbol}
\usepackage{mdframed}


\DeclareSymbolFontAlphabet{\mathbb}{AMSb}
\DeclareSymbolFontAlphabet{\mathbbl}{bbold}




\usepackage[capitalise]{cleveref}
% \usepackage{xcolor}
\usepackage{dsfont}

\newcommand{\softmax}{\text{softmax}}
\newcommand{\CH}{\text{CH}}
\newcommand{\F}{\mathbb{F}}

\newtheorem{prop}{Proposition}





\usepackage{tikz}
\usetikzlibrary{positioning}
% \usepackage{floatrow}
% Table float box with bottom caption, box width adjusted to content
\usepackage{makecell}
\usetikzlibrary{fit}
\usetikzlibrary{shapes.geometric}








\def\lhat{\hat{\ell}}

\def\ch{\mathbf{CH}}
\newcommand{\zetaB}{\mbox{\boldmath$\zeta$\unboldmath}}
\newcommand{\RBB}{\mathbb{R}}
\newcommand{\EBB}{\mathbb{E}}
\newcommand{\PBB}{\mathbb{P}}
\newcommand{\FM}{\mathcal{F}}
% \newcommand{\O}{\mathcal{O}}

\newcommand\ball{\mathbb{B}}
\newcommand\sphere{\mathbb{S}}
\newcommand{\vv}{\ensuremath{\mathbf v}}

\newcommand{\defeq}{\stackrel{\text{def}}{=}}
\newcommand{\elad}[1]{$\ll$\textsf{\color{blue} Elad : #1}$\gg$}
\newcommand{\FIX}[1]{\textsf{\color{red} FIX ME : #1}}
\def\ltil{{{\tilde{\ell}}}}
\def\btalpha{{\bm{\tilde{\alpha}}}}
\def\balpha{{\bm{\alpha}}}
\def\talpha{{\tilde{\alpha}}}
\def\btbeta{{\bm{\tilde{\beta}}}}
\def\bbeta{{\bm{\beta}}}
\def\tbeta{{\tilde{\beta}}}
\def\btgamma{{\bm{\tilde{\gamma}}}}
\def\bgamma{{\bm{\gamma}}}
\def\tgamma{{\tilde{\gamma}}}

\newcommand{\g}{\mathbf{g}}


\def\X{{\mathcal X}}
\def\H{{\mathcal H}}
\def\Y{{\mathcal Y}}
\def\W{{\mathcal W}}
\def\R{{\mathcal R}}
\def\S{{\mathcal S}}
\def\SP{{\mathbb S}}
\def\B{{\mathbb B}}
\def\E{{\mathbb E}}
% \newcommand{\E}{\mathbb{E}}

% notation here
\newcommand{\ftil}{\tilde{f}}

\def\hestinv{\tilde{\nabla}^{-2}}
\def\hest{\tilde{\nabla}^{2}}
\def\hessinv{\nabla^{-2}}
\def\hess{\nabla^2}
\def\grad{\nabla}


% notation

\newcommand{\re}{{\text{Re}}}
%\newcommand{\R}{\mathcal{R}}
%\newcommand{\C}{\mathcal{C}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\cE}{\mathcal{E}}
\renewcommand{\sp}{\mathrm{span}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\cor}{\mathrm{cor}}
\newcommand{\sign}{\text{ } \mathrm{sign}}

\def\W{{\mathcal W}}
\def\mA{{\mathcal A}}
\def\fhat{{\hat{f}}}


\newcommand{\bzero}{\ensuremath{\mathbf 0}}
\newcommand{\ba}{\ensuremath{\mathbf a}}
\newcommand{\y}{\ensuremath{\mathbf y}}
\newcommand{\z}{\ensuremath{\mathbf z}}
\newcommand{\h}{\ensuremath{\mathbf h}}
\newcommand{\K}{\ensuremath{\mathcal K}}
\renewcommand\L{\mathcal{L}}
\renewcommand\F{\mathcal{F}}
%\newcommand{\C}{\ensuremath{\mathcal C}}

\def\bb{\mathbf{b}}
%\def\bc{\mathbf{c}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\C{{\mathcal C}}

%\def\be{\mathbf{e}}
\def\etil{\tilde{\mathbf{e}}}
%\def\bk{\mathbf{k}}
\def\bu{\mathbf{u}}
\def\x{\mathbf{x}}
\def\y{\mathbf{y}}
\def\w{\mathbf{w}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}

\def\bw{\mathbf{w}}
%\def\ba{\mathbf{a}}
\def\bA{\mathbf{A}}
\def\bS{\mathbf{S}}
\def\bG{\mathbf{G}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bV{\mathbf{V}}
\def\bone{\mathbf{1}}

\def\regret{\mbox{{Regret}}}
\def\mregret{\mbox{{MemoryRegret}}}
\def\mregret{\mbox{{ControlRegret}}}

\def\ytil{\tilde{{y}}}
\def\yhat{\hat{{y}}}
\def\what{\hat{{w}}}
\def\xhat{\hat{\mathbf{x}}}
\def\xbar{\bar{\mathbf{x}}}


% comments, etc
\newcommand{\ignore}[1]{}
\newcommand{\nb}[1]{\noindent{\textcolor{cyan}{\{{\bf nataly:} \em #1\}}}}
\newcommand{\ar}[1]{\noindent{\textcolor{red}{\{{\bf arun:} \em #1\}}}}
\newcommand{\eh}[1]{\noindent{\textcolor{blue}{\{{\bf EH:} \em #1\}}}}
\newcommand{\pn}[1]{\noindent{\textcolor{blue}{\{{\bf PN:} \em #1\}}}}
\newcommand{\js}[1]{\noindent{\textcolor{blue}{\{{\bf JS:} \em #1\}}}}
\newcommand{\kl}[1]{\noindent{\textcolor{magenta}{\{{\bf KL:} \em #1\}}}}
\newcommand{\ks}[1]{\noindent{\textcolor{orange}{\{{\bf KS:} \em #1\}}}}
\newcommand{\hl}[1]{\noindent{\textcolor{purple}{\{{\bf HL:} \em #1\}}}}
% for emails
\newcommand{\email}[1]{\texttt{#1}}
\newcommand{\bregt}[1]{\Phi_{R_{#1}}}

%% JMLR theorems adjustments
%\setlength{\topsep}{\medskipamount}
%
%\newtheoremstyle{jmlrthm} % name
%	{\topsep}		% Space above
%	{\topsep}		% Space below
%	{\itshape}	% Body font
%	{}						% Indent amount
%	{\bfseries}	% Theorem head font
%	{}						% Punctuation after theorem head
%	{0.33em}		% Space after theorem head
%	{}  					% Theorem head spec (can be left empty, meaning ?normal?)
%
%\newtheoremstyle{jmlrdef} % name
%	{\topsep}		% Space above
%	{\topsep}		% Space below
%	{}						% Body font
%	{}						% Indent amount
%	{\bfseries}	% Theorem head font
%	{}						% Punctuation after theorem head
%	{.33em}			% Space after theorem head
%	{}  					% Theorem head spec (can be left empty, meaning ?normal?)
%
%\renewcommand\qedsymbol{\BlackBox}
%%\renewenvironment{proof}[1][Proof]{\par\noindent{\bfseries\upshape #1\ }}{\hfill\BlackBox\\[\medskipamount]}
%\renewenvironment{proof}[1][Proof]{\par\noindent{\bfseries\upshape #1\ }}{\hfill\BlackBox\\}


% theorems
\theoremstyle{plain}
%\theoremstyle{jmlrthm}
% \newtheorem{theorem}{Theorem}[section]
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}

\newtheorem*{theorem*}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem*{corollary*}{Corollary}
\newtheorem*{proposition*}{Proposition}
\newtheorem*{claim*}{Claim}
\newtheorem*{fact*}{Fact}
\newtheorem*{observation*}{Observation}
\newtheorem*{assumption*}{Assumption}

\theoremstyle{definition}
%\theoremstyle{jmlrdef}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem*{definition*}{Definition}
\newtheorem*{remark*}{Remark}
\newtheorem*{example*}{Example}


% repeated theorems
\theoremstyle{plain}
%\theoremstyle{jmlrthm}
\newtheorem*{theoremaux}{\theoremauxref}
\gdef\theoremauxref{1}

\newenvironment{repthm}[2][]{%
    \def\theoremauxref{\cref{#2}}
    \begin{theoremaux}[#1]
    }{%
    \end{theoremaux}
}

%\newtheoremstyle{theoremrep}
%	{\topsep}{\topsep}              %%% space between body and thm
%	{\itshape}                      %%% Thm body font
%	{}                              %%% Indent amount (empty = no indent)
%	{\bfseries}                     %%% Thm head font
%	{}                             %%% Punctuation after thm head
%	{0.33em}                             %%% Space after thm head
%	{\cref{#3}}
%
%\theoremstyle{theoremrep}
%\newtheorem{repthm}{dontcare}


% % old refs - use \cref{} instead!
% \newcommand{\secref}[1]{Section~\ref{#1}}
%\newcommand{\secref}[1]{Sec.~\ref{#1}}
%\newcommand{\figref}[1]{Figure~\ref{#1}}
%\renewcommand{\eqref}[1]{Eq.~(\ref{#1})}
%\newcommand{\lemref}[1]{Lemma~\ref{#1}}

% \newcommand{\thmref}[1]{Theorem~\ref{#1}}
% \newcommand{\appref}[1]{Appendix~\ref{#1}}
% \newcommand{\algref}[1]{Algorithm~\ref{#1}}

% style defs
%\renewcommand{\le}{\leqslant}
%\renewcommand{\ge}{\geqslant}
%\renewcommand{\leq}{\le}
%\renewcommand{\geq}{\ge}

% bold serif
\DeclareMathAlphabet{\mathbfsf}{\encodingdefault}{\sfdefault}{bx}{n}

% operators
\DeclareMathOperator*{\err}{error}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\supp}{supp}
%\DeclareMathOperator*{\poly}{poly}
\let\Pr\relax
\DeclareMathOperator{\Pr}{\mathbb{P}}

% cases
\newcommand{\mycases}[4]{{
    \left\{
    \begin{array}{ll}
    {#1}
        & {\;\text{#2}} \\[1ex]
        {#3} & {\;\text{#4}}
    \end{array}
    \right. }}

\newcommand{\mythreecases}[6] {{
    \left\{
    \begin{array}{ll}
    {#1}
        & {\;\text{#2}} \\[1ex]
        {#3} & {\;\text{#4}} \\[1ex]
        {#5} & {\;\text{#6}}
    \end{array}
    \right. }}

% macros
\newcommand{\lr}[1]{\!\left(#1\right)\!}
\newcommand{\lrbig}[1]{\big(#1\big)}
\newcommand{\lrBig}[1]{\Big(#1\Big)}
\newcommand{\lrbra}[1]{\!\left[#1\right]\!}
\newcommand{\lrnorm}[1]{\left\|#1\right\|}
\newcommand{\lrset}[1]{\left\{#1\right\}}
\newcommand{\lrabs}[1]{\left|#1\right|}
%\newcommand{\set}[1]{\{#1\}}
\newcommand{\abs}[1]{|#1|}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\renewcommand{\t}[1]{\smash{\tilde{#1}}}
\newcommand{\wt}[1]{\smash{\widetilde{#1}}}
\newcommand{\wh}[1]{\smash{\widehat{#1}}}
\renewcommand{\O}{\mathcal{O}}
%\renewcommand{\O}{\mathcal{O}}
\newcommand{\OO}[1]{\O\lr{#1}}
\newcommand{\tO}{\wt{\O}}
\newcommand{\tTheta}{\wt{\Theta}}
% \newcommand{\E}{\mathbb{E}}
\newcommand{\EE}[1]{\E\lrbra{#1}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\tsum}{\sum\nolimits}
\newcommand{\trace}{\mathrm{tr}}
\newcommand{\ind}[1]{\mathbb{I}\!\lrset{#1}}
\newcommand{\non}{\nonumber}
\newcommand{\poly}{\mathrm{poly}}

% \newcommand{\tr}{^{\mathsmaller\top}}
\newcommand{\tr}{^{\mkern-1.5mu\mathsf{T}}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\st}{\star}
\renewcommand{\dag}{\dagger}

%\newcommand{\kl}[2]{\mathsf{D}_\mathrm{KL}(#1,#2)}
\newcommand{\tv}[2]{\mathsf{D}_{\mathrm{TV}}(#1,#2)}
\newcommand{\ent}{\mathsf{H}}
\newcommand{\info}{\mathsf{I}}

\newcommand{\reals}{\mathbb{R}}
\newcommand{\eps}{\varepsilon}
\newcommand{\ep}{\varepsilon}
%\newcommand{\eps}{\epsilon}
\newcommand{\sig}{\sigma}
\newcommand{\del}{\delta}
\newcommand{\Del}{\Delta}
\newcommand{\lam}{\lambda}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\thalf}{\tfrac{1}{2}}

\newcommand{\eqdef}{:=}
\newcommand{\eq}{~=~}
\renewcommand{\leq}{~\le~}
\renewcommand{\geq}{~\ge~}
\newcommand{\lt}{~<~}
\newcommand{\gt}{~>~}
\newcommand{\then}{\quad\Rightarrow\quad}

\let\oldtfrac\tfrac
\renewcommand{\tfrac}[2]{\smash{\oldtfrac{#1}{#2}}}

\def\dist{{\bf Dist}}

\let\nablaold\nabla
\renewcommand{\nabla}{\nablaold\mkern-2.5mu}
%\let\cdotold\cdot
%\renewcommand{\cdot}{\mkern-2.5mu\cdotold\mkern-2.5mu}
%\newcommand{\param}{\cdotold}


%\newcommand{\diag}{\mathrm{diag}}
\newcommand{\nf}[2]{\nicefrac{#1}{#2}}
\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mat}[1]{\bm{#1}}
\newcommand{\ten}[1]{\mathcal{#1}}
\newcommand{\frob}[1]{\|#1\|_2}
\newcommand{\p}[2]{\textrm{Pr}[ #1\in #2] }
\newcommand{\pe}[2]{\mathop{\textrm{Pr}}\limits_{#1}\left[#2\right] }
%\newcommand{\one}[1]{\mathds{1}[#1]}
\newcommand{\inp}[2]{\left\langle #1,#2\right\rangle}
\newcommand{\beps}{\bm{\eps}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\RE}[3]{\E{#1}{\sup_{#2}#3}}
%\newcommand{\rc}[1]{R\left(#1\right)}



\newcommand{\EEc}[2]{\mathbb{E}\left[#1\left|#2\right.\right]}
\newcommand{\EEcc}[2]{\mathbb{E}\left[\left.#1\right|#2\right]}
\newcommand{\EEcs}[3]{\mathbb{E}_{#3}\left[\left.#1\right|#2\right]}
\newcommand{\EEcct}[2]{\mathbb{E}_t\left[\left.#1\right|#2\right]}


\newcommand{\pa}[1]{\left(#1\right)}
\newcommand{\bpa}[1]{\bigl(#1\bigr)}


\usepackage{bbm}
\newcommand{\loss}{\ell}
\newcommand{\hloss}{\wh{\ell}}
\newcommand{\tloss}{\wt{\ell}}
\newcommand{\rew}{r}
\newcommand{\hrew}{\wh{\rew}}
\newcommand{\trew}{\wt{\rew}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\Dw}{\mathcal{D}}
\newcommand{\Sw}{\mathcal{S}}
\newcommand{\Rw}{\mathcal{R}}
 \newcommand{\tOO}{\wt{\OO}}
\newcommand{\II}[1]{\mathbb{I}_{\left\{#1\right\}}}
\newcommand{\I}[1]{\mathbbm{1}{\left[#1\right]}}
\newcommand{\PP}[1]{\mathbb{P}\left[#1\right]}
 \newcommand{\PPt}[1]{\mathbb{P}_t\left[#1\right]}
\newcommand{\EEt}[1]{\mathbb{E}_t\left[#1\right]}
 \newcommand{\ev}[1]{\left\{#1\right\}}

 \newcommand{\G}{\mathcal{G}}
\newcommand{\hI}{\widehat{I}}
\newcommand{\tI}{\widetilde{I}}
\newcommand{\tp}{\wt{p}}
\newcommand{\tq}{\wt{q}}
\newcommand{\tC}{\widetilde{C}}
\newcommand{\tR}{\widetilde{R}}
 \renewcommand{\th}{\ensuremath{^{\mathrm{th}}}}
\def\argmin{\mathop{\rm arg\, min}}
\newcommand{\hL}{\wh{L}}
\newcommand{\tL}{\wt{L}}
 \newcommand{\simt}{\stackrel{t}{\sim}}
\newcommand{\simtm}{\stackrel{t-1}{\sim}}
\newcommand{\simtp}{\stackrel{t+1}{\sim}}

   
\newcommand{\exph}{\textsc{Exp3}\xspace}
\newcommand{\exphix}{\textsc{Exp3-IX}\xspace}
\newcommand{\exphp}{\textsc{Exp3.P}\xspace}
\newcommand{\expn}{\textsc{Exp4}\xspace}
\newcommand{\expnix}{\textsc{Exp4-IX}\xspace}
\newcommand{\expnp}{\textsc{Exp4.P}\xspace}
\newcommand{\exphs}{\textsc{Exp3.S}\xspace}
\newcommand{\exphsix}{\textsc{Exp3-SIX}\xspace}
\newcommand{\lexph}{\textsc{LazyExp2}\xspace}
\newcommand{\hedge}{\textsc{Hedge}\xspace}
\newcommand{\green}{\textsc{Green}\xspace}
\newcommand{\polyinf}{\textsc{PolyINF}\xspace}
\newcommand{\osmd}{\textsc{OSMD}\xspace}
\newcommand{\scrible}{\text{SCRiBLe}\xspace}
\newcommand{\ra}{\rightarrow}
\newcommand{\transpose}{^\mathsf{\scriptscriptstyle T}}

 \newcommand{\onenorm}[1]{\norm{#1}_1}
\newcommand{\infnorm}[1]{\norm{#1}_\infty}



\usepackage{todonotes}
\definecolor{PalePurp}{rgb}{0.66,0.57,0.66}
\newcommand{\todoG}[1]{\todo[color=PalePurp!30]{#1}}
\newcommand{\todoGI}[1]{\todo[inline,color=PalePurp!30]{#1}}

  
 
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}
 
\DeclareSymbolFontAlphabet{\mathbb}{AMSb}

\newcommand{\gest}[1]{\tilde{\nabla}_{#1}}
\newcommand{\hestn}[1]{\tilde{H}_{#1}}
\newcommand{\func}{\mathbf{ f}}
\newcommand{\iprod}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\fiprod}[2]{\left\langle #1, #2 \right\rangle_F}
\newcommand{\that}{\widehat{t}}

\newcounter{lecounter}
\newcommand{\labeledle}[1]{%
    \refstepcounter{\lecounter}%
    \label{le:#1}%
    \le_{\text{\normalfont\footnotesize\ref{\le:#1}}}%
}

\newcommand{\first}{\underset{\dot{}}{m}}

% Control symbols
\newcommand{\uv}{\mathbf{u}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\ynat}{\mathbf{y}^{K}}
\newcommand{\xnat}{\mathbf{x}^{K}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\embed}{\mathfrak{e}}

\newcommand{\smoothfBS}[1]{\Tilde{f}_{#1}^{\ball,\sphere}}
\newcommand{\smoothfSS}[1]{\Tilde{f}_{#1}^{\sphere,\sphere}}
\newcommand{\smoothfBB}[1]{\Tilde{f}_{#1}^{\ball,\ball}}

